Two-Sided Time-Independent Regret for Matching Markets with Limited Interviews

Two-sided matching platforms rely on preferences from both sides, yet participants can evaluate only a small fraction of potential partners. In practice, they use low-cost pre-match screening, e.g., interviews, profile views, or trial tasks, to form noisy impressions before committing to applications and offers. We study bandit learning in matching markets with interviews, modeling these interactions as queried \emph{hints}~\citep{DBLP:conf/innovations/BhaskaraGIKM23} that reveal partial preference information to both sides while constraining subsequent applications. Our framework also allows firm-side uncertainty: firms, like agents, learn their preferences and may make early hiring mistakes. To address this, we introduce strategic deferral, a firm-side action that permits temporary vacancy, corrects premature commitments, and enables decentralized learning under coarse anonymous feedback. We design algorithms for centralized and decentralized markets and show that a constant number of interviews per round suffices for horizon-independent regret, improving over the $O(\log T)$ guarantees known without interviews. Our bounds are near-optimal: the centralized guarantee is within a factor $m$ of an information-theoretic lower bound, while decentralized algorithms match it up to polynomial factors in structured markets and remain horizon-independent in general markets.

==> AllP.tex <==
\section{Single Agent Bandits with Hints}
\subsection{$\ALLP$ Algorithm \cite{bhaskara2022online}}
In this section we utilize another estimator named $\UCB'$ which is a function of sample mean and variance. So, we would have
$$ \label{cucbp:1}
\hat{\mu}_{a,f}(t)=\frac{\sum_{t'\in T_{a,f}(t)} X_{a,f}(t')}{T_{a,f}(t)} \quad \hat{\sigma}^2_{a,f}(t)=\frac{\sum_{t'\in T_{a,f}(t)}\left(X_{a,f}(t')-\hat{\mu}_{a,f}(t)\right)^2}{T_{a,f}(t)}
$$
Now we define
\begin{align}\label{cucbp:2}
\hat{u}_{a,f}(t) = \UCB'_{a,f}(t) = \hat{\mu}_{a,f}(t) + \epsilon\hat{\sigma}^2_{a,f}(t)
\end{align} 
The $\ALLP$ algorithm utilizes $\UCB'$s to query for hints, achieving constant regret for a single learner aiming to identify the best arm based on its corresponding distribution mean. The author proved that as few as three queried observations are sufficient to achieve constant regret. In the $\ALLP$ algorithm, learner $a$ queries the arms with the first and second highest $\UCB'_a$ values, $f_a^1(t)$ and $f_a^2(t)$ and pulls the arm with the higher reward. The third observation is conducted in a \emph{Round-Robin} manner, and this arm is never pulled. The algorithm then updates $\hat{\mu}_{a,f}(t)$ and $\hat{\sigma}^2_{a,f}(t)$. The regret is also defined as
\begin{align}
R_{a}(T) \coloneqq T u_{a,f^1_a} - \sum_{t=1}^T \min\left\{u_{a,f^1_a}, \mathbb{E}\left[\max\left\{ X_{a,f^2_a(t)}(t), X_{a,f^{2}_a(t)}(t)\right\}\right]\right\} \label{reg:ap}
\end{align}


\begin{algorithm}[H]
\caption{$\ALLP$}\label{alg:ap}
\begin{algorithmic}[1]
\Require $T$, $i$
\For{$ t \in  [T]$}
\State Observe $X_{t \% m,t}(t)$
\State Observe $X_{a,f^1_a(t)}(t)$
\State Observe $X_{a,f^{2}_a(t)}(t)$
\State Pull the arm corresponding to $\arg\max\left\{X_{a,f^1_a(t)}(t), X_{a,f^{2}_a(t)}(t)\right\}$
\State Update $\hat{u}_a(t+1)$ using equation \eqref{cucbp:2}
\EndFor
\end{algorithmic}
\end{algorithm}

The main result of this work is presented in the following theorem:

\begin{theorem}\label{thm:apreg}
    Under a collision-free model, the regret of the $\ALLP$ algorithm for an agent $a$ is $R_a(T) \in O\left(m^2\right)$.
\end{theorem}
The proof of Theorem \ref{thm:apreg} is highly dependent on the following Lemma:

\begin{lemma}\label{lemma:RPI}
    Let $X$ and $Y$ be independent random variables supported on $[0,1]$ whose means satisfy $\mu_Y \geq \mu_X$, and let $Z=\max \{X, Y\}$. Then \[\mathbf{E}[Z] \geq \mu_X+\sigma_X^2 / 2,\]
\end{lemma}
where this inequality is called \emph{Reverse Prophet Inequality}.


\subsubsection{The intuition behind the proof of Theorem \ref{thm:apreg}}
Let us assume agent $a$ is at the topmost layer of the underlying $\alpha$-reducible market, with its match denoted by $f^*_a$. By the definition of $\alpha$-reducible markets, this pair $(a, f^*_a)$ prefers each other the most. This agent employs the $\ALLP$ algorithm, and we assume a collision-free dynamic for now to analyze the regret of $a$ independently. Theorem \ref{thm:apreg} implies that after $m^2$ rounds of round-robin observations, the arms are sorted in a structured order such that if an arm $f \neq f^*_a$ has a greater $\UCB'$ value than $f^*_a$, i.e., $\hat{u}_a(f) > \hat{u}_a(f^*_a)$, then $\sigma^2_{a,f} \geq 2\Delta_{a,f}$, where $\Delta_{a,f} \doteq u_a(f^*_a) - u_a(f)$. By the results of Lemma \ref{lemma:RPI}, the Reverse Prophet Inequality, the $\ALLP$ algorithm suffers from zero regret from that moment till the end of the game, according to the regret definition \eqref{reg:ap}, since $u_a(f^*_a) = u_a(f) + \Delta_{a,f}$.

\subsubsection{Extended $\ALLP$ algorithm} \label{sec:eap}
Unlike the classical multi-armed bandit problem, where the goal is to find the best arm, in matching markets it may be more important to identify the $i$-th best arm. To address this, we propose an algorithm called Extended $\ALLP$ ($\EAP$), which extends the standard $\ALLP$ method to identify the $i$-th top arm.

The regret for this algorithm is defined as:

\begin{align}
R^i_{a}(T) \coloneqq T u_{a,f^i_a} - \sum_{t=1}^T \min\left\{u_{a,f^i_a}, \mathbb{E}\left[\max\left\{ X_{a,f^i_a(t)}(t), X_{a,f^{i+1}_a(t)}(t)\right\}\right]\right\} \label{reg:eap}
\end{align}

where $u_{a,f^i_a}$ represents the utility of agent $a$ for their $i$-th preferred arm with respect to $u_{a,f}$. 
The $\EAP$ algorithm is detailed below:


\begin{algorithm}[H]
\caption{Extended $\ALLP$ ($\EAP$)}\label{alg:eap}
\begin{algorithmic}[1]
\Require $T$, $i$
\For{$ t \in  [T]$}
\State Observe $X_{t \% m,t}(t)$
\State Observe $X_{a,f^i_a(t)}(t)$
\State Observe $X_{a,f^{i+1}_a(t)}(t)$
\State Pull the arm corresponding to $\arg\max\left\{X_{a,f^i_a(t)}(t), X_{a,f^{i+1}_a(t)}(t)\right\}$
\State Update $\hat{u}_a(t+1)$ using equation \eqref{cucbp:2}
\EndFor
\end{algorithmic}
\end{algorithm}

In the regret expression, when an arm with a mean greater than $u_{a,f^i_a}$ appears in the $i$-th or $i+1$-th position of the sorted $\UCB'$s, the regret is zero. Therefore, the goal is to bound the total number of times when arms with means less than or equal to $u_{a,f^i_a}$ are selected.

We define the sets $U_a$ and $L_a$ as follows:
\[
U_a = \{f \in \mathcal{F} : u_{a,f} > u_{a,f^i_a}\}, \quad L_a = \{f \in \mathcal{F} : u_{a,f} \leq u_{a,f^i_a}\}
\]

Next, we need to bound the total number of times an arm $f \in U_a$ appears in the indices in $[i:m]$ of the sorted $\hat{u}_a$ that contributes to zero regret until time step $t$, denoted by $Z_{a,f}(t)$. To bound $Z_{a,f}(t)$, we use the following tail bounds from Audibert \etal \cite{audibert2009exploration}:


Finally, the regret of the Extended $\ALLP$ ($\EAP$) algorithm can be bounded as follows:

\begin{theorem}\label{thm:eap-regret}
    Assuming $t \geq m^2$, the regret of $\EAP$ satisfies:
    \[
    R_{a,f}(T) \leq O(m^2) + \sum_{s>t} 9 m^2 \Delta^{\max}_a e^{-c \Delta^{\min}_a \frac{s}{m}} \leq O(m^2).
    \]
\end{theorem}


The intuition behind this theorem is that having no conflict (every agent be a single learner) among agents $\intesize = 3$ is enough for each of them to learn their $i-$th preferred firm with constant regret using the $\EAP$ algorithm \ref{alg:eap}. This can provide a learner $a$ with the ability to learn their sorted sequence of firms regarding their $u_a(f)$s. 
\begin{lemma} \label{lemma:EAP}
    Given time step $t \geq m^2$, $\sum_{f \in U_a} Z_{a,f}(t)$ under $\EAP$ is at most $\sum_{s>t} 9 m e^{-c \Delta_{\min} \frac{s}{m}}$.
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:etc}]
    \label{proof:etc}
    Throughout this proof we denote $t=\frac{mk}{\intesize}$ as a shorthand. In order for the ranking $\vec{O}_a(t)$ to not be valid there must exist a pair of arms $f,f'$ such that $u_a(f)>u_a(f')$, but $\hat{u}_{a,f}(t)<\hat{u}_{a,f'}(t)$. This can happen only when $\hat{u}_{a, f}(t) \geq \hat{u}_{a, f'}(t)$. The probability of this event is equal to
    
    {\footnotesize
    \begin{align*}
     \Pr(\hat{u}_{a, f}(t) \geq \hat{u}_{a, f'(t)}(t))&=\Pr(\hat{u}_{a, f'(t)}(t)-u_a(f')-\hat{u}_{a, f}(t)+u_a(f) \leq u_a(f)-u_a(f')\\
     &\leq \mathbb{P}(\hat{u}_{a, f'_a(t)}-u_a(f^*_a)-\hat{u}_{a, f}(t)+u_a(f) \leq \Delta_{a}^\text{min})
    \end{align*}
    }
    
    
    Since each agent interviews each firm exactly $k$ times during the exploration stage and since the rewards from each firm are 1-sub-Gassian, we know that $\widehat{u}_{a, f^{\prime}}(t)-u_a\left(f^{\prime}\right)-\widehat{u}_{a, f}(t)+u_a(f)$ is $\sqrt{2 / k}$-sub-Gaussian. Therefore,
    $$
    \mathbb{P}\left(\widehat{u}_{a, f}(t) \geq \widehat{u}_{a, f^*_a(t)}\right) \leq e^{-\frac{k \Delta_a^2}{4}}
    $$
    The conclusion follows by a union bound over all possible firms $f$.
\end{proof}



\begin{proof}[Proof of Lemma \ref{lemma:etcreg}]
Setting $k=\max \left\{1, \frac{4}{\Delta_{a}^{\text{min}^2}} \log \left(1+\frac{T \Delta_{a}^{\text{min}^2}n}{4}\right)\right\}$ would provide us sub-linear regret.
if $k=1$, then we would have $T \leq \frac{4 \exp \left(\frac{\Delta_{a}^{\text{min}^2}}{4}\right)-1}{n}$ ad it means that $I$ is smaller than a constant. So
$$
R_{a}(T) \leq T \leq O(1)
$$
otherwise, we can replace $K$ in the Regret bound and write

{
\footnotesize
$$
\begin{aligned}
R_{a}(T) & \leq k \sum_{t=1}^{\frac{m}{\intesize}} \Delta_{a, f_{a}(t)}+\left(T-k \frac{m}{\intesize}\right) \Delta_{a}^\text{max} \frac{mn}{\intesize} \exp \left(-\frac{k \Delta_{a}^{\text{min}^2}}{4}\right), \\
& \leq \frac{4}{\Delta_{a}^{\text{min}^2}} \ln \left(1+\frac{T \Delta_{a}^{\text{min}^2}n}{4}\right) \frac{m}{\intesize}+\left(T-\frac{4m}{\Delta_{a}^{\text{min}^2} \intesize} \ln \left(1+\frac{T \Delta_{a}^{\text{min}^2}n}{4}\right)\right) \frac{mn}{\intesize} \frac{4}{4+T \Delta_{a}^{\text{min}^2}n}, \\
& \leq \frac{4}{\Delta_{a}^{\text{min}^2}} \ln \left(1+\frac{T \Delta_{a}^{\text{min}^2}n}{4}\right) \frac{m}{\intesize}+\frac{4mn}{\intesize}.
\end{aligned}
$$
}
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:eap-regret}]
    To prove the Theorem \ref{thm:eap-regret}, we first bound the total number of times that an arm $f\in U_a$ whose $\UCB'$ index is less than that of some arm $f'\in L_a$. At every of such moments, there is an arm $u'\in U_a$ whose index in the sorted $\UCB'$ list lies in $[i,m]$. The underlying reason is that if all $f' \in L_a$ lie in one of those indices, there would be no such pair like $f$ and $f'$. In Lemma~\ref{lemma:EAP}, we prove that the total number of those moments is at most $\sum_{s=m^2}^{T} 9 m e^{-c \Delta_{\min} \frac{s}{m}}$. Thus the aggregated regret for those moments is at most $$\sum_{s=m^2}^{T} 9 m^2 \Delta^{\max} e^{-c \Delta^{\min} \frac{s}{m}} \leq O(m^2).$$
    In the other moments, the algorithm has 
    either an arm $f \in U_a$ in the indices between $\left[i,m\right]$ of the sorted $\UCB'$ list which provides zero regret for the algorithm (including the cases in which some $f$ lies in the indices $i$ or $(i+1)$ or the $i$th and $(i+1)$ indices contain some arm $f'$ that has its $\alpha \leq \frac{1}{2}$)
    or all arms $f' \in L_a$ occupy all $\left[i,m\right]$ indices. There
    % all indices $\left[i,m\right]$ contain arms $l \in L_a$.
    in the former the regret is 0; however in the latter cases the total amount of regret is bounded by a constant multiplied by the regret of running \textit{All Probe} algorithm over the arm set equal to $L_a$. Thus, the total regret of those moments is also bounded by $O(m^2)$ which is induced directly form the result in \cite{bhaskara2022online}. 
\end{proof}


\begin{theorem} \label{Aud:thr}
    For any time $t \geq 1$, the following tail bounds hold:
    \begin{enumerate}
        \item For $q \geq \frac{1}{18}$, we have: $\operatorname{Pr}\left[\abs{\hat{\mu}_{a,f}(t) - \mu_i} > q \sigma_i^2\right] \leq 3 e^{-\frac{q \sigma_{a,f}^2 T_{a,f}(t)}{23}}$.
        \item For $q \geq \frac{1}{18}$, we have: $\operatorname{Pr}\left[\hat{\sigma}^2_{a,f}(t) > (1+q) \sigma_i^2\right] \leq 3 e^{-\frac{q \sigma_{a,f}^2 T_{a,f}(t)}{23}}$.
        \item $\operatorname{Pr}\left[\hat{\sigma}^2_{a,f}(t) < 0.65 \sigma_i^2\right] \leq 3 e^{-0.01 \sigma_{a,f}^2 T_{a,f}(t)}$.
    \end{enumerate}
\end{theorem}


\begin{proof}[Proof of Lemma \ref{lemma:EAP}]
    The key point to the proof is that, whenever an arm $f\in U_a$ appears in indices $[i:m]$, another arm $f' \in L_a$ has to be located in $[1: i-1]$ indices. Thus we define an event $ S_{a,f,f'}(t) \coloneqq  \1{\UCB'_{a,f'}(t) > \UCB'_{a,f}(t)}$, which means that having arm $f'$ appear in lower index than $f$. Notice, for any \(f' \in L_a\) \[
    Z_{a,f}(T) = \sum_{t=1}^T S_{a,f,f'}(t).
    \]
    Now for a such $f,f'$ we try to bound 
    $$
    \Pr\left(\sum_{f \in U_a, f' \in L_a} S_{a,f,f'}(t) \geq 1\right).
    $$
    We can write
    \begin{align}
        \Pr\left(\sum_{f \in U_a} S_{a,f,f'}(t) \geq 1\right) &\overset{(a)}\leq \mathbb{E}[\sum_{f \in U_a} S_{a,f,f'}(t)]
        \label{eq:markov}
        \\
        &= \sum_{f \in U_a} \mathbb{E}[S_{a,f,f'}(t)]\label{eq:linearity}\\
        &= \sum_{f \in U_a} \Pr(S_{a,f,f'}(t) = 1)\\
        &= \sum_{f \in U_a} \Pr(\UCB'_{a,f'}(t) > \UCB'_{a,f}(t))\label{mpr:lemma},
    \end{align}
    where the inequality~\eqref{eq:markov} directly comes from the Markov inequality, and linearity of expectation is applied in~\eqref{eq:linearity}.

    Having \eqref{mpr:lemma}, we will bound the probability of the event $(\UCB'_{a,f'}(t) > \UCB'_{a,f}(t))$.

In this regard, we can write (for simplicity we omit $t$ and $a$ from the arithmetics):
   \begin{align}
        \Pr\left(\UCB'_{f'} > \UCB'_{f}\right) &= \Pr(\hat{u}_{f'}+ \epsilon\hat{\sigma}^2_{f'} > \hat{u}_{f} + \epsilon\hat{\sigma}^2_{f})\\
         &=  \Pr(\hat{u}_{f'} + \epsilon\hat{\sigma}^2_{f'} + \Delta_{f,f'} > \hat{u}_{f} + \epsilon\hat{\sigma}^2_{u}+\Delta_{f,f'})\\
         &= \Pr(\hat{u}_{f'}-u_{f'}+\epsilon\hat{\sigma}^2_{f'} + u_{u} - \hat{u}_{f} - \epsilon\hat{\sigma}^2_{f} > \Delta_{f,f'})\\
         &\overset{(a)}\leq \Pr\left(\hat{u}_{f'}+\epsilon\hat{\sigma}^2_{f'}>u_{f'} +\frac{\Delta_{f,f'}}{2}\right) + \Pr\left(u_{f} - \hat{u}_{f} - \epsilon\hat{\sigma}^2_{f}>\frac{\Delta_{f,f'}}{2}\right)\\
         &=  \Pr\left(\hat{u}_{f'}+\epsilon\hat{\sigma}^2_{f'}>u_{f'} +\frac{\Delta_{f,f'}}{2}\right) + \Pr\left(\hat{u}_f+\epsilon\hat{\sigma}^2_f<u_{f'}+\frac{\Delta_{f,f'}}{2}\right) \label{zlem:pr},
    \end{align}
    Defining $\alpha$ and $\beta$ such that $\Delta_{f,f'} = \alpha\sigma^2_{f'} = \beta \sigma^2_f$, we consider three different cases for $\alpha$ and $\beta$ to bound the \eqref{zlem:pr}. 
\begin{case}
    $\alpha,\beta \geq \frac{1}{2}$. 
 
    By Theorem \ref{Aud:thr} we would have 
    \[\Pr\left(\hat{\sigma}^2_{f'} \geq \left(1+\frac{69}{100}\right)\sigma^2_{f'}\right) \leq 3e^{-0.06\Delta_{f,f'}\frac{t}{n}}. \]
    
 Thus, we can be sure that $\hat{\sigma}^2_{f'} \leq (1+\frac{69}{100})\sigma^2_{f'}$ holds with a probability close to 1. Now we write 
    \begin{align*}
       \Pr\left(\hat{u}_{f'}+\epsilon\hat{\sigma}^2_{f'}>u_{f'} +\frac{\Delta_{f,f'}}{2}\right) &= \Pr\left(\hat{u}_f' - u_f' > \frac{\alpha\sigma^2_{f'}}{2} - \epsilon\hat{\sigma}^2_{f'}\right)\\
       &\overset{(a)}= \Pr\left(\hat{u}_{f'} - u_{f'} > (\frac{\alpha}{2}-1.69\epsilon)\sigma^2_{f'}\right)\\
       &\leq \Pr\left(\hat{u}_{f'} - u_{f'} > 0.16\sigma^2_{f'}\right)\\
       &\leq 3e^{-0.0025\Delta_{f,f'}\frac{t}{n}} \label{hatmu:c1},
    \end{align*}
In (a) we used $\epsilon=0.1$.
Analogously, we use the same approach to prove

\[\Pr\left(\hat{u}_u+\epsilon\hat{\sigma}^2_u<u_f'+\frac{\Delta_{f,f'}}{2}\right) \leq 3e^{-0.0025\Delta_{f,f'}\frac{t}{n}}.\]
\end{case}

\begin{case}
    $\alpha \geq \frac{1}{2}, \beta \leq \frac{1}{2}$

    In this case we can bound the probability of $\hat{u}_{f'}+\epsilon\hat{\sigma}^2_{f'}>u_{f'} +\frac{\Delta_{f,f'}}{2}$ with the same technique we used Case 1. So we know
    \[\Pr\left(\hat{u}_{f'}+\epsilon\hat{\sigma}^2_{f'}>u_{f'} +\frac{\Delta_{f,f'}}{2}\right)\leq 3e^{-0.0025\Delta_{f,f'}\frac{t}{n}},\]

    For the second part we can demonstrate that
    \begin{align*}
        \Pr\left(\hat{u}_u+\epsilon\hat{\sigma}^2_u<u_{f'}+\frac{\Delta_{f,f'}}{2}\right) &\leq \Pr\left(\hat{u}_u+\epsilon\hat{\sigma}^2_u<u_u\right)\\
    &\leq\Pr\left(u_u-\hat{u}_u > \epsilon\sigma^2_u\right)\\
    &\overset{(a)}\leq\Pr\left(u_u-\hat{u}_u > 0.065 \sigma^2_u \right)\\
    &\overset{(b)}\leq 3 e^{-0.0025\Delta_{f,f'}\frac{t}{n}}.
    \end{align*}
    where both (a) and (b) are directly derived from the theorem \ref{Aud:thr}.
\end{case}
\begin{case}
    $\alpha < \frac{1}{2}$
    
    Based on the proofs for Cases 1 and 2, at time step $t$, for any arm $f''$ which is located in the indices between $f$ and $f'$ ,$\UCB'_{f''} > \UCB'_f$, one of these conditions holds with high probability:
    \begin{enumerate}
        \item $f'' \in U_a$
        \item $f'' \in L_a \text{ s.t. }\Delta_{f,f''}<\frac{1}{2}\hat{\sigma}^2_{f''}$ 
        
    \end{enumerate}
    Now we can prove that for either cases the instant regret would be zero. 
    Assume that $f_1$ and $f_2$ are the arms located on indices $i$-th and $i+1$-th respectively. (w.l.o.g we assume that $u_{f_1} \leq u_{f_2}$)
    \begin{itemize}
        \item If either $f_1\in U_a$ or $f_2 \in U_a$, then we can write:
    \begin{align*}
        \mathbb{E}\left[\max\{X_{f_1},X_{f_2}\}\right] &\geq \max\{u_{f_1},u_{f_2}\}\\
        &\geq u_{a,f^i_a}
    \end{align*}
    which induces a zero instant regret.
    \item Otherwise $f_1$ satisfies condition 2. Therefore we would have
    \begin{align*}
         \mathbb{E}\left[\max\{X_{f_1},X_{f_2}\}\right]&\overset{(a)}\geq u_{f_1} + \frac{\sigma^2_{f_1}}{2}\\
         &\overset{(b)}>u_{f_1}+\Delta_{u,f_1}\\
         &\geq u_{a,f^i_a}
    \end{align*}
    where (a) holds because the Reverse Prophets Inequality proven by Bhaskara \etal \cite{bhaskara2022online}, and the inequality (b) is condition 2's constraint.

    In this case, the instant regret would also be zero.
    \end{itemize}
    
\end{case}

\end{proof}

==> Discussions.tex <==
\section{Extended Introduction} \label{appx:discussion}


\subsection{Related Works}


\subsection{Remarks}
\paragraph{Regret Bound Evaluation Criteria.}
To evaluate the cost of decentralizing $\FGS$, we compare the regret of our decentralized algorithms with the optimal centralized bound $O(nm^2)$ from \cref{prop:ciarr}. We call a decentralized algorithm \emph{ideal} if its regret exceeds the centralized optimum by at most an $O(n^2)$ factor, which corresponds to the worst-case number of rounds needed for a distributed execution of $\FGS$. In more structured markets, distributed $\FGS$ may complete much faster (for example, in $O(n)$ rounds in $\alpha$-reducible instances), which motivates an \emph{adaptively ideal} notion in which the regret scales only with the actual distributed $\FGS$ runtime of the underlying market. \amcomment{maybe move it to remark after theorem statements}

==> ICML/intro-v4.tex <==
\section{Introduction}\label{sec:intro}

Two-sided matching markets~\citep{roth1992two} provide a foundational model for labor markets~\citep{roth1984evolution}, school choice~\citep{abdulkadirouglu2003school}, and online platforms~\citep{hitsch2010matching}. A market comprises two sides (e.g., \(n\) agents and \(m\) firms), each with preferences over the other side. A matching is \emph{stable} if no agent--firm pair would both prefer to deviate from their current assignments~\citep{gale1962college}. 
In many markets, preferences are \emph{not known a priori}: participants learn them through interaction, and any given participant can only evaluate a small fraction of potential partners. This motivates \emph{bandit learning} in matching markets~\citep{liu2020competing,maheshwari2022decentralized,liu2021bandit,kong2023player,ghosh2024competing}, where agents repeatedly apply to firms, observe outcomes, and aim to learn a stable matching while minimizing regret. Most existing work assumes (i) only agents are uncertain and (ii) firms follow fixed, known preferences and always hire among applicants. These assumptions simplify decentralized dynamics, but do not capture the following two pervasive features of real markets.
% \textbf{pre-matching interviews} and \textbf{firm-side uncertainty}.

% \hbcomment{minor comment: the last sentence of last paragraph and paragraph title of next paragraph are somewhat repetitive. is there a better solution?}
% \mo{I am commenting out the above comment: the last paragraph sets the stage and then the next two expands on them. }

\noindent\textbf{Two missing ingredients: interviews and uncertain firms.}
First, \amedit{we introduce a model,} where participants engage in low-cost preliminary interactions (interviews, \amedit{internships}, visits) before submitting final applications. Such interactions produce \emph{\amedit{pre-application} noisy side-observations} of match quality that can accelerate learning. This resembles \emph{bandits with hints}~\citep{bhaskara2022online,mirfakhar2025heterogeneous} and, more broadly, \emph{algorithms with predictions}~\citep{lykouris2021competitive}. \amedit{However, unlike prior hinted models, which focus on single-agent settings, interviews in our multi-agent market simultaneously \emph{reveal information} and \emph{restrict feasible actions}, since an agent may apply only to an interviewed firm~\citep{lee2017interviewing,beyhaghi2021randomness}. As a result, pre-matching hints come at a substantial cost of shrinked action sets and thus intensified competition.}

 % However, interviews create a key structural constraint absent from existing hinted-bandit models: they simultaneously \emph{reveal information} and \emph{restrict feasible actions}, since an agent may apply only to an interviewed firm~\citep{lee2017interviewing,beyhaghi2021randomness}.

Second, firms may also be uncertain about their preferences (i.e., their rankings must be learned). Early misrankings can cause firms to reject strong candidates, slowing convergence to stability and increasing regret. To model how firms hedge against uncertainty in practice, we allow a firm to \emph{defer} hiring in a round (remain vacant) rather than commit to an applicant it currently deems suboptimal. We emphasize that this is a \emph{modeled action option} (not a game-theoretic manipulation) \amedit{that offers a modular extension of prior models to handle uncertainty on the firm side}: it expands the firm action space in a way that can stabilize \emph{decentralized \amedit{two-sided} learning} dynamics and is consistent with evidence that firm-side hiring deferrals can shape stable outcomes in static/non-learning settings~\citep{kupfer2018influence}.

\noindent\textbf{Model at a glance.}
We study two-sided bandit learning with interviews and uncertainty on \emph{both} sides. In  round \(t\), every agent \(a\) selects \(k\) firms to interview. Each interviewed pair \((a,f)\) yields stochastic, noisy feedback to \emph{both} sides with unknown means \(\mu_{a,f}\) and \(\mu_{f,a}\), representing their expected utilities from matching with each other. After interviewing, each agent applies to one of its interviewed firms; a firm may accept its most-preferred applicant \emph{or defer} and remain vacant. When a match occurs, both sides receive stochastic rewards drawn from the corresponding distributions.

We evaluate performance via \emph{agent regret}: the gap between the expected reward of the agent's stable match and the agent's accrued reward over \(T\) rounds. We study both a \emph{centralized} setting with an interview allocator and \emph{decentralized} settings without it. A central challenge in decentralization is the information revealed to agents: we restrict attention to \emph{minimal public firm-side signals} revealed to all agents\textemdash either \emph{vacancy-only} feedback (whether a firm filled its position) or \emph{anonymous hiring-change} feedback (whether a firm's hire changed), without identities. As shown in Appendix~\ref{sec:decwithvf}, such coarse firm-side signal is necessary for decentralized algorithms especially in unstructured markets.

\noindent\textbf{A guiding question.}
Existing bandit-matching work without interviews typically yields regret that scales at least logarithmically with the horizon, often \(O(\log T)\), even under stronger observability assumptions~\citep{liu2020competing,maheshwari2022decentralized,liu2021bandit}. Interviews add side-observations before committing to an application, suggesting that learning could be dramatically faster. This leads to our central question:
\emph{Can a market leverage a small number of interviews per round to learn a stable matching with \textbf{horizon (time)-independent} regret, in a decentralized manner with only \textbf{anonymous} firm-side signals, even when firms themselves are uncertain and may defer hiring?}
Answering this question requires addressing two challenges.
% \noindent\textbf{Technical challenges.}


% Designing dynamics that are both stable and low-regret under such non-identifying feedback is nontrivial.
\noindent$\blacktriangleright$ \textit{Uncertain firms and controlled deferral:}
When firms learn their rankings, early misrankings can induce rejections of strong applicants, creating feedback loops that redirect agents and slow convergence. Allowing firms to defer can mitigate premature commitments, but it must be carefully controlled: deferral should not itself become a source of regret, and it must support convergence to stable outcomes.


\amedit{\noindent$\blacktriangleright$ \textit{Interviews as hints under competition and stability.}
Interviews provide side-observations but also constrain actions: agents may apply only to interviewed firms. This differs from single-agent hints~\cite{bhaskara2023bandit} and related extensions~\cite{wei2020taking,mirfakhar2025heterogeneous}, where rewards are always attainable. Here, restricting actions to interviewed sets intensifies competition, so agents may remain unmatched regardless of how informative their interviews are. Rewards depend on both sides' uncertain preferences, firms may strategically defer, and decentralized agents observe only vacancy or anonymous hiring-changes rather than match identities or firm's preferences, making stability substantially harder to maintain. We also note that~\cite{liu2021bandit}, they assumed this signals to contain the identites of the match and the assumption of the certain firms' fixed preferences are also known to the agents.}

% \hbcomment{We sometimes use $O(1)$ and $O(\log T)$ and drop other terms and sometimes use $O(f(n,m))$. Is this ok, or should we be consistent?}
% \mo{I am commenting out the above comment: I am fine with the current versions in the early part of contributions, we say high-level only horizon-independent matters, then in detailed contributions we say explicit regret.}
% \begin{table*}[t]
%     \centering
    
%     \begin{tabularx}{0.80\textwidth}{ccccc}

%         \toprule
%         Algorithm                       & D/C & Regret                 & Queried Hints                  & Communication           \\
%         \toprule
%         $\HCLA$ (Algorithm~\ref{routin:hcla})      & C   & $O\left(MK^{2M}\right)$   & $O\left(MK^M \log T\right)$    & N/A                            \\
%         \toprule
%         $\GHCLA$ (Algorithm~\ref{routin:hcla2})      & C   & $O\left(M^4K\right)$   & $O\left(M^2K \log T\right)$    & N/A                            \\

%         \midrule
%         $\GPHCLA$ (Algorithm~\ref{routin:hcla1})    & C   & $O\left(M^4K\right)$   & $O\left(MK \log T\right)$      & N/A                            \\
%         \midrule
%         $\HDETC$ (Algorithm~\ref{routin:hdetc})$^\dagger$     & D   & $O\left(M^3K^2\right)$ & $O\left(M^3K \log (MT)\right)$ & $O\left(\log T\right)$             \\
%         \midrule
%         $\EBHDETC$ (Algorithm~\ref{routin:ebhdetc}) & D   & $O\left(M^3K^2\right)$ & $O\left(M^3K \log (MT)\right)$ & $O\left(\log T\right)$           \\
%         \bottomrule
%     \end{tabularx}
%     \caption{Regret, Queried Hints, and Communication Bounds for Centralized and Decentralized Algorithms (
%     `C' and `D' stand for centralized and decentralized algorithms respectively, 
%     $^\dagger$ indicates that \HDETC{} relies on the knowledge of minimum gap)}
%     \label{demo-table}
% \end{table*}

\begin{table}[t]
\caption{Regret Bounds. $(*)$ denotes centralized, $(\dagger)$ coordinated decentralized, and $(\ddagger)$ coordination-free decentralized. In all decentralized variants, firms follow strategic rejection (\cref{alg:fdrr}).}
\label{sample-table}
\centering
\small
\begin{tabular}{@{} l l l l @{}}
\toprule
Algorithm & Market & Feedback & Regret \\
\midrule
$\cref{alg:ciarr}^{*}$ & General & N/A & $O(nm^2)$ \\
$\cref{alg:drr}^{\dagger}$ & $\alpha$-reducible & $\VF$ & $O(n^3m^2)$ \\
$\cref{alg:drr}^{\dagger}$ & General & $\VF$ & $O(n^4m^2)$ \\
$\cref{alg:ancdrr}^{\ddagger}$ & $\alpha$-reducible & $\VFP$ & $O(n^3m^2)$ \\
$\cref{alg:Eancdrr}^{\ddagger}$ & General & $\VFP$ & $O\!\left(\epsilon^{-1} n^5 m^4\right)$ \\
\bottomrule
\end{tabular}
\end{table}


\noindent\textbf{Contributions.}
We introduce a two-sided bandit model with interviews and uncertain firms, and show that interviews enable \(O(1)\) (\emph{horizon-independent}) learning regret for stable matchings in both centralized and decentralized markets, with explicit near-optimal dependence on market parameters.

\amedit{\noindent$\blacktriangleright$ \textit{Modeling uncertain firms with a deferral option.}
We model firm-side uncertainty and introduce deferral as a modular primitive for two-sided learning (\autoref{sec:model}), extending firms' action space with the option to remain vacant (as shown by~\cref{examp:introstrategic}). This yields \emph{strategic} firms and can be plugged into prior works' models to relax the restrictive assumption of fixed, known firm preferences. We then design a strategic rejection/deferral policy (\cref{alg:fdrr}) that limits harmful deferrals while enabling stable learning dynamics.





\noindent$\blacktriangleright$ \textit{Two interviews per round suffice for horizon-independent regret.}
We formalize interviews as bandit hints in a two-sided market and show that \emph{two interviews per round}, using only empirical means as estimators to form estimated preference lists, suffice for horizon-independent regret in our main settings (\cref{thm:ciarr}). In the single-agent case, this resolves and strengthens the conjecture of~\cite{bhaskara2023bandit}, which proved sufficiency of three hints using UCB-V but left empirical means open and conjectured three hints were necessary. We then extend this guarantee to a two-sided stability learning with uncertain firms and strategic deferral.}


\noindent$\blacktriangleright$ \textit{Centralized allocation: learning the agent-optimal stable matching.}
In the centralized setting (\autoref{sec:centralized}), we design a central interview allocator (\texttt{CIA}) that coordinates interviews and applications. Building on deferred acceptance~\citep{gale1962college}, we give an algorithm that learns the agent-optimal stable matching in \(O(nm^2)\) time under both certain and uncertain firms (\cref{thm:ciarr}).

\noindent$\blacktriangleright$ \textit{Decentralized learning.}
We present two decentralized algorithms under minimal anonymous feedback. Under vacancy-only feedback \(\VF\) (\cref{sec:decwithvf}), we provide a coordinated algorithm (\cref{alg:drr}), achieving \(O(n^3m^2)\) regret in structured markets (\cref{thm:alphadecreg}) and \(O(n^4m^2)\) regret in general markets (\cref{thm:decreg}). Under anonymous hiring-change feedback \(\VFP\) (\cref{sec:non-coop}), we design a coordination-free algorithm (\cref{alg:ancdrr}), achieving \(O(n^3m^2)\) regret in structured markets (\cref{thm:noncoalphadecreg}). Extending the coordination-free approach to general markets (\cref{sec:noncoopgen}) requires three interviews per round and mild assumptions, yielding \(O(1)\) regret (\cref{thm:noncogendecreg}).


% The exponentially large factor $\epsilon^{-1}$ reflects the need to rule out blocking-pair resolution cycles that may arise in general markets under coordination-free dynamics; such cycles do not occur in $\alpha$-reducible markets. Similar large constants also appear in the $O(\log T)$ bounds of~\cite{liu2021bandit}, albeit under more informative feedback than our $\VFP$.


% \paragraph{Technical Contributions.}
% \textcolor{orange}{Our contributions can be viewed in several layers. First, we resolve a single-agent open question raised by~\cite{bhaskara2023bandit} in the queried-hints model: time-independent $O(1)$ regret is achievable with only two queried observations per round using empirical-mean estimates. Second, we lift this idea to learning in competitive two-sided matching markets by modeling interviews as pre-application information. In this setting, interviews are not merely informative hints or free observations: they also restrict feasible actions, intensify competition among agents, and interact with firm-side preferences. Thus, unlike the single-agent case where querying the top estimated arms suffices, interview sets must be chosen carefully because pre-application information does not by itself guarantee reward.Finally, we introduce strategic deferral as a modeling primitive for firm-side uncertainty. Since interviews provide two-sided information in practice, we relax the standard assumption that firm preferences are fixed and known a priori. Instead, uncertain firms may defer hiring to avoid committing to potentially suboptimal matches. This makes learning harder: even after an agent carefully interviews and applies to a firm, the firm may strategically remain vacant. Nevertheless, this primitive enables two-sided learning and coordination-free dynamics, and provides a modular way to extend prior matching-learning models beyond the certain-firm setting. Building on these ideas, we design centralized and decentralized algorithms with time-independent regret, improving over prior $O(\log T)$ guarantees at the cost of polynomial factors in the number of agents and firms. Our centralized bound is within a factor $m$ of the optimal time-independent benchmark, and we conjecture it to be asymptotically tight. The decentralized guarantees then quantify the additional cost of decentralization under different feedback models, with further optimality discussion deferred to the appendix.}

==> NO_FSF.tex <==
\subsection{Definition of Convergence}

\begin{definition}[Convergence of a Learning Algorithm]\label{def:convergence}
A learning algorithm $\pi$ is said to \emph{converge} to a perfect matching $(a,\FM_a(t))_{a \in \AG}$ if there exists a time step $t \in [T]$ such that for all $t' \ge t$, we have $\FM_a(t') = \FM_a(t)$ and $\FM_a(t') \neq \emptyset$ for every agent $a \in \AG$.
\end{definition}

\subsection{Necessity of Adding Firm-Side Feedback ($\VF(t)$ and $\VFP(t)$)} \label{Sec:justig}
We now describe how a fully decentralized algorithm without signaling should operate. In the signaling-based approach, coordination among all agents was required whenever a re-run of \( \FGS \) was initiated by some agent. A natural starting point for removing signaling is to employ the triggering condition defined earlier, which was originally used to decide when to send the re-run signal based solely on individual observations from round-robin interviews, independent of other agents’ actions. However, our previous regret analysis relied heavily on the \( f'_a(t) \), which formed a matching as the output of \( \FGS \). In a fully decentralized setting, agents must instead respond to changes caused by events in \( \mathcal{S}_a \) detected by other agents, updating their interviewing sets so that the resulting allocation remains not only a matching but also stable with respect to the current estimations. This dependency makes a direct extension of Algorithm~\ref{alg:drr} unsuitable in its current form. 

We highlight two main challenges in adhering to the previous model while attempting to design fully decentralized algorithms. Through clarifying examples and impossibility lemmas, we show that the original framework is too restrictive; consequently, we refine the model to make it compatible with the design of fully decentralized algorithms that achieve time-independent regret.


By the following example, 
% which mirrors the setup of Example~\ref{examp:drrs}, 
we illustrate why the condition defined in \( \mathcal{S}_a \) may not, by itself, be sufficient in the case of fully decentralized learning with non-collaborative agents. In particular, such a condition can lead to linear regret for some agents, even in the presence of round-robin interviews. This observation provides a plausible motivation to refine the model accordingly.


\begin{example}\label{examp:fdrrs}
    Let \( \mathcal{A} = \{a_1, a_2, a_3\} \) and \( \mathcal{F} = \{f_1, f_2, f_3\} \), with true preferences:
    \[
    \begin{array}{lr}
    \PL_{a_1}: \langle f_1 \succ f_2 \succ f_3\rangle &  \PL_{f_1}: \langle a_1 \succ a_2 \succ a_3\rangle \\
    \PL_{a_2}: \langle f_2 \succ f_3 \succ f_1\rangle & \PL_{f_2}: \langle a_1 \succ a_2 \succ a_3\rangle \\
    \PL_{a_3}: \langle f_3 \succ f_1 \succ f_2\rangle & \PL_{f_3}: \langle a_1 \succ a_2 \succ a_3\rangle
    \end{array}
    \]
    The unique stable matching under these preferences is \((a_1,f_1), (a_2,f_2), (a_3,f_3)\).

    Consider a time step \( t \) immediately after a run of \( \FGS \), where the estimated preference lists are:
    \[
    \begin{array}{lr}
    \EPL_{a_1}(t): \langle f_2 \succ f_1 \succ f_3\rangle & I_{a_1} = \{f_2, \RR_{a_1}\} \\
    \EPL_{a_2}(t): \langle f_2 \succ f_3 \succ f_1\rangle & I_{a_2} = \{f_3, \RR_{a_2}\} \\
    \EPL_{a_3}(t): \langle f_3 \succ f_1 \succ f_2\rangle & I_{a_3} = \{f_1, \RR_{a_3}\}
    \end{array}
    \]
    Here, agent \( a_1 \) is the only one whose estimated preference list is incorrect. Agents \( a_2 \) and \( a_3 \) have already learned their true lists, which remain valid thereafter. Consequently, \( t > \sup \{\mathcal{S}_{a_2}\} \) and \( t > \sup \{\mathcal{S}_{a_3}\} \), implying that neither \( a_2 \) nor \( a_3 \) will detect a triggering event to change their interview sets.

    Agent \( a_1 \), however, is expected to maintain a valid \( \EPL_{a_1} \) most of the time. Eventually, at some time step \( t' \), its list will correctly place \( f_1 \) at the top:
    \[
    \EPL_{a_1}(t') : \langle f_1 \succ f_2 \succ f_3\rangle.
    \]
    Following our decentralized approach, agent \( a_1 \) updates their interview set to:
    \[
    I_{a_1} = \{f_1, \RR_{a_1}\}.
    \]
    This change blocks agent \( a_3 \) from interviewing with \( f_1 \), prompting \( a_3 \) to re-evaluate \( \EPL_{a_3}(t) \) and update their interview set to:
    \[
    I_{a_3} = \{f_2, \RR_{a_3}\}.
    \]
    This, in turn, leaves agent \( a_2 \) continuing with:
    \[
    I_{a_2} = \{f_3, \RR_{a_2}\},
    \]
    which remains unchanged due to \( a_2 \)'s already correct preference list. However, since \( f_3 \) is suboptimal for \( a_2 \), this choice can persist until the end of the game, potentially leading to linear regret for \( a_2 \).
\end{example}

% We then employ this illustrative example to prove the following impossibility lemma which eliminates the possibility of designing a fully-decentralized algorithm that achieves time-independent regret.
% \begin{lemma}\label{lem:fdrr-impossible}
% With respect to the notion of decentralization introduced in Definition~\ref{def:decentralized}, no deterministic decentralized learning algorithm without firm-side feedback can achieve time-independent regret.
% \end{lemma}

% \begin{proof}
% Assume, for contradiction, that there exists a profile of learning policies 
% \(\Pi = (\pi_i)_{i \in \mathcal{A}}\), where each \(\pi_i\) is a deterministic fully-decentralized learning policy for agent \(i\), that guarantees time-independent regret. Consider the globally-ranked instance described in Example~\ref{examp:fdrrs}. In this instance, agent \(a_1\) is the most preferred agent for all firms. Consequently, all changes in \(I_{a_1}\) are driven solely by updates to \(\EPL_{a_1}\), since no other agent can ever block \(a_1\).

% Now, recall the trapping event from Example~\ref{examp:fdrrs}, where agent \(a_2\) has already learned its true preference list and thus observes no further changes in \(\EPL_{a_2}\). Under this event, if agent \(a_2\) becomes stuck with the interviewing set \(I_{a_2} = \{f_3, \RR_{a_2}\}\), achieving time-independent regret would require that agent \(a_1\) places \(f_3\) in its interviewing set, thereby blocking \(a_2\) and forcing it to eventually move to \(f_2\). This would then lead the market toward the optimal matching.

% However, \(a_1\) cannot distinguish between different problem instances, since it is never blocked and its updates depend solely on its own preference list. To see this, construct a new instance identical to Example~\ref{examp:fdrrs} from the perspective of \(a_1\), but with valuations adjusted so that the bad event occurs immediately after the last time step when \(f_3 \in I_{a_1}\). From this point onward, \(a_2\) is never blocked by \(a_1\), and thus remains indefinitely stuck with \(f_3\).

% The only remaining possibility is for \(a_2\) to deterministically attempt \(f_2\) even when not blocked. But this strategy fails in instances where the trapping event occurs later, since \(\EPL_{a_2}\) will not change, and \(a_2\) cannot distinguish between the two cases. As a result, any deterministic fully-decentralized policy profile \(\Pi\) will inevitably cause some agent (here, \(a_2\)) to incur linear regret in at least one valid problem instance.

% Therefore, no deterministic fully-decentralized learning algorithm can guarantee time-independent regret.
% \end{proof}

% Through the following Example we also illustrate another crucial problems  illustrating a synchronization problem that may occur and put the whole market stuck inside a sub-optimal matching forever that would cause into linear regret for some agent which introduces another sufficient reason to tilt the model a bit to desing a fully-decentralized algorithm that achieves time independent regret.

==> Neurips26/checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

    \item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction clearly state the main claims of the paper, which are supported by the theoretical results and analyses presented in the subsequent sections. The claims are consistent with the contributions outlined in the paper, and any assumptions or limitations are also acknowledged.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
              \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers.
              \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings.
              \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
          \end{itemize}

    \item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper includes a discussion of the limitations in the conclusion and Appendix~\ref{sec:remarks3}.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper.
              \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
              \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
              \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
              \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
              \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
              \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
              \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
          \end{itemize}

    \item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides all necessary assumptions and complete proofs (in appendix) for the theoretical results.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper does not include theoretical results.
              \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
              \item All assumptions should be clearly stated or referenced in the statement of any theorems.
              \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition.
              \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
              \item Theorems and Lemmas that the proof relies upon should be properly referenced.
          \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper does not include experiments.
              \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
              \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable.
              \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
              \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
                    \begin{enumerate}
                        \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
                        \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
                        \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
                        \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
                    \end{enumerate}
          \end{itemize}


    \item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that paper does not include experiments requiring code.
              \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
              \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
              \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
              \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
              \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
              \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
              \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
          \end{itemize}


    \item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper does not include experiments.
              \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
              \item The full details can be provided either with the code, in appendix, or as supplemental material.
          \end{itemize}

    \item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 

    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper does not include experiments.
              \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
              \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
              \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
              \item The assumptions made should be given (e.g., Normally distributed errors).
              \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
              \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
              \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
              \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
          \end{itemize}

    \item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is mainly theoretical and does not include large-scale experiments.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper does not include experiments.
              \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
              \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute.
              \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper).
          \end{itemize}

    \item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in the paper adheres to the NeurIPS Code of Ethics.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
              \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
              \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
          \end{itemize}


    \item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is mainly theoretical and does not have direct societal impacts.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that there is no societal impact of the work performed.
              \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
              \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
              \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
              \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
              \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
          \end{itemize}

    \item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is mainly theoretical and does not pose such risks.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper poses no such risks.
              \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters.
              \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
              \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
          \end{itemize}

    \item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is mainly theoretical and does not use existing assets.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper does not use existing assets.
              \item The authors should cite the original paper that produced the code package or dataset.
              \item The authors should state which version of the asset is used and, if possible, include a URL.
              \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
              \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
              \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
              \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
              \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
          \end{itemize}

    \item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is mainly theoretical and does not release new assets.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper does not release new assets.
              \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
              \item The paper should discuss whether and how consent was obtained from people whose asset is used.
              \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
          \end{itemize}

    \item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is mainly theoretical and does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
              \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper.
              \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector.
          \end{itemize}

    \item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is mainly theoretical and does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
              \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.
              \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution.
              \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
          \end{itemize}

    \item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
          %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is mainly theoretical and does not involve LLMs usage beyond writing, editing, or formatting purposes.
    \item[] Guidelines:
          \begin{itemize}
              \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
              \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
          \end{itemize}

\end{enumerate}

==> RR.tex <==


\subsection{Degrees of Centralization in Interview Allocation}
Since the final application $\FA_a(t)$ of each agent $a$ must lie within its interviewing set $\INT_a(t)$, achieving time-independent regret in stable matching with interviews critically depends on how outreach $\RO_a(t)$—and hence $\INT_a(t)$—is determined, i.e., on the allocation of interviews. 
As justified earlier in the description of the model, we adopt the assumption $\RO_a(t)=\INT_a(t)$, which makes interview allocation equivalent to setting the outreach set $\RO_a(t)$. 
For both reward non-sensitive and reward-sensitive settings, we design algorithms that differ in their degree of centralization. In general, we classify interview allocation algorithms into three subclasses by their centralization: \emph{Centralized}, \emph{Decentralized with Cooperative Agents}, and \emph{Decentralized with Non-Cooperative Agents}.


\begin{itemize}
    \item \textbf{Centralized Algorithms.}  
    We assume an omniscient oracle, referred to as the \textbf{C}entral \textbf{I}nterview \textbf{A}llocator ($\CIAP$), which observes the estimated preference lists of all agents and specifies the interviewing sets $\INT_a(t)$ at each time step. With such centralized control, agents do not need to coordinate to avoid collisions, as all conflicts are resolved by $\CIAP$.

  \item \textbf{Decentralized with Cooperative Agents.}  
Agents determine their interviewing sets $\INT_a$ from local observations without a central oracle.  
Conflicts are not externally resolved, but agents may still cooperate via \emph{implicit signaling} in the system’s dynamics.  
To enable this, we assume that at the end of each round, all agents observe the set of unmatched firms $\VF(t)$.  

\item \textbf{Decentralized with Non-Cooperative Agents.}  
Agents act as independent utility-maximizers, relying only on their own observations and limited firm feedback. No coordination is permitted, making this the most restrictive setting.  

\xw{Reading the above paragraph, I think you want to say \emph{cooperative agents} can communicate through collision, 
\emph{non-cooperative} cannot utilize collision. But other than that, non-cooperative agents still follow the pre-assigned algorithm? 
Maybe you can explicitly name the later as ``communication-restricted'' agents?
Coordination is a very general term. Is executing the Gale-Shapley algorithm a coordination? Without the GS algorithm, how to find a stable match?}

\end{itemize}

We formalize our notion of decentralization in the following definition, which captures both decentralized-with-cooperative-agents and decentralized-with-non-cooperative-agents settings.

\begin{definition}[Decentralized Setup]\label{def:decentralized}
In the \emph{Decentralized} setup, each agent $a \in \AG$ updates its interviewing set $\INT_a(t)$ solely based on its own observations at time $t$, which consist of:
\begin{enumerate}
    \item its current estimated preference list $\EPL_a(t)$;
    \item whether the firm $\FA_a(t-1)$ that $a$ applied to and was matched with in the previous round (i.e., $\FA_a(t-1) = \FM_a(t-1)$) remains available as a match. For example, if $a$ is blocked by competitors, then $\FM_a(t) = \emptyset$ despite $\FA_a(t) = \FM_a(t-1)$;
    \item limited firm-side feedback: specifically, the set of unmatched firms at the end of each round.
\end{enumerate}
\end{definition}




% Within the decentralized class, we distinguish two regimes: \hbcomment{are these supposed to show up as bullet points?}
% - In the case of \emph{cooperative agents}, implicit communication through collisions or firm feedback may be used to coordinate.  
% - In the case of \emph{non-cooperative agents}, agents act independently as utility-maximizers, with no such coordination.








==> RS.tex <==
\section{Reward Sensitive Algorithms}
\input{ucb}

==> Rews.tex <==
\section{Reward non-Sensitive and Reward Sensitive Algorithms}
Based on the defined model, and assuming that agents are the applying side who make decisions and determine the outcome of the matching, the additional observations obtained during interviews can be viewed as \emph{hints} about the rewards of being matched with a firm, without requiring an actual match. These hints enable agents (and firms) to form more accurate beliefs and to make better-informed choices when selecting their interviewing set $\INT_a$ and ultimately the firm $\FA_a$ they apply to at each round. In the following, we present two approaches for leveraging these hints to substantially reduce regret to be time-independent.



The first class, which we call \emph{reward non-sensitive algorithms},
% \amcomment{We may want to revisit this terminology.} 
uses the information obtained from interviews, $X_{a,f}(t)$ for $f \in \INT_a(t)$, solely to refine utility estimates for future outreach decisions $\RO_a(t+1)$ and to predetermine the final application choice $\FA_a(t)$ before the realized rewards from interviews are revealed. 
In other words, the realized rewards do not affect the choice of $\FA_a(t)$. 
For instance, a naive strategy for agent $a$ is to always include in $\RO_a(t)$ the firm $f_t$ with the highest estimated utility $\hat{u}_{a,f_t}(t)$ (along with other firms) and then set $\FA_a(t) = f_t$, regardless of the realized rewards from other firms in $\INT_a(t)$. 
Suppose $f'_t \in \RO_a(t)$ is the second-best firm by estimated utility, with $\hat{u}_{a,f_t}(t) > \hat{u}_{a,f'_t}(t)$. 
Reward non-sensitive algorithms ignore the possibility that $f'_t$ could yield a higher instantaneous reward in that round, i.e., $X_{a,f'_t}(t) > X_{a,f_t}(t)$. 
 


In contrast, \emph{reward-sensitive algorithms} use estimated utilities only to determine the outreach and interview sets $\RO_a(t)$ and $\INT_a(t)$, but after interviewing, they also incorporate realized rewards when choosing the final application $\FA_a(t)$. 
For example, an agent may include the two top firms $f_t$ and $f'_t$ in $\RO_a(t)$, and after observing interview outcomes, select \(
\FA_a(t) = \argmax_{f \in \{f_t, f'_t\}} X_{a,f}(t).
\)
This approach can yield higher instantaneous rewards—and thus lower regret—provided the agent is admitted by the chosen firm.  

In single-agent settings, reward-sensitive algorithms are often expected to achieve lower regret than reward non-sensitive ones, as they adapt choices to realized rewards, though this need not hold in full generality. 
In competitive multi-agent markets, however, where each firm admits only one agent per round, they introduce new challenges: stochastic rewards may cause agents to deviate from their stable preferences, and simultaneous pursuit of high-reward firms increases the risk of collisions. 
These challenges make the design of reward-sensitive algorithms more delicate. 
In this work, we analyze both classes of algorithms and show that reward-sensitive policies can still achieve time-independent regret in structured markets with unique stable matchings.





==> backup/etc.tex <==
\section{Centralized Explore-then-Commit Algorithm in $\alpha$-reducible Markets}\label{sec:etc}
In this algorithm, each agent \( a \) updates their belief over firms \( f \in \mathcal{I}_a \) by computing the empirical mean:
\[
\hat{u}_{a,f}(t) = \hat{\mu}_{a,f}(t) = \frac{1}{T_{a,f}(t)} \sum_{t'=1}^t \mathbbm{1}\left\{f \in \mathcal{I}_a(t')\right\} X_{a,f}(t'),
\]
where \( T_{a,f}(t) \) denotes the number of times agent \( a \) has interviewed with firm \( f \) up to round \( t \). At each round, agent \( a \) constructs an ordered preference list \( \hat{O}_a(t) \) by sorting firms in descending order of their estimated valuations \( \hat{u}_{a,f}(t) \). This list is submitted to the central platform to determine interview assignments.

During the exploration phase, the platform arbitrarily partitions the firms into groups \( B_1, B_2, \dots, B_{m / \intesize} \), each of size \( \intesize \). Agents are similarly partitioned into groups of the same size and assigned to buckets in a round-robin manner, such that at each time step, every agent interviews with all firms from their assigned bucket. This bucketization strategy is inspired by the structure of \(\alpha\)-reducible markets and Lemma~\ref{l1}. 

If the platform could identify the fixed pair \( (a, f^*_a) \) for each agent \( a \), assigning each agent to the bucket containing their matched firm \( f^*_a \) and submitting the corresponding partial preference lists to the \(\FGS\) algorithm would recover the unique stable matching for the full market.

After the exploration phase concludes, both agents and firms proceed to the exploitation phase. Agents submit updated partial preference lists, and the platform runs the \(\FGS\) algorithm to compute the matching. Each agent is then restricted to be matched with a firm from their assigned bucket \( B_i \), i.e., \( f_a(t) \in B_i \).

\begin{lemma}\label{l1}
In an \(\alpha\)-reducible market, if each agent \( a \) has their true match \( f^*_a \) included in their interviewed set \( \mathcal{I}_a \), then submitting these partial preference lists to the \(\FGS\) algorithm yields the unique stable matching with respect to the full preference profiles.
\end{lemma}





\begin{algorithm}
\caption{Explore-Then-Commit}\label{alg:etc}
\begin{algorithmic}
\Require $T,\ \intesize,\ k\geq 0$, $u_f(a)$
\For{$t=1,2,3,...,t\leq\frac{m}{\intesize}k$}
\State $I_a(t)=B_{t \% \intesize}$, $\forall a \in\mathcal{A}$ 
\EndFor
\State run $\FGS$ over $\vec{O}_a(t)$s to find the $\hat{f}^*$s. 
\State  $I_a(t)=B_{i:f^*_a\in B_i}, $$\forall a \in\mathcal{A}$ 




\end{algorithmic}
\end{algorithm}

Now, we define \emph{valid} preference lists which is borrowed from \cite{liu2020competing}:
\begin{definition}
We call the $\hat{O}_a(t)$ a valid list if whenever a firm $f_a$ has lower index in $\hat{O}_a(t)$ than $f_j$, then $u_a(f_a)\geq u_a(f_j)$.
\end{definition}

\begin{lemma}\label{l3} \cite{liu2020competing}
In case of multiple optimal stable matchings, if all agents submit valid $\hat{O}_a(t)$s, then running $\FGS$ over them would find a stable matching which provides all agents weakly better matches.
\end{lemma}

\begin{lemma}\label{l2}
In $\alpha-reducible$ markets, if every agent $a$ submits a valid $\hat{O}_a(t)$, then running $\FGS$ on the reported lists would exactly be the unique stable matching.
\end{lemma}



lemma \ref{l3}, is important in regret analysis. Now, we can prove that the probability of submitting valid lists after $\frac{m}{\intesize}.k$ rounds of exploration would be considerably low. 

\begin{lemma} \cite{liu2020competing} \label{lemma:etc}
    Consider the agent $a$ and let $\Delta_{a, f}=u_a(f^*_a)-u_a(f)$ and $\Delta_{a}^\text{min}=\min _{f: \Delta_{a, f}>0} \Delta_{a, f}$. Then, if $a$ follows the Explore-then-Commit platform, we have
$$
\mathbb{P}\left(\hat{O}_a(t) \text{ is invalid} \right) \leq \frac{m}{\intesize} e^{-\frac{k\Delta_{a}^{\text{min}^2}}{2}} .
$$
\end{lemma}



\subsection{ETC Regret Analysis}
\begin{lemma}\label{lemma:etcreg}
The regret of ETC algorithm\ref{alg:etc} for an agent $a$ would be:
$$
R_a(T) \leq k \sum_{t=1}^\frac{m}{\intesize} \Delta_{a, f_a(t)}+(T-k \frac{m}{\intesize}) \Delta_{a, \max } n \frac{m}{\intesize} \exp \left(-\frac{k \Delta_{a}^{\text{min}^2}}{4}\right)
$$
\end{lemma}






==> backup/multi-agent-EAP.tex <==
\section{\xw{Multi-Agent Market Matching with Interview Constraint}}

\subsection{\xw{Objectives}}

\paragraph{\xw{Maximize the cumulative reward:}}

\paragraph{\xw{Find a stable matching:}}

\todo{Please fill in the definition of both objectives, and explain what our algorithm aims for?}

\subsection{Multi-Agent EAP}\label{meap:def}
In this section, we focus on extending our algorithm to the multi-agent case in which the firms that each agent gets matched to at each time step are decided by the $\FGS$ algorithm. In this context, agents can choose and apply to the companies using the EAP algorithm (Algorithm~\ref{alg:eap}) tuned with different $i$ values that each agent separately decides upon. However, the major problem in the multi-agent setting is that $I_{a'}(t)$\todo{\(I_{a'}(t)\) is the input \(i\) for EAP algorithm of agent \(a\) at time \(t\)? why \(a'\) instead of \(a\)?} affects the instant regret of agent $a$. Thus, each agent has to efficiently tune their $i$ value to be able to utilize the excellent result of Theorem \ref{thm:eap-regret} and suffer from constant regret while learning their stable match.

\subsubsection{Multi-Agent EAP (MAEAP) meta-algorithm}
In this meta-algorithm, each agent $a\in \mathcal{A}$ at each time step $t$ keeps a probability vector $\Vec{P}_a(t) \xw{= (P_{a,f}(t))_{f\in\mathcal{F}}}$ over all the firms (arms), where $P_{a,f}(t)$ is the probability of firm $f$ being chosen by $a$ as one of the three firms they want to interview. At each time step, each agent $a$ passes through the arms in their sorted $\UCB'$ list \xw{in a descending order}. For each arm $f$, the agent tosses a biased coin, which appears as Heads with the corresponding probability $P_{a,f}(t)$. Then, \xw{agent} $a$ would apply and interview with the first two arms for which their coins both land on Heads. Let's call them $f_1$ and $f_2$, and one other firm $f_{RR}$, which is chosen with the Round-Robin Approach ($I_a(t) = \{f_1,f_2,f_{RR}\}$). After the interview part, each agent submits a partially ordered preference list of $f_1$, $f_2$, and $f_{RR}$, which would be either $\xw{\langle}f_1,f_2,f_{RR}\xw{\rangle}$ or $\xw{\langle}f_2,f_1,f_{RR}\xw{\rangle}$ depending on which of $f_1$ and $f_2$ has a greater instant reward at that time step. Then, the agent observes the $\FGS$'s outcome and updates $\Vec{P_{a}(t)}$ \todo{It should be \(\Vec{P}_{a}(t)\), not \(\Vec{P_{a}(t)}\)} to obtain $\Vec{P_a(t+1)}$ for the next round. Different algorithms could be achieved based on the variety of approaches that agents can utilize to initialize and update the vector $\Vec{P_a}$ over time. So we show the 

So the meta-algorithm is
\begin{algorithm}[H]
\caption{ Multi-Agent Extended \textit{All Probe} (MAEAP)}\label{alg:eap}
\begin{algorithmic}[1]
\Require \xw{decision rounds} $T$, \xw{number of firms} $F$, \xw{add the physical meaning of \(i\) here} $i$
\For{$ t \in  [T]$}
\State Observe $X_{t\%F,t}$
\State Observe $X_{(\UCB_{a,i,t}')^{-1},t}$
\State Observe $X_{(\UCB_{a,i+1,t}')^{-1},t}$
\State Pull the arm with the $\arg\max\{X_{(\UCB_{a,i,t}')^{-1},t},X_{(\UCB_{a,i+1,t}')^{-1},t}\}$
\State Update $\UCB'_a$ as \eqref{cucbp:2}
\EndFor
\end{algorithmic}
\end{algorithm}

\subsection{Centralized $\UCB'$ Interview Allocation} \label{sec:cucbp}
After analyzing the EAP algorithm for a single learner, we utilize it in the multi-agent setting while the Interview Allocation is done by a central platform.
In this section which is inspired by a result in \cite{liu2020competing}. Here, the agents keep and update their estimations using $\UCB'$ which is defined in \eqref{cucbp:2}. At each time step $t$, the agents submit their sorted list of estimations\todo{is this estimates? or UCBs? estimation is a process.} to a central platform that is responsible for Allocating the Interviews(Observations) for the agents.

According to corollary \ref{cor1:eap} As a centralized platform, it should allocate the interviews in such a way that the firms in $I_a(t)$ which are likely to get matched with \xw{the agent $a$ appear before the $f^*_a$ in the submitted preference list (sorted $\UCB'$ list $\hat{O}_a(t)$).}\todo{cannot understand the sentence.} In this regard, we propose an algorithm which\xw{where?} the central platform can utilize to help the agents suffer from a constant regret. As an example, if agent $a$ submits $\hat{O}_a(t) = <f_1,f_2,f_3,\dots,f^*_a,\dots,f_{|\mathcal{F}|}>$,\todo{use \(\langle \rangle\)} Then the interview allocation  $I_a(t)= \{f_1,f_2,f_{rr}\}$, $I_{f_1} = \{a\}$, and $I_{f_2} = \{a\}$ provides the agent $a$ with a \textit{"Good Observation"}.\todo{what is \(I_f\) why use \(I\) that is already used for \(I_a\)?}
The more \textit{Good Observation}s agents get, the more the multi-agent setting be like the single-agent setting which is proven to suffer from a regret like $O(|\mathcal{F}|^2)$ for each of them. The Two-Stage $\FGS$ Interview Allocation helps the Central Platform to provide each agent with \textit{"Good Observations"} at most of the time steps.
The \textit{pseudo-code} below describes how the agent $a$ interacts with the Centralized Interview Allocation Platform (CIAP) and the role the centralized platform plays there.
\begin{algorithm}[H]
\caption{ Centralized Interview Allocation Platform $(\CIAP)$}\label{routin:cucbp}
\begin{algorithmic}[1]
\For{$ t \in  [T]$}
\State agent $a$ submits $\hat{O}_a(t)$ to the $\CIAP$
\State $\CIAP$ runs $\TSGIA$ over the $\hat{O}s$ \xw{\(\hat{O}_a(t)\)'s for all agent \(a\)}  and returns $I_a(t)$s
\State agent $a$ observes $I_a(t)\doteq\{f'_a(t),f''_a(t),f_{rr}(t)\}$
\State agent $a$, interviews with $I_a(t)$ and updates the $\hat{O}_a(t)$ to the $\hat{O}_a(t+1)$.
\State agent $a$ submits the $\hat{O}_a(t+1)$ to the $\FGS$ and obtains the utility of the firm he/she gets matched to.

\EndFor
\end{algorithmic}
\end{algorithm}



\subsubsection{Two-Stage $\FGS$  Interview Allocation (TSGIA)}
The idea behind this algorithm is that agents are interested in interviewing with firms that are likely to hire them. Thus, $\FGS$ run over the uncertain submitted $\hat{O}_a$s might be useful to help the agents interview with plausible firms during the learning process. As described in routine \ref{routin:cucbp}, $\CIAP$ is responsible to help the agents to attend interviews which increases their probability of getting hired. 
In this algorithm, the central platform adds a notion of interviewing budgets \todo{use single character symbol may be better, as \(Ib\) may be misunderstood as \(I\cdot b\) and we do have a notation \(I\)} $Ib(f) \in \mathbb{R}$ \todo{\(\mathbb{R}\)? why not \(\mathbb{N}^+\)?} 
\todo{why \((f)\)? is this specific for a firm? or for agents? or in general?} to each firm and runs one-to-many version of $\FGS$ over the submitted preference lists,lets assume that $f'_a(t)$ be the match of agent $a$ at the end of this step. Then the platform eliminates the $f'_a(t)$ from the preference list of each agent $a$ and runs the many-to-one version of $\FGS$ on the new preference lists and the result would be $f''_a(t)$ as the matched firm for some agents $a$.

The reason behind adding Interviewing budgets to firms to transform the one-to-one $\FGS$ to the one-to-many $\FGS$ is to make sure that acceptable ratio (preferably all) of the agents gain \textit{"Good Observation"}s \todo{try ``a''} in the $\alpha$-\textit{reducible}. Here we present an example that shows why using many-to-one $\FGS$ for the interview allocation can help all agent's to observe \textit{"Good Observation"}s. Let's assume that at time step $t$ $$\hat{O}_{a_1}(t) = <f^*_{a_2}, f^*_{a_1},\dots> \quad \hat{O}_{a_2}(t) = <f^*_{a_3}, f^*_{a_2}, f^*_{a_4},\dots>$$
$$\PL_{f^*_{a_1}} = <a_1,\dots> \quad \PL_{f^*_{a_2}} = <a_1,a_2,\dots>\quad \PL_{f^*_{a_3}} = <a_2,\dots>$$
Running $\TSGIA$ with two stages of one-to-one $\FGS$ would have $I_{a_1}(t) = \{f^*_{a_2}, f^*_{a_1},f_{rr}\}$ and $I_{a_2}(t) = \{f^*_{a_3}, f^*_{a_4},f_{rr}\}$ which means $a_1$ gains \textit{"Good Observation"}s but $a_2$ does not. However, if we allow the interview allocation be a one-to-many matching with the budget at least two for each firm then the interview allocation of $\TSGIA$ would be $I_{a_1}(t) = \{f^*_{a_2}, f^*_{a_1},f_{rr}\}$ and $I_{a_2}(t) = \{f^*_{a_3}, f^*_{a_2},f_{rr}\}$ which provides \textit{"Good Observation"}s for both. 

Now that we can make sure that the $\TSGIA$ with two stages of many-to-one can help the agents to get \textit{"Good Observation"}s more often but how to set the budgets? What about the result of the main one-to-one $\FGS$; In other words, does having good observations guarantee that the agents will be hired by that one firm they are looking for? The short answer to both questions is how we define regret and the structure of the underlying $\alpha$-\textit{reducible} market. 

\begin{itemize}
    \item ((Disjoint Interview Allocation))

    This approach of interview allocation allows the agents to have mutually disjoint interviewing sets $I_a(t)$. In other words, setting $Ib(f) = 1$ for all firms, the algorithm would let all agents to choose among the two firm they interviewed with \todo{why? If budget is \(1\), how many number of firms one agent can interview?} which is exactly following the nature of EAP algorithm. If we can guarantee that $\TSGIA$, that applies the Disjoint Interview Allocation approach, provides all agents with the  \textit{"Good Observation"}s then every agent would suffer from a constant regret. 
    Here the $\TSGIA$ would be like:
    \begin{algorithm}[H]
\caption{ $\TSGIA$ with disjoint interviews}\label{alg:TSGIA_DI}
\begin{algorithmic}[1]
\Require $\hat{O}_a(t)$ \xw{for all agents \(a\)}, $Ib(f) = 1$

\State $M_1 \leftarrow \FGS(\hat{O})$
\State $\hat{O}_a' = \hat{O}_a \backslash M_1\xw{(a),} \quad  \forall a \in \mathcal{A}$

\State $M_2 \leftarrow \FGS(\hat{O}')$
\State return $I_a(t) = \{M_1(a),M_2(a),f_{rr}\}$ \xw{to each agent \(a\)}
\end{algorithmic}
\end{algorithm}

This algorithm allows us to let the notion of regret to remain as what is defined in \eqref{reg:eap}. However, the problem is that the result of running $\CIAP$ using this variation of $\TSGIA$ depends strongly on the structure of the market. To shed some light on the issue, based on what is mentioned in the corollary \ref{cor1:eap}, if the $f^*_{a}$ is the $i$-th preferred firm, having $M_1(a)\text{ and }M_2(a)$ located at any two indices in the interval $[1,i]$ the observation would be counted as a \textit{"Good Observation"}. So the portion of \textit{"Good Observation"}s an agent $a$ receives through time highly depends on where the fixed match of others are lying in their preference lists as well as how the preference list of the first looks like. The more similarity among the the preference lists, the more collisions pops up, and the less \textit{"Good Observation"}s the agents in the lower layers of $\alpha$-\textit{reducibility} would get.
\end{itemize}

\subsection{\xw{Theoretical Analysis}}

\begin{theorem}
    \xw{analyze the regret of \TSGIA}
\end{theorem}

\subsection{\xw{Simulation Results?}}

==> backup/ucb-v.tex <==


\subsection{$\ALLP^{\hat{\mu}}$ Algorithm with empirical mean}
In this section, we address a conjecture posed by the authors in~\cite{bhaskara2022online}, which questions the validity of Theorem~\ref{thm:apreg} when the simple empirical mean is used in place of $\UCB'$. The motivation for analyzing this variant lies in the observation that the \(\ALLP\) algorithm does not explicitly solve the \emph{Best Arm Identification} problem. Consequently, suboptimal arms with high variance may continue to be pulled with non-negligible probability, even toward the end of the time horizon. When extending this algorithm to the problem of learning stable matchings in two-sided markets, this limitation becomes more consequential: the objective shifts from merely achieving agent-wise acceptable regret to learning the \emph{true stable matching} that is globally optimal under the market's structure. 

To this end, we first prove the theorem under the special case of \emph{Bernoulli} reward distributions and then extend the result to arbitrary reward distributions. The algorithm under consideration is precisely \(\ALLP\) (Algorithm~\ref{alg:ap}), where the arms \( f^1_a(t) \) and \( f^2_a(t) \) are selected based on their empirical means \(\hat{\mu}\), rather than UCB estimates.




\begin{algorithm}[H]
\caption{$\ALLP^{\hat{\mu}}$ ($\APEM$)}\label{alg:apmh}
\begin{algorithmic}[1]
\Require $T$,
\For{$ t \in  [T]$}
\State Observe $X_{a,f_{t \% m}}(t)$
\State Observe $X_{a,f^1_a(t)}(t)$
\State Observe $X_{a,f^{2}_a(t)}(t)$
\State Pull the arm corresponding to $\arg\max\left\{X_{a,f^1_a(t)}(t), X_{a,f^2_a(t)}(t)\right\}$
\State Update the empirical means to $\hat{u}_{a,f^1_a(t)}(t+1)$, $\hat{u}_{a,f^2_a(t)}(t+1)$, $\hat{u}_{a,f_{t \% m}}(t+1)$.
\EndFor
\end{algorithmic}
\end{algorithm}


\subsubsection{Warm-Up: $\ALLP^{\hat{\mu}}$ over \emph{Bernoulli} distributions}
 Now by the proof of Lemma \ref{lemma:allpmuber} we introduce the intuition behind the correctness of this conjecture for \emph{Bernoulli} distributions and move further to prove the same argument for the broader class of underlying distributions.  

\begin{lemma}\label{lemma:allpmuber}
Given $p_1\geq p_2 \geq \cdots \geq p_m$, where $p_i$ is the mean of a Bernoulli distribution associated with the arm $f_i \in \mathcal{F}$ from the perspective of the agent $a \in \mathcal{A}$. The regret of $\ALLP^{\hat{\mu}}$ is of $O(m^2).$
\end{lemma}

\begin{proof}[proof 1]
We begin the proof by calculating \(\mathbf{E}\left[\max\{X_{p_i} X_{p_j}\}\right]\), where \(X_{p_i}\) and \(X_{p_j}\) are random variables sampled from Bernoulli distributions corresponding to the arms \(i\) and \(j\), respectively. Specifically, we can write:  
\begin{align}
 \mathbf{E}\left[\max\{X_{p_i} X_{p_j}\}\right] = p_i + \left(1 - p_i\right)p_j.   \label{eq:allpmubern}
\end{align}


Lets $i_t$ and $j_t$, respectively, denote the indices of the arms with the highest (\(f_a^1(t)\)) and second-highest(\(f_a^2(t)\)) empirical means, which are selected to be hinted and pulled by the \(\ALLP^{\hat{\mu}}\) algorithm. Without loss of generality, we assume $i\leq j$. Accordingly, we partition the time horizon \([T]\) into the occurrence  of \emph{Good Events} (\(\mathcal{G}\)) and \emph{Bad Events} (\(\mathcal{B}\)) as follows:

\begin{align}
 \mathcal{G} &= \{t\geq 1: 1 \in \{i_t,j_t\}\} \cup \{t\geq 1: p_{i_t} + \left(1-p_{i_t}\right)p_{j_t} \geq p_1\},\\
 \mathcal{B} &= \{t\geq 1: p_{i_t} + \left(1-p_{i_t}\right)p_{j_t} < p_1\}. \label{eq:Badev}
\end{align}
Now, we can argue that at every moment during \emph{Good Events}, the regret is \(0\). By Jensen's inequality, it can be observed that:  
\[
\mathbf{E}\left[\max\{X_{p_{i_t}}, X_{p_{j_t}}\}\right] \geq \max\{p_{i_t}, p_{j_t}\},
\]  
which implies zero regret at every time step \(t\) where \(1 \in \{i_t, j_t\}\). At other moments during \emph{Good Events}, the regret is also zero due to Equation~\eqref{eq:allpmubern}.

Now we finish the proof by bounding  $\mathbf{E}\left[\abs{\mathcal{B}}\right]$. In this respect,we can observe that at each moment at which a \emph{Bad Event} happens, the empirical mean of the chosen arms $i_t$ and $j_t$ are at least as large as that of  the optimal arm $p_1$, while their means satisfy the condition in \eqref{eq:Badev}. Therefore, we can write:
\footnotesize{
\begin{align}
    \Pr\left(\hat{\mu}_{i_t}(t) \geq \hat{\mu}_{1}(t) \land \hat{\mu}_{j_t}(t) \geq \hat{\mu}_{1}(t) \mid t \in \mathcal{B} \right) &\leq  \Pr\left(\hat{\mu}_{i_t}(t)+\hat{\mu}_{j_t}(t) \geq 2\hat{\mu}_{1}(t) \mid t \in \mathcal{B}\right),\nonumber\\
    &\leq \Pr\left(\hat{\mu}_{i_t}(t)+\hat{\mu}_{j_t}(t) \geq 2\hat{\mu}_{1}(t) \mid p_{i_t} + \left(1-p_{i_t}\right)p_{j_t} < p_1\right),\nonumber\\
    &\leq \Pr\left(\hat{\mu}_{i_t}(t)-p_{i_t}+\hat{\mu}_{j_t}(t) - p_{j_t} \geq 2\hat{\mu}_{1}(t)-p_1-p_{i_t}p_{j_t}\right),\nonumber\\
    &\leq \Pr\left(\abs{\hat{\mu}_{i_t}(t)-p_{i_t}}+\abs{\hat{\mu}_{j_t}(t) - p_{j_t}} \geq 2\hat{\mu}_{1}(t)-p_1-p_{i_t}p_{j_t}\right),\nonumber\\
    &\leq \Pr\left(\abs{\hat{\mu}_{i_t}(t)-p_{i_t}}+\abs{\hat{\mu}_{j_t}(t) - p_{j_t}} \geq \left(\hat{\mu}_{1}(t)-p_1\right)+\hat{\mu}_{1}(t) -p_{i_t}p_{j_t}\right). \label{ineq:badeventpr}
\end{align}
}
We then prove that the probability given in $\eqref{ineq:badeventpr}$ vanishes very fast due to the round-robin exploration done by $\ALLP^{\hat{\mu}}$ which consequently results into time independent upper bound for $\mathbf{E}[\abs{\mathcal{B}}]$ which is equivalent to constant regret. 
\end{proof}
The following Corollary~\ref{cor:allbernbut1} illustrates the underlying idea of how this approach can be extended to encompass broader classes of distributions.

\begin{corollary} \label{cor:allbernbut1}
Let \( X \) and \( Y \) be random variables such that \( X \) is drawn from a Bernoulli distribution with mean \( \mu_X \), and \( Y \) is drawn from an arbitrary distribution with mean \( \mu_Y \). We can then write:  
\begin{align*}
    \mathbf{E}\left[\max\{X, Y\}\right] &= \mu_X + \left(1 - \mu_X\right) \int_{t=0}^{1} t f_Y(t) \, dt, \\
    &= \mu_X + \left(1 - \mu_X\right) \mu_Y, \\
    &= \mu_X + \mu_Y - \mu_X \mu_Y.
\end{align*}
This result allows us to replicate the proof of Lemma~\ref{lemma:allpmuber} for this case as well.
\end{corollary}

\subsubsection{$\ALLP^{\hat{\mu}}$ over arbitrary distributions}

The next step is to extend this approach to cases where all arms are associated with distributions defined on discrete probability spaces, and then generalize it further. Our objective is to establish a form like:  
\[
\mathbf{E}[\max\{X, Y\}] = \mu_X + \mu_Y - f(f_X, f_Y),
\]
where \( f(f_X, f_Y) \) is a real-valued function. This formulation allows us to generalize Lemma~\ref{lemma:allpmuber} to cover arbitrary distributions supported on \([0,1]\), provided \( f(f_X, f_Y) < \mu^* \), where \( \mu^* \) represents the mean of the distribution associated with the optimal arm. By Lemma~\ref{lemma:Expmax}, we demonstrate that this argument holds for every probability distribution from which \(X\) and \(Y\) are sampled.  

\begin{lemma}\label{lemma:Expmax}
Let \(X\) and \(Y\) be independent random variables supported on \([0,1]\), with means satisfying \(\mu^* \geq \mu_Y \geq \mu_X\). Then:  
\[
\mathbf{E}[\max\{X,Y\}] = \mu_X + \mu_Y - f(f_X, f_Y),
\]
where \(f(f_X, f_Y) \leq \mu^*\).
\end{lemma}

\begin{proof}
We prove Lemma~\ref{lemma:Expmax} by starting with the inequality:  
\begin{align*}
    \mu_X &\leq \mathbf{E}[\max\{X, Y\}],\\
          &= \mu_X + \mu_Y - f(f_X, f_Y),\\
          &\leq \mu_X + \mu^* - f(f_X, f_Y).
\end{align*}
From this, it follows that \(f(f_X, f_Y) \leq \mu^*\), completing the proof.  
\end{proof}

Lemma~\ref{lemma:Expmax} supports our hypothesis about the generalized form of Lemma~\ref{lemma:allpmuber} for arbitrary bounded probability distributions. Now we have all the ingredients to prove Theorem

\begin{theorem}
    Given $\mu_1\geq \mu_2 \geq \cdots \geq \mu_m$, where $\mu_i$ is the mean of an arbitrary reward distribution supported on $[0,1]$ associated with the arm $f_i \in \mathcal{F}$ from the perspective of the agent $a \in \mathcal{A}$. The regret of $\ALLP^{\hat{\mu}}$ is of $O(m^2).$
\end{theorem}


However, determining precise bounds for the number of required round-robin hints depends heavily on the nature of the distributions that govern the difference \(\mu^* - f(f_X, f_Y)\). In the following, we describe a method to achieve accurate bounds for \(f(f_X, f_Y)\).  

The example below provides additional clarification for the case of Bernoulli distributions, which we will generalize to all probability distributions.


\begin{example}
Here we assume $\sum_i p_i, \sum_j q_j = 1$, and $\mu_X = \sum_i p_ix_i$, and $\mu_Y = \sum_j q_jy_j$.
\begin{figure}[ht]
    \centering
    \begin{tikzpicture}
    % Left vertical dashed line
    \draw[thick, dashed] (-2, 0) -- (-2, 5);
    % Points and labels on the left line
    \node[fill, circle, inner sep=2pt] at (-2, 4.5) {};
    \node[anchor=east] at (-2, 4.5) {\((x_1, p_1)\)};
    \node[fill, circle, inner sep=2pt] at (-2, 2.5) {};
    \node[anchor=east] at (-2, 2.5) {\((x_2, p_2)\)};
    \node[fill, circle, inner sep=2pt] at (-2, 0.7) {};
    \node[anchor=east] at (-2, 0.7) {\((x_3, p_3)\)};
    
    % Right vertical dashed line
    \draw[thick, dashed] (2, 0) -- (2, 5);
    % Points and labels on the right line
    \node[fill, circle, inner sep=2pt] at (2, 4) {};
    \node[anchor=west] at (2, 4) {\((y_1, q_1)\)};
    \node[fill, circle, inner sep=2pt] at (2, 1.5) {};
    \node[anchor=west] at (2, 1.5) {\((y_2, q_2)\)};
    \node[fill, circle, inner sep=2pt] at (2, 0.35) {};
    \node[anchor=west] at (2, 0.35) {\((y_3, q_3)\)};
    
    % Dashed arrows from (x_i, p_i) to (y_i, q_i)
    \draw[thick, dashed] (-2, 4.5) -- node[midway, sloped, above] {\(\rightarrow\)} (2, 4);
    \draw[thick, dashed] (-2, 2.5) -- node[midway, sloped, above] {\(\rightarrow\)} (2, 1.5);
    \draw[thick, dashed] (-2, 0.7) -- node[midway, sloped, above] {\(\rightarrow\)} (2, 0.35);
    
    % Dashed arrows from (y_i, q_i) to (x_{i+1}, p_{i+1}), reversed direction
    \draw[thick, dashed] (-2, 2.5) -- node[midway, sloped, above] {\(\leftarrow\)} (2, 4);
    \draw[thick, dashed] (-2, 0.7) -- node[midway, sloped, above] {\(\leftarrow\)} (2, 1.5);
\end{tikzpicture}
\end{figure}

Now we can write
\begin{align}
\mathbf{E}\left[\max\{X,Y\}\right] &= p_1x_1 + \left(1-p_1\right)\mathbf{E}\left[\max\{X,Y\}\mid X \neq x_1\right],\nonumber\\
&= p_1x_1 + \left(1-p_1\right)q_1y_1 + \left(1-q_1\right)\mathbf{E}\left[\max\{X,Y\}\mid Y \neq  y_1\right],\nonumber\\
&\cdots,\nonumber\\
&= 
\end{align}
\end{example}







% \begin{corollary}\label{cor1:eap}
% For a given integer $i$ and agent $a$, we assume $f^{i}_a$  be the $a$'s $i$-th best first regarding the ground truth and $k$ denotes the size of the set $K\coloneqq \{f\in L_a: \Delta_{a,f^{i^{th}}_a,f} = \alpha\sigma^2_f, \alpha\leq \frac{1}{2}\}$. Then running EAP over any two chosen arms from indices $[i,i+k]$ at each time step would provide the agent a with a regret similar to the bound of Theorem \ref{thm:eap-regret}.
% \end{corollary}


==> dfgs.tex <==

\subsection{~\cref{obs:drr1}}
\begin{restatable}{lemma}{obsdrrone}\label{obs:drr1}
In a matching market $\MM$ where firms follow~\cref{alg:fdrr} and agents follow~\cref{alg:drr}, at the end of any updating phase that starts at time $\TGS$, the applications $(a,\FA_a(\TGS+3n^2))_{a\in\AG}$ form a matching that matches all agents.
\end{restatable}
\begin{proof}
Since the beginning of the updating phase at time $\TGS$, each agent $a$ selects its applied firm according to
\[
\FA_a(t) = \argmax_{f \in \CSV_a(t)} \hat{u}_{a,f}(\TGS),
\]
that is, with respect to its estimated preference list $\EPL_a(\TGS)$. Consequently, during the updating phase, each agent effectively traverses $\EPL_a(\TGS)$ in descending order, applying to increasingly less preferred firms until reaching one that does not reject it in favor of another agent. Once an agent $a$ becomes matched to a firm $f=\FA_a(t)$, it continues to apply to $f$ in subsequent rounds until either the updating phase ends or $f$ rejects $a$ by hiring another agent. Therefore, whenever the application profile $(a,\FA_a(t))_{a\in\AG}$ does not form a perfect matching, there exists at least one agent who advances to a less preferred firm in the next round.

In addition to rejections caused by competing applicants, agents may experience \emph{strategic rejections}. However, by construction, the rejection variable $r_{a,f}$ is updated only when firm $f$ hires another agent, i.e., when $\NH_f(t)=1$, and not when $f$ strategically abstains from hiring. As a result, following a strategic rejection, agents reapply to the same firm in the subsequent round. Moreover, under~\cref{alg:fdrr}, no firm performs strategic rejections in two consecutive rounds during an updating phase. Along with the observations that agents wont apply to a firm more thean once if they become rejected in favor of hiring other agent implying that each firm can reject a given agent at most twice during the whole updataing stage staring from $\TGS$, at most one strategically and one in favor of hiring another agent. 

It follows that as long as the applications do not form a perfect matching, within at most two rounds there exists at least one agent who moves to a less preferred firm. Since each agent’s match during the updating phase is restricted to the top $n$ firms in $\EPL_a(\TGS)$, the application profile forms a perfect matching within at most $2n^2+1$ rounds. In particular, after at most $3n^2$ rounds from the start of an updating phase, the applications $(a,\FA_a(t))_{a\in\AG}$ form a perfect matching. As a consequence, each agent applies to at most the top $n$ firms in its estimated preference list during a single updating phase.

% If firms are certain and always hire under Algorithm~\ref{alg:fdrr}, then by the definition of $\CSV_a(t)$ and the decision rule of agents based on their estimated preference lists at time step $\TGS$, 
% coordinating on setting $r_{a,f}(\TGS) = 0$ for all firms ensures that agents following Algorithm~\ref{alg:drr} effectively simulate the execution of $\FGS$ on $\EPL_a(\TGS)$. 
% For any market, such a run of $\FGS$ is guaranteed to complete within at most $n^2$ rounds. However, in the case of \emph{uncertain} firms, some firms may temporarily refrain from hiring at a time step $t$. 
% According to the update rule for $r_{a,f}$ during the updating phase, when agent $a$ is rejected by its selected firm $\FA_a(t)$ due to $\NH_{\FA_a(t)}(t)=0$, 
% it sets $\FA_a(t+1) = \FA_a(t)$ and remains at that firm in the next round. 
% At this point, $a$ is either hired or blocked by another agent. 
% If $a$  the most preferred applicant, then there will be no subsequent time step at which $a$ is rejected again due to strategic non-hiring. 
% Hence, each agent can experience at most one rejection caused by a firm’s strategic non-hiring per round, 
% which in the worst case adds only one additional round for every rejection. 
% Consequently, $3n^2$ rounds are sufficient for all agents to obtain distinct assignments $\FA_a(\TGS + 3n^2)$, completing the updating phase.

\end{proof}

\subsection{Proof of Observation~\ref{obs:drr2}}


\begin{restatable}{observation}{obsdrrtwo}\label{obs:drr2}
The total number of updating stages is given by 
\(
    \mathbb{E}\!\left[\left|\bigcup_{a \in \AG} \left(\mathcal{S}^{\mathrm{inc}}_{a} \cup \mathcal{S}^{\mathrm{rej}}_{a}\right)\right|\right].
\)
\end{restatable}
%\obsdrrtwo*
\begin{proof}
This holds because whenever an agent $a \in \AG$ detects an event in $\mathcal{S}^{\mathrm{inc}}_a$, 
it abstains from applying in that round, which is subsequently revealed to all other agents 
through their detection of events in $\mathcal{S}^{\mathrm{vac}}_{a'}$. 
Similarly, if $a$ detects an event in $\mathcal{S}^{\mathrm{rej}}_a$, it indicates that at that time step 
the agent was strategically not hired, an event that is also reflected to others 
via $\mathcal{S}^{\mathrm{vac}}_{a'}$ in the firm-side feedback. 
Therefore, every initialization of a new distributed $\FGS$ run is ultimately triggered 
by at least one agent $a$ detecting the current time step $t$ as belonging to 
either $\mathcal{S}^{\mathrm{inc}}_a$ or $\mathcal{S}^{\mathrm{rej}}_a$.

\end{proof}

\subsection{Proof of Lemma~\ref{lemma:alphadec}}
\begin{restatable}{lemma}{lemmalphadec}\label{lemma:alphadec}
In an $\alpha$-reducible market, with strategic firms following~\cref{alg:fdrr} and agents following~\cref{alg:drr}, the total number of updating stages is $O(nm^2)$.
\end{restatable}
%\lemmalphadec*
\begin{proof}

    Consider the unique stable matching \((a_i, f_i)_{i \in [n]}\) in an $\alpha$-reducible market.
For each \(i \in [n]\), define the set of time steps
\[
\mathcal{G}_i \doteq \{t \in \mathcal{C} : \forall j \in [i],\ \FA_{a_j}(t) = f_j\},
\]
namely, the rounds in which agents \(a_1, \ldots, a_i\) all apply to their respective stable partners.
Its complement \(\Bar{\mathcal{G}}_i\) consists of rounds in which at least one of these agents is not matched to its stable partner.

We now bound the expected number of switching events across all agents. In particular, with respect to~\cref{obs:drr2}, we bound
\(
\mathbb{E}\!\left[\left|\bigcup_{a_i\in \AG}\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i} \right|\right]
\)
as follows:
{\small
\begin{align}
\mathbb{E}\!\left[\left|\bigcup_{a_i\in \AG}\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i} \right|\right]
&=\mathbb{E}\!\left[\!\left|\bigcup_{a_i\in \AG}
\!\!\left(
\!\{t\!\in\!\mathcal{S}^{\mathrm{inc}}_{a_i}\!\cup\!\mathcal{S}^{\mathrm{rej}}_{a_i}:t\!\in\!\Bar{\mathcal{G}}_i\}
\cup
\{t\!\in\!\mathcal{S}^{\mathrm{inc}}_{a_i}\!\cup\!\mathcal{S}^{\mathrm{rej}}_{a_i}:t\!\in\!\mathcal{G}_i\}
\!\right)\!\right|\!\right] \nonumber\\
&\leq
\mathbb{E}\!\left[\!\left|\bigcup_{a_i\in \AG}
\!\!\left(
\Bar{\mathcal{G}}_i
\cup
\{t\!\in\!\mathcal{S}^{\mathrm{inc}}_{a_i}\!\cup\!\mathcal{S}^{\mathrm{rej}}_{a_i}:t\!\in\!\mathcal{G}_i\}
\right)\!\right|\!\right] \nonumber\\
&\overset{(a)}{\leq}
\mathbb{E}\!\left[\!\left|
\bigcup_{a_i\in \AG}\!\left(\Bar{\mathcal{E}}_{a_i,f_i}\!\cup\!\Bar{\mathcal{E}}_{f_i,a_i}\right)
\cup
\bigcup_{a_i\in \AG}\!\left(
\{t\!\in\!\mathcal{S}^{\mathrm{inc}}_{a_i}\!\cup\!\mathcal{S}^{\mathrm{rej}}_{a_i}:t\!\in\!\mathcal{G}_i\}
\right)
\!\right|\!\right] \nonumber\\
&\overset{(b)}{\leq}
\mathbb{E}\!\left[\!\left|
\bigcup_{a_i\in \AG}\!\left(\Bar{\mathcal{E}}_{a_i,f_i}\!\cup\!\Bar{\mathcal{E}}_{f_i,a_i}\right)
\cup
\bigcup_{a_i\in \AG}\!\left(
\!\{t\!\in\!\mathcal{S}^{\mathrm{inc}}_{a_i}\!\cup\!\mathcal{S}^{\mathrm{rej}}_{a_i}:
(t\!\in\!\mathcal{G}_i)
\land
(t,t\!-\!1\!\in\!\mathcal{E}_{a_i,f_i}\!\cap\!\mathcal{E}_{f_i,a_i})\!\}
\right)
\!\right|\!\right] \nonumber\\
&\overset{(c)}{\leq}
\sum_{i\in[n]}\Bigg(
\mathbb{E}\!\left[\!\left|\Bar{\mathcal{E}}_{a_i,f_i}\right|\!\right]
+\mathbb{E}\!\left[\!\left|\Bar{\mathcal{E}}_{f_i,a_i}\right|\!\right]
+\!\!\sum_{f\in\mathcal{H}_{a_i,f_i}}\!\!
\mathbb{E}\!\left[\!\left|\!\{t:
f\!\in\!\hat{\mathcal{L}}_{a_i,f_i}(t\!-\!1)
\!\cap\!\hat{\mathcal{H}}_{a_i,f_i}(t)\}\!\right|\!\right]\Bigg), \nonumber\\
% &\hspace{2.3cm}
% +\!\!\sum_{a\in\mathcal{H}_{f_i,a_i}}\!\!
% \mathbb{E}\!\left[\!\left|\!\{t:
% a\!\in\!\hat{\mathcal{L}}_{f_i,a_i}(t\!-\!1)
% \!\cap\!\hat{\mathcal{H}}_{f_i,a_i}(t)\}\!\right|\!\right]
% \Bigg) \nonumber\\
&\overset{(d)}{\leq}
\sum_{a_i\in\AG}
\frac{4m \exp\!\left(-\tfrac{(\overline{\Delta}^{\texttt{min}}_{a_i})^2}{2m}\right)}{1 - \exp\!\left(-\tfrac{(\overline{\Delta}^{\texttt{min}}_{a_i})^2}{2m}\right)}
+
\sum_{f_i\in\FI}
\frac{4n \exp\!\left(-\tfrac{(\overline{\Delta}^{\texttt{min}}_{f_i})^2}{2m}\right)}{1 - \exp\!\left(-\tfrac{(\overline{\Delta}^{\texttt{min}}_{f_i})^2}{2m}\right)}
\in O(nm^2),
\label{eq:alphadGS}
\end{align}
}

Here, inequality~(a) follows from the fact that if \(t \in \Bar{\mathcal{G}}_i\), then either some agent \(a_j\) has an invalid estimated preference list at time \(\TGS\), or there exists a time step \(t' \in [\TGS, \TGS + 3n^2]\) at which the firm \(f_j\), for some \(j \in [i]\), has an invalid estimated preference list.


The justification of inequality~(b) follows by considering the possible cases when
$t-1 \in \mathcal{G}_i$.

\begin{itemize}
\item[(i)]
Either $\EPL_{a_i}(t-1)$ or $\EPL_{f_i}(t-1)$ is invalid.
In this case,
$t-1 \in \Bar{\mathcal{E}}_{a_i,f_i} \cup \Bar{\mathcal{E}}_{f_i,a_i}$,
and the subsequent execution of $\FGS$ can be charged to round $t-1$ as an instance of an invalid preference list.

\item[(ii)]
Both $\EPL_{a_i}(t-1)$ and $\EPL_{f_i}(t-1)$ are valid, but at least one becomes invalid at time $t$.
If $\EPL_{a_i}(t)$ becomes invalid, then $t \in \mathcal{S}^{\mathrm{inc}}_{a_i}$, corresponding to a switching event by the agent.
If instead $\EPL_{f_i}(t)$ becomes invalid, firm $f_i$ may perform a strategic rejection, yielding
$t \in \mathcal{S}^{\mathrm{rej}}_{a_i}$.
In either case, the ensuing updating phase, and hence the next execution of $\FGS$, is associated with
$t \in \Bar{\mathcal{E}}_{a_i,f_i} \cup \Bar{\mathcal{E}}_{f_i,a_i}$.

\item[(iii)]
Both $\EPL_{a_i}(t-1)$ and $\EPL_{a_i}(t)$, as well as $\EPL_{f_i}(t-1)$ and $\EPL_{f_i}(t)$, are valid.
Suppose first that firm $f_i$ performs a strategic rejection at time $t$, i.e., $t\in \mathcal{S}_{f_i}$.
This action is observed by agent $a_i$ through $\VFP(t)$, and therefore implies $t\in \mathcal{S}^{\mathrm{rej}}_{a_i}$.

Since all agents $a_j$ for $j\in[i-1]$ are matched to their stable partners $f_j$, and since $t\in \mathcal{E}_{f_i,a_i}$, we claim that there must exist some agent $a_j$ whose estimated preference list was invalid at some time during the previous updating phase $[\TGS,\TGS+3n^2]$.
Indeed, the strategic rejection by $f_i$ can only be triggered if there exists an agent $a_j$ that $f_i$ truly prefers (i.e., $a_j \in \mathcal{H}_{f_i,a_i}$) but that was previously rejected by $f_i$ during the updating phase.
Concretely, during the updating phase, agent $a_j$ applied to $f_i$ and was rejected at some time $t'$, which means that at the time of rejection $a_j \in \hat{\mathcal{L}}_{f_i,a_i}$.
After this rejection, $a_j$ subsequently applied to (and matched with) some firm $f_j$ that it estimated to be less preferred.
Given that $f_i$ later performs a strategic rejection, this sequence of events implies that $a_j$'s estimated preference list must have been invalid at time $t'$.


Otherwise, if no strategic rejection occurs at time $t$ and $t \in \mathcal{S}^{\mathrm{inc}}_{a_i}$, then since
$t-1,t \in \mathcal{E}_{a_i,f_i} \cap \mathcal{E}_{f_i,a_i}$,
a switching event of type $\mathcal{S}^{\mathrm{inc}}_{a_i}$ implies that there exists a firm
$f \in \mathcal{H}_{a_i,f_i}$ such that
$f \in \hat{\mathcal{L}}_{a_i,f_i}(\TGS)$ but
$f \in \hat{\mathcal{H}}_{a_i,f_i}(t)$.
% Similarly, for a strategic rejection by $f_i$ at time $t$, there must exist an agent
% $a \in \mathcal{H}_{f_i,a_i}$ that was previously rejected in favor of $a_i$ and is now estimated to be preferred to $a_i$,
% which again yields $t \in \mathcal{S}^{\mathrm{rej}}_{a_i}$.
\end{itemize}

These cases together establish inequality~(c). Inequality (d) then follows with the same approach as used in the proof of Lemma~\ref{lemma:valid-rr}.
\end{proof}

\subsection{Proof Sketch of Theorem~\ref{thm:alphadecreg} for the agent $a_1$} \label{proof:sketchthmalphareg}

\begin{proof}[Proof sketch of~\cref{thm:alphadecreg}]
We decompose the regret of agent $a_1$ into the regret incurred during updating phases $\mathcal{U}$ and committing phases $\mathcal{C}$ as:
\(\mathbb{E}[R_{a_1}(\mathcal{T})]=\mathbb{E}[R_{a_1}(\mathcal{U})]+\mathbb{E}[R_{a_1}(\mathcal{C})]\).

We first bound the updating-phase regret. By \cref{obs:drr2} and \cref{lemma:alphadec}, the expected number of updating stages is time-independent, and each stage incurs regret at most $3n^2$; hence 
{\small\begin{align}
  \mathbb{E}[R_{a_1}(\mathcal{U})]\le 3n^2\,\mathbb{E}\!\left[\left|\bigcup_{a_i\in \AG}(\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i})\right|\right]\in O(n^3m^2)  
\end{align}}

For the committing phase, we show $\mathbb{E}[R_{a_1}(\mathcal{C})]\le \mathbb{E}\!\left[\left|\bigcup_{a_i\in \AG}(\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i})\right|\right]+\mathbb{E}[|\Bar{\mathcal{E}}_{a_1,f_1}|]+\mathbb{E}[|\Bar{\mathcal{E}}_{f_1,a_1}|]$. Applying \cref{lemma:alphadec} and \cref{lemma:valid-rr} (for agents and firms) yields the claimed $\,O(n^3m^2)\,$ bound. The first term accounts for signaling rounds, which happen at most once per committing stage, immediately before an updating phase, when an agent detects a switching condition and abstains from applying.

Now fix a committing interval $[t_1:t_2]$. If $\FM_{a_1}(t_1)=f_1$, then $a_1$ incurs no regret over $[t_1:t_2]$. Otherwise, since $a_1$ and $f_1$ are mutual top choices in the unique stable matching, the most recent updating phase must have started at some $\TGS\in \Bar{\mathcal{E}}_{a_1,f_1}\cup \Bar{\mathcal{E}}_{f_1,a_1}$, i.e., at that time at least one of $a_1$ or $f_1$ had an invalid estimated list.

If $f_1$ strategically rejects $a_1$ during this updating phase, then the resulting committing interval has length one and is already covered by the signaling term. Otherwise, in an $\alpha$-reducible market, this invalidity persists throughout $[t_1:t_2]$ until a new updating phase is triggered, which can happen only when (i) $a_1$ detects a preference inconsistency, (ii) $f_1$ strategically rejects, or (iii) another agent initiates a new updating phase. Thus each committing interval can be uniquely charged to an invalidity event on either the agent or firm side, and these intervals are disjoint. Consequently, the total committing-phase regret excluding signaling rounds is bounded by $\mathbb{E}[|\Bar{\mathcal{E}}_{a_1,f_1}|]+\mathbb{E}[|\Bar{\mathcal{E}}_{f_1,a_1}|]\in O(m^2+nm)$.
\end{proof}
\subsection{Proof of Theorem~\ref{thm:alphadecreg}} \label{proof:thmalphareg}
\thmalphadecreg*
\begin{proof}
We decompose the regret of agent $a_i$ into two components:
(i) regret incurred during \emph{updating} phases, denoted by $\mathcal{U}$, and
(ii) regret incurred during \emph{committing} phases, denoted by $\mathcal{C}$.
Formally, the expected regret satisfies
\begin{align}
\mathbb{E}\!\left[R_{a_i}(T)\right]
&=
\mathbb{E}\!\left[R_{a_i}(\mathcal{U})\right]
+
\mathbb{E}\!\left[R_{a_i}(\mathcal{C})\right] \nonumber\\
&=
\underbrace{
\sum_{t \in \mathcal{U}}
\left(
u_{a_i,f_i}
-
\mathbb{E}[X_{a_i,\FM_{a_i}(t)}]
\right)
}_{\text{updating regret}}
+
\underbrace{
\sum_{t \in \mathcal{C}}
\left(
u_{a_i,f_i}
-
\mathbb{E}[X_{a_i,\FM_{a_i}(t)}]
\right)
}_{\text{committing regret}}.
\label{eq:decregalpha}
\end{align}
We bound these two terms separately.

We begin with the cumulative regret incurred during the updating phases. By construction, each updating phase lasts at most $3n^2$ rounds, and in each such round an agent incurs regret at most one. Moreover, by\cref{obs:drr2} and~\cref{lemma:alphadec}, the expected number of updating phases is bounded by the number of switching events across all agents. Consequently,
\begin{align}
\sum_{t \in \mathcal{U}}
\left(
u_{a_i,f_i}
-
\mathbb{E}[X_{a_i,\FM_{a_i}(t)}]
\right)
&\le
3n^2 \cdot\,
\mathbb{E}\!\left[
\left|
\bigcup_{a \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a
\right)
\right|
\right].
\label{ineq:update-regret}
\end{align}

    
   We now focus on the second term, corresponding to regret incurred during committing phases.
Let
\[
\bigcup_{a \in \AG} \left(\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a\right)
= \{t_1,t_2,\ldots\}
\]
denote the set of switching times, ordered increasingly.
The $j$-th committing phase is defined as the interval
\[
[t'_j : t_{j+1}],
\qquad
\text{where } t'_j \doteq t_j + 3n^2 + 1,
\]
corresponding to the period between the $j$-th and $(j+1)$-th distributed executions of $\FGS$.
The collection of committing intervals is therefore
\[
\mathcal{K}
\doteq
\left\{
[t'_j,\, t_{j+1}] :
j \in \left[\left|\!\bigcup_{a \in \AG}(\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a)\right|\right]
\right\}.
\]

The expected regret incurred during committing phases can then be written as
{\small\begin{align}
\mathbb{E}\!\left[R_{a_i}(\mathcal{C})\right]
&=
\sum_{t \in \mathcal{C}}
\left(
u_{a_i,f_i}
-
\mathbb{E}[X_{a_i,\FM_{a_i}(t)}]
\right) \nonumber\\
&=
\mathbb{E}\!\left[
\sum_{j=1}^{|\mathcal{K}|}
\sum_{t \in [t'_j,\, t_{j+1}]}
\Big(
u_{a_i,f_i}
-
X_{a_i,\FM_{a_i}(t'_j)}(t)
\Big)
\right],\nonumber\\
&\overset{(a)}{\le} \mathbb{E}\!\left[
\left|
\bigcup_{a \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a
\right)
\right|
\right] +
\mathbb{E}\!\left[
\sum_{j \in [|\mathcal{K}|]}
\bigl(t_{j+1}-1-t'_j\bigr)
\;\middle|\;
\FM_{a_i}(t'_j) \in \mathcal{L}_{a_i,f_i}
\right],  \nonumber\\
&\le
\mathbb{E}\!\left[
\left|
\bigcup_{a \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a
\right)
\right|
\right]+\mathbb{E}\!\left[
\sum_{j \in [|\mathcal{K}|]}
\bigl(t_{j+1}-1-t'_j\bigr)
\;\middle|\;
\FM_{a_i}(t'_j) \in \mathcal{L}_{a_i,f_i} \land t'_j  \in \mathcal{G}_{i-1}
\right]
+
\mathbb{E}\!\left[
\sum_{j \in [|\mathcal{K}|]}
\bigl(t_{j+1}-1-t'_j\bigr)
\;\middle|\;
t'_j \in \Bar{\mathcal{G}}_{i-1}
\right], \nonumber\\
&\overset{(b)}{\le}
\mathbb{E}\!\left[
\left|
\bigcup_{a \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a
\right)
\right|
\right]+ \mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{a_i,f_i}\right|\right]
+
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{f_i,a_i}\right|\right]
+
\mathbb{E}\!\left[
\sum_{j \in [|\mathcal{K}|]}
\bigl(t_{j+1}-1-t'_j\bigr)
\;\middle|\;
t'_j \in \Bar{\mathcal{G}}_{i-1}
\right], \nonumber\\
&\overset{(c)}{\le}
\mathbb{E}\!\left[
\left|
\bigcup_{a \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a
\right)
\right|
\right]+
\sum_{j=1}^{i}
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{a_j,f_j}\right|\right]
+
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{f_j,a_j}\right|\right],\label{ineq:finalalphadec}
\end{align}
}
    
    
    Inequality~(a) follows by accounting for single round at the end of each committing phase, $t_{j+1}$ in which agent $a_i$ intentionally refrains from applying in order to signal coordination to other agents. Such a signaling round occurs at most once per committing phase, immediately before the subsequent updating phase. By~\cref{obs:drr2}, the expected number of these signaling rounds is bounded by
\(
\mathbb{E}\!\left[
\left|
\bigcup_{a \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a
\right)
\right|
\right].
\) This term also includes the cases when $a_i$ was strategically rejected during the last updating stage.

    Inequality~(b) follows from the structure of $\alpha$-reducible markets. 
Condition on $t'_j \in \mathcal{G}_{i-1}$, so that the first $i-1$ agents are matched to their optimal firms, while agent $a_i$ is matched suboptimally to some firm in $\mathcal{L}_{a_i,f_i}$. 
By $\alpha$-reducibility, one of the following must hold.

(i) Either agent $a_i$ has applied to its optimal firm $f_i$ and was rejected during the last updating stage. In this case, firm $f_i$ must be matched to a suboptimal agent due to an invalid estimated preference list during the preceding updating phase. This firm-side invalidity can persist during the committing phase, but at most until $f_i$'s preference list become valid at which it strategically rejects its current match cause $a_i$ which was previously rejected now becomes a preferred agent than its current applicant.

(ii) Alternatively, agent $a_i$ has not applied to $f_i$ while updating and is matched to a less preferred firm. This implies that $a_i$’s estimated preference list was already invalid at the start of the updating phase phase, and this agent-side invalidity may persist until it is corrected.

In both cases, the committing regret incurred while $t'_j \in \mathcal{G}_{i-1}$ can be uniquely charged to an invalidity event in either the agent’s or the firm’s estimated preference list. Consequently, the total committing regret of agent $a_i$ over all such disjoint intervals is bounded by
\(
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{a_i,f_i}\right|\right]
+
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{f_i,a_i}\right|\right].
\)
 
  
Moreover, to establish inequality~(c), we bound
\begin{align*}
\mathbb{E}\!\Bigg[
\sum_{j \in [|\mathcal{K}|]}
\bigl(t_{j+1}-1-t'_j\bigr)
\;\Bigg|\;
t'_j \in \Bar{\mathcal{G}}_{i-1}
\Bigg]
&\le
\mathbb{E}\!\Bigg[
\sum_{j \in [|\mathcal{K}|]}
\bigl(t_{j+1}-1-t'_j\bigr)
\;\Bigg|\;
\FM_{a_{i-1}}(t'_j) \neq f_{i-1}
\;\land\;
t'_j \in \mathcal{G}_{i-2}
\Bigg] \\
&\quad\quad\qquad+
\mathbb{E}\!\Bigg[
\sum_{j \in [|\mathcal{K}|]}
\bigl(t_{j+1}-1-t'_j\bigr)
\;\Bigg|\;
t'_j \in \Bar{\mathcal{G}}_{i-2}
\Bigg], \\
&\le
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{a_{i-1},f_{i-1}}\right|\right]
+
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{f_{i-1},a_{i-1}}\right|\right] +
\mathbb{E}\!\Bigg[
\sum_{j \in [|\mathcal{K}|]}
\bigl(t_{j+1}-1-t'_j\bigr)
\;\Bigg|\;
t'_j \in \Bar{\mathcal{G}}_{i-2}
\Bigg], \\
&\vdots\\
&\le\sum_{j=1}^{i-1}
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{a_j,f_j}\right|\right]
+
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{f_j,a_j}\right|\right],
\end{align*}
where each step is followed with the same rationale we had to achieve inequality (b).




Finally, applying Lemmas~\ref{lemma:valid-rr} on inequalities~\eqref{ineq:finalalphadec},~\cref{ineq:update-regret}, and~\cref{lemma:alphadec} the total regret is bounded as
        {\small
            \begin{align*}
                \mathbb{E}\!\left[R_{a_i}(T)\right]&\leq \left(3n^2+1\right)\cdot \left( \sum_{a_j\in\AG}
\frac{4m \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{a_j})^2}{2m}\right)}{1 - \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{a_j})^2}{2m}\right)}
+
\sum_{f_j\in\FI}
\frac{4n \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{f_j})^2}{2m}\right)}{1 - \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{f_j})^2}{2m}\right)}\right)\\
&\quad +
               \left( \sum_{j=1}^i
\frac{4\left|\mathcal{L}_{a_j,f_j}\right| \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{a_j})^2}{2m}\right)}{1 - \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{a_j})^2}{2m}\right)}
+
\frac{4n \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{f_i})^2}{2m}\right)}{1 - \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{f_i})^2}{2m}\right)}\right) \in O\left(n^3m^2+ m\cdot\left(
\sum_{j=1}^{i}
\left|\mathcal{L}_{a_j,f_j}\right|
+
\left|\mathcal{L}_{f_j,a_j}\right|\right)\right)
            \end{align*}
        }
\end{proof}







\subsection{Extension of Algorithm~\ref{alg:drr}'s Analysis to General Markets} \label{sec:deccoordgen}
We extend the results established for $\alpha$-reducible markets in the main body to general, unstructured matching markets, where no structural assumptions are imposed and multiple stable matchings may exist.


\subsubsection{\textbf{An Upper Bound on the Expected Number of Updating Stages}}
We first extend \cref{lemma:alphadec} to general matching markets in order to bound the expected number of updating stages. In the absence of structural assumptions, this bound becomes market-independent and necessarily larger than in the $\alpha$-reducible case.

\begin{restatable}{lemma}{lemmadec}\label{lemma:dec}
In a matching market $\MM$, with strategic firms following~\cref{alg:fdrr} and agents following~\cref{alg:drr}, the total number of distributed runs of $\FGS$ (i.e., the number of updating phases) is time-independent
and of $O(n^2m^2)$.
\end{restatable}

\begin{proof}
In a general matching market $\MM$, as introduced earlier, we denote the agent-optimal and agent-pessimal stable matches of agent $a \in \AG$ by $\overline{f^*_a}$ and $\underline{f^*_a}$, respectively. By the lattice structure of stable matchings, the agent-optimal stable matching coincides with the firm-pessimal one: in particular, if $\overline{f^*_a}=f$, then $\underline{a^*_f}=a$, and if $\underline{f^*_a}=f$, then $\overline{a^*_f}=a$.

Before proceeding to the proofs, we introduce the event
\(
\psi_{\mathcal{F}} \doteq \psi^{(1)}_{\mathcal{F}} \cap \psi^{(2)}_{\mathcal{F}}.
\)
We first define
\begin{align*}
\psi^{(1)}_{\FI}
&\doteq
\left\{
t \in [T] :
\forall f \in \FI,\;
t \in \bigcap_{a \in \mathcal{L}_{f,\overline{a^*_f}}}
\mathcal{E}_{f,a}
\right\},\\[4pt]
\psi^{(2)}_{\FI}
&\doteq
\left\{
t \in [T] :
\forall f \in \mathcal{F},\;
\Bigl(
t \in \mathcal{E}_{f,\overline{a^*_f}}
\ \land\
\forall a \in \mathcal{H}_{f,\overline{a^*_f}},\;
a \in \hat{\mathcal{H}}_{f,\overline{a^*_f}}(t)
\Bigr)
\right\}.
\end{align*}


accordingly, $\psi_{\mathcal{\FI}}$ is the set of time steps at which, for every firm \( f \in \mathcal{\FI} \), the estimated preference list of \( f \) correctly orders all agents that are strictly less preferred than its agent-optimal match \( \overline{a^*_f} \) and all the agents which are strictly preferred tp \( \overline{a^*_f} \) are ranked higher but not ordered.

We also define the event $\zeta_{\AG}$ as
\begin{align*}
\zeta_{\AG}
\doteq
\left\{
t \in [T] :
\forall a \in \AG,\;
t \in
\bigcap_{f \in \{\underline{f^*_a}\} \cup \mathcal{H}_{a,\underline{f^*_a}}}
\mathcal{E}_{a,f}
\right\}.
\end{align*}
That is, $\zeta_{\AG}$ is the set of time steps at which, for every agent $a$, the estimated preference list correctly orders its agent-pessimal stable match $\underline{f^*_a}$ and all firms strictly preferred to it, according to the ground-truth preferences.

We also define $\TGS(t)$ as the initial time step of the most recent updating stage by time $t$.



We now follow the proof using~\cref{obs:drr2} that the expected number of updating phases is bounded by
\(
\mathbb{E}\!\left[\left|\bigcup_{a_i\in \AG}\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i} \right|\right].
\)
Thus we write
\begin{align*}
\mathbb{E}\!\left[\left|\bigcup_{a_i\in \AG}\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i} \right|\right]
&=
\mathbb{E}\!\left[\sum_{t=1}^T\mathbb{1}\left\{t \in \bigcup_{a_i\in \AG}\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i} \right\}\right],\\
&\leq
\mathbb{E}\!\left[\sum_{t=1}^T\mathbb{1}\left\{t \in \bigcup_{a_i\in \AG}\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i} \land \exists t' \in[\TGS(t),t-1], t' \in \Bar{\psi}_\FI \cup \Bar{\zeta}_{\AG} \right\}\right] +\\
&\qquad\quad\mathbb{E}\!\left[\sum_{t=1}^T\mathbb{1}\left\{t \in \bigcup_{a_i\in \AG}\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i} \land \forall t' \in[\TGS(t),t-1], t' \in \psi_\FI \cap \zeta_{\AG} \right\}\right],\\
&\overset{(a)}\leq \mathbb{E}\!\left[\sum_{t=1}^T\mathbb{1}\left\{ \exists t' \in[\TGS(t),t-1], t' \in \Bar{\psi}_\FI \cup \Bar{\zeta}_{\AG} \right\}\right] + \mathbb{E}\!\left[\sum_{t=1}^T\mathbb{1}\left\{t \in \bigcup_{a_i\in \AG}\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i} \land t \in \Bar{\psi}_\FI \cup \Bar{\zeta}_{\AG} \right\}\right],\\
&\overset{(b)}\leq\mathbb{E}\!\left[\left|\Bar{\psi}_\FI \cup \Bar{\zeta}_{\AG}\right|\right].
\end{align*}
Inequality~(a) follows by a case analysis.

(i) If there exists a time step $t' \in [\TGS(t),t-1]$ such that
$t' \in \Bar{\psi}_\FI \cup \Bar{\zeta}_{\AG}$, then the updating phase initiated at $\TGS(t)$
is charged to this violation.

(ii) Otherwise, for all $t' \in [\TGS(t), t-1]$ we have
$t' \in \psi_\FI \cap \zeta_{\AG}$.
In this case, throughout the updating phase starting at $\TGS(t)$,
all firms have valid estimated preference lists with respect to their
agent-optimal matches $\overline{a^*_f}$, and all agents have valid
estimated preference lists with respect to their agent-pessimal matches
$\underline{f^*_a}$.
Consequently, the matching $(a,\underline{f^*_a})_{\forall a \in \AG}$
remains stable with respect to the estimated preferences at all time steps
in $[\TGS(t), t-1]$, and no switching condition can be triggered.

Moreover, since the distributed $\FGS$ run by the agents returns the
agent-optimal (and firm-pessimal) stable matching under the current
estimated preferences, it follows that for every agent $a \in \AG$,
$\FA_a(t)$ is ranked no worse than $\underline{f^*_a}$ under $\EPL_a(t)$,
and for every firm $f \in \FI$, the agent matched to $f$ is ranked no better
than $\overline{a^*_f}$ under $\EPL_f(t)$.

Therefore, any switching event at time $t$ must correspond to a violation
of either $\zeta_{\AG}$ or $\psi_\FI$:
\begin{itemize}
    \item If $t \in \mathcal{S}^{\mathrm{inc}}_a$ for some agent $a$, then $a$ detects a
    preference invalidity with respect to some
    $f \in \mathcal{H}_{a,\underline{f^*_a}}$, implying that
    $t \in \Bar{\zeta}_{\AG}$.
    \item If $t \in \mathcal{S}^{\mathrm{rej}}_a$ for some agent $a$, then the firm
    $f=\FA_a(t)$ performs a strategic rejection because its estimated
    preference list becomes invalid with respect to some
    $a' \in \mathcal{L}_{f,\overline{a^*_f}}$, implying that
    $t \in \Bar{\psi}_{\FI}$.
\end{itemize}



Inequality~(b) then follows since each updating phase can be uniquely associated with a time
step in $\Bar{\psi}_\FI \cup \Bar{\zeta}_{\AG}$, and such violations are counted at most once.

We complete the proof by bounding the two terms in
\[
\mathbb{E}\!\left[\left|\Bar{\psi}_\FI \cup \Bar{\zeta}_{\AG}\right|\right]
\;\le\;
\mathbb{E}\!\left[\left|\Bar{\zeta}_{\AG}\right|\right]
+
\mathbb{E}\!\left[\left|\Bar{\psi}_\FI\right|\right]
\]
separately.

To bound $\mathbb{E}\!\left[\left|\Bar{\zeta}_{\AG}\right|\right]$, we write
\begin{align}
 \mathbb{E}\!\left[\left| \Bar{\zeta}_{\AG}\right|\right]
 &= \mathbb{E}\!\left[\left|
 \left\{t \in [T]:
 \exists a \in \AG,\;
 \exists f \in \{\underline{f^*_a}\} \cup \mathcal{H}_{a,\underline{f^*_a}},
 \ t \in \Bar{\mathcal{E}}_{a,f}
 \right\}
 \right|\right],\nonumber\\
 &\leq
 \sum_{a\in \AG}
 \sum_{f \in \{\underline{f^*_a}\} \cup \mathcal{H}_{a,\underline{f^*_a}}}
 \mathbb{E}\!\left[\left| \Bar{\mathcal{E}}_{a,f}\right|\right],\nonumber\\
 &\leq
 \sum_{a\in \AG}
 \sum_{f \in \{\underline{f^*_a}\} \cup \mathcal{H}_{a,\underline{f^*_a}}}
 \frac{4|\mathcal{L}_{a,f}|
 \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{a,f})^2}{2m}\right)}
 {1 - \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{a,f})^2}{2m}\right)},
 \label{ineq:zeta}\\
 &\in
 \sum_{a\in \AG}
 \sum_{f \in \{\underline{f^*_a}\} \cup \mathcal{H}_{a,\underline{f^*_a}}}
 O\!\left(m\cdot|\mathcal{L}_{a,f}|\right)
 \;\in\; O(n^2m^2),\nonumber
\end{align}
where the final bound follows from~\cref{lemma:valid-rr}.

For $\mathbb{E}\!\left[\left|\Bar{\psi}_\FI\right|\right]$, we then write
\begin{align}
   \mathbb{E}\!\left[\left|\Bar{\psi}_\FI\right|\right]
   &= \mathbb{E}\!\left[\left|\Bar{\psi}^{(1)}_\FI \cup \Bar{\psi}^{(2)}_\FI\right|\right],\nonumber\\
   &\leq
   \mathbb{E}\!\left[\left|\Bar{\psi}^{(1)}_\FI\right|\right]
   +
   \mathbb{E}\!\left[\left|\Bar{\psi}^{(2)}_\FI\right|\right],\nonumber\\
   &\leq
   \mathbb{E}\!\left[\left|\Bar{\psi}^{(1)}_\FI\right|\right]
   +
   \mathbb{E}\!\left[
   \left|
   \left\{t \in [T]:
   \exists f \in \FI,\;
   t \in \Bar{\mathcal{E}}_{f,\overline{a^*_f}}
   \ \lor\
   \left(\exists a \in \mathcal{H}_{f,\overline{a^*_f}},
   \ a \in \hat{\mathcal{L}}_{f,\overline{a^*_f}}(t)\right)
   \right\}
   \right|
   \right],\nonumber\\
&\leq
\mathbb{E}\!\left[\left|\Bar{\psi}^{(1)}_\FI\right|\right]
+
\sum_{f \in \FI}\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{f,\overline{a^*_f}}\right|\right]
+
\mathbb{E}\!\left[
\left|
\left\{t \in [T]:
\exists a \in \mathcal{H}_{f,\overline{a^*_f}},
\ a \in \hat{\mathcal{L}}_{f,\overline{a^*_f}}(t)
\right\}
\right|
\right],\nonumber\\
   &\leq
   \sum_{f\in \FI}
   \sum_{a \in \mathcal{L}_{f,\overline{a^*_f}}}
   \frac{4|\mathcal{L}_{f,a}|
   \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{f,a})^2}{2m}\right)}
   {1 - \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{f,a})^2}{2m}\right)}
   +
   \frac{4n
   \exp\!\left(-\tfrac{(\overline{\Delta}^{\texttt{min}}_{f})^2}{2m}\right)}
   {1 - \exp\!\left(-\tfrac{(\overline{\Delta}^{\texttt{min}}_{f})^2}{2m}\right)},
   \label{ineq:psi}\\
   &\in
   \sum_{f\in \FI}
   \sum_{a \in \mathcal{L}_{f,\overline{a^*_f}}}
   O\!\left(m\cdot|\mathcal{L}_{f,a}| + nm\right)
   \;\in\; O(n^2m^2),\nonumber
\end{align}
where the final bound follows by applying the same argument used to bound
$\mathbb{E}\!\left[\left|\Bar{\zeta}_{\AG}\right|\right]$ to
$\mathbb{E}\!\left[\left|\Bar{\psi}^{(1)}_\FI\right|\right]$,
and then invoking~\cref{lemma:valid-rr} for the remaining term.
Finally, we got
{\small
\begin{align*}
    \mathbb{E}\!\left[\left|\bigcup_{a_i\in \AG}\mathcal{S}^{\mathrm{inc}}_{a_i}\cup \mathcal{S}^{\mathrm{rej}}_{a_i} \right|\right] \leq \sum_{a\in \AG}
 \sum_{f \in \{\underline{f^*_a}\} \cup \mathcal{H}_{a,\underline{f^*_a}}}
 \frac{4|\mathcal{L}_{a,f}|
 \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{a,f})^2}{2m}\right)}
 {1 - \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{a,f})^2}{2m}\right)} + \sum_{f\in \FI}
   \sum_{a \in \mathcal{L}_{f,\overline{a^*_f}}}
   \frac{4|\mathcal{L}_{f,a}|
   \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{f,a})^2}{2m}\right)}
   {1 - \exp\!\left(-\tfrac{(\Delta^{\texttt{min}}_{f,a})^2}{2m}\right)}
   +
   \frac{4n
   \exp\!\left(-\tfrac{(\overline{\Delta}^{\texttt{min}}_{f})^2}{2m}\right)}
   {1 - \exp\!\left(-\tfrac{(\overline{\Delta}^{\texttt{min}}_{f})^2}{2m}\right)},
\end{align*}
which is of $O(n^2m^2)$.
}
\end{proof}
\subsubsection{\textbf{Proof of Convergence to a Stable Matching}}

We outline here the key convergence argument and discuss the impossibility of guaranteeing convergence to the agent-optimal stable matching.

\begin{proposition}\label{prop:coopgenmarket}
In a matching market $\MM$, where agents follow Algorithm~\ref{alg:drr} and strategic firms follow Algorithm~\ref{alg:fdrr}, the algorithms converge to a stable matching, which is not necessarily agent-optimal.
\end{proposition}

\begin{proof}
By Definition~\ref{def:convergence}, convergence implies the existence of a time $t$ such that
$\FM_a(t') = \FM_a(t'-1)$ for all $t' > t$ and all agents $a$.
Let $t_1$ denote the start of the final committing phase.
By Observation~\ref{obs:drr1}, agents commit to a perfect matching
$(a,\FA_a(t_1))_{\forall a \in \AG}$ throughout $[t_1,T]$.

Since no switching condition is triggered after $t_1$, no agent detects a preference-list inconsistency and no firm performs a strategic rejection.
Consequently, each agent $a$ has already been rejected by every firm in
$\hat{\mathcal{H}}_{a,\FA_a(t_1)}(t_1)$, and each firm $f$ is matched with its most preferred agent among those who applied during the final updating phase.

Therefore, no blocking pair exists, and the matching
$(a,\FA_a(t_1))_{\forall a \in \AG}$ is stable.
Finally, as illustrated in Example~\ref{examp:coordfgs}, the limiting stable matching need not be agent-optimal.
\end{proof}

\subsubsection{\textbf{Crucial Observations}}
We now present two crucial observations that will be used repeatedly in the proof of~\cref{thm:decreg}.




The following observations clarify how the set of top-$n$ firms constrains stable outcomes in general markets.

\begin{observation}\label{obs:gmarket1}
In any matching market $\MM$, for every agent $a \in \AG$, the agent-optimal stable match
$\overline{f^*_a}$ belongs to the set of top-$n$ firms $\FI^{(n)}_a$. Formally,
\[
\overline{f^*_a} \in \FI^{(n)}_a.
\]
\end{observation}

\begin{proof}
Running $\FGS$ on the ground-truth preference lists yields the agent-optimal stable matching.
Since there are $n$ agents, each agent can be rejected at most $n-1$ times during the execution
of $\FGS$. Therefore, the agent-optimal stable match of any agent must lie among its top $n$
ranked firms, that is, in $\FI^{(n)}_a$.
\end{proof}

\begin{observation}\label{obs:gmarket2}
In any matching market $\MM$, if for some agent $a \in \AG$ the agent-pessimal stable match
$\underline{f^*_a}$ does not belong to the set $\FI^{(n)}_a$, that is,
\(
\underline{f^*_a} \notin \FI^{(n)}_a,
\)
then the market admits more than one stable matching. Equivalently,
\(
\underline{f^*_a} \neq \overline{f^*_a}.
\)
\end{observation}

\begin{proof}
If $\underline{f^*_a} \notin \FI^{(n)}_a$ while $\overline{f^*_a} \in \FI^{(n)}_a$ by
Observation~\ref{obs:gmarket1}, then the agent-optimal and agent-pessimal stable matches of $a$
must be distinct. Hence, the market admits more than one stable matching.
\end{proof}



\begin{observation}\label{obs:topnescorrect}
In a matching market $\MM$ with strategic firms following~\cref{alg:fdrr} and agents following~\cref{alg:drr}, consider any updating stage starting at time $\TGS$, and let
\(
t' \doteq \TGS + 3n^2 + 1
\)
denote the start of the subsequent committing phase. Then, in the perfect matching
$(a,\FM_a(t'))_{\forall a \in \AG}$ to which agents commit, each agent $a$ is matched to a firm
$\FM_a(t')$ that belongs to its top-$n$ estimated firms at time $\TGS$, i.e.,
\[
\FM_a(t') \in \hat{\FI}^{(n)}_a(\TGS).
\]
\end{observation}


\begin{proof}
The key observation is that,
throughout the updating stage, agents select their actions based on the estimated preference
lists fixed at time $\TGS$. As a result, during the ensuing distributed execution of $\FGS$,
each agent applies only to firms among its top-$n$ estimated choices at time $\TGS$, which
implies the claim.
\end{proof}

Now we conclude this section with the following lemma, which plays a crucial role in the proof of~\cref{thm:decreg}.

\begin{lemma}\label{lemma:sortedcommit}
In a matching market $\MM$ with strategic firms following~\cref{alg:fdrr} and agents following~\cref{alg:drr}, consider any updating stage starting at time $\TGS$, and let
\(
t' \doteq \TGS + 3n^2 + 1
\)
denote the start of the subsequent committing phase. Suppose that the perfect matching
$(a,\FM_a(t'))_{\forall a \in \AG}$ to which agents commit is not stable with respect to the ground-truth preferences.
If there exists a time step $t'' \ge t'$ during the committing phase such that
\[
t'' \in \Gamma^{(n)}_\AG \cap \Gamma^{(n)}_\FI,
\]
then agents initiate the next updating phase at time $t''+1$.
\end{lemma}


\begin{proof}
The claim follows from~\cref{obs:topnescorrect} together with the~\cref{def:globaltopkalign} of
$\Gamma^{(n)}_\AG$ and $\Gamma^{(n)}_\FI$.

Since the perfect matching $(a,\FM_a(t'))_{\forall a \in \AG}$ is not stable with
respect to the ground-truth preferences, there must exist at least one agent or
firm whose top-$n$ estimated preference list was not aligned with the ground truth
(either elementwise or orderwise) during the updating phase starting at $\TGS$.
Equivalently, there exists a time step
\(
t_1 \in [\TGS,\TGS+3n^2]
\)
such that
\(
t_1 \notin \Gamma^{(n)}_\AG \cap \Gamma^{(n)}_\FI.
\)

We now show that this misalignment either persists throughout the entire committing
phase or persists up to exactly one round before its end, that is, until time
$t''-1$. Specifically, the violation persists throughout the committing phase until the
first time step $t''$ such that
\(
t'' \in \Gamma^{(n)}_\AG \cap \Gamma^{(n)}_\FI,
\)
at which point it is detected and necessarily triggers a switching (signaling)
event that initiates a new updating phase in the subsequent round, namely at time
$t''+1$.



Now consider the committing phase, and let $t'' \ge t'$ be the first time step such
that
\(
t'' \in \Gamma^{(n)}_\AG \cap \Gamma^{(n)}_\FI.
\)
If no such time step exists, then the entire committing phase is contained in
$\Gamma^{(n)}_\AG \cap \Gamma^{(n)}_\FI$.

At time $t''$, all agents’ top-$n$ estimated firms and all firms’ estimated
preference lists coincide with the ground truth. However, the matching
$(a,\FM_a(t'))_{\forall a \in \AG}$ remains unchanged throughout the committing
phase and is assumed to be unstable with respect to the ground-truth preferences,
and hence also unstable with respect to the estimated preferences at time $t''$.
Therefore, a blocking pair must exist.

Let $\langle a_i, \FM_{a_j} \rangle$ be such a blocking pair under the ground-truth
preferences. By definition of a blocking pair, we have
\(
\FM_{a_j}(t') \underset{\PL_{a_i}}{>} \FM_{a_i}(t')
\quad\text{and}\quad
a_i \underset{\PL_{\FM_{a_j}(t')}}{>} a_j.
\)

We now consider the following cases.

\paragraph{(i)}
If $\FM_{a_i}(t') \notin \FI^{(n)}_{a_i}$, then since at time $t''$ we have
\(
\FI^{(n)}_{a_i} = \hat{\FI}^{(n)}_{a_i}(t'')
\)
both elementwise and orderwise, it follows that
\(
\FM_{a_i}(t') \notin \hat{\FI}^{(n)}_{a_i}(t'').
\)
This constitutes a preference-list inconsistency for agent $a_i$, and therefore
\(
t'' \in \mathcal{S}^{\mathrm{inc}}_{a_i}.
\)

\paragraph{(ii)}
If $\FM_{a_i}(t') \in \FI^{(n)}_{a_i}$ and agent $a_i$ did not apply to
$\FM_{a_j}$ during the previous updating phase, then necessarily
\(
\FM_{a_j}(\TGS) \underset{\PL_{a_i}}{<} \FM_{a_i}(\TGS).
\)
At time $t''$, since the top-$n$ estimated firms are fully aligned with the ground
truth, this ordering reverses to
\(
\FM_{a_j}(t'') \underset{\PL_{a_i}}{>} \FM_{a_i}(t''),
\)
which again induces a preference-list inconsistency for agent $a_i$ and implies
\(
t'' \in \mathcal{S}^{\mathrm{inc}}_{a_i}.
\)

\paragraph{(iii)}
If $\FM_{a_i}(t') \in \FI^{(n)}_{a_i}$ and agent $a_i$ did apply to
$\FM_{a_j}$ during the previous updating phase but was rejected, then necessarily
\(
\FM_{a_j}(\TGS) \underset{\PL_{a_i}}{>} \FM_{a_i}(\TGS),
\)
which is consistent with both the ground-truth preferences and the estimated
preferences at time $t''$. However, $\FM_{a_j}(t')$ must have rejected $a_i$ at some earlier time
$t'''$ due to a preference-list inconsistency, being matched instead with its
current match $a_j$. This implies
\(
a_i \underset{\PL_{\FM_{a_j}(t''')}}{<} a_j.
\)
At time $t''$, the estimated preference list of firm $\FM_{a_j}(t'')$ becomes fully
aligned with the ground truth, which now satisfies
\(
a_i \underset{\PL_{\FM_{a_j}(t'')}}{>} a_j.
\)
By definition, this triggers a firm-side strategic rejection by $\FM_{a_j}$, and
hence
\(
t'' \in \mathcal{S}^{\mathrm{rej}}_{a_j}.
\)

In all cases, a switching condition is triggered at time $t''$, and therefore
$t''+1$ is the first round of the next updating phase.


Since preferences are now correctly estimated at time $t''$, this blocking pair
is also detected under the estimated preference lists, which triggers a switching
condition for either agent $a_i$ or firm $f_j$.
Consequently, agents coordinate to initiate a new updating phase in the next round,
that is, at time $t''+1$. 
\end{proof}

\subsubsection{\textbf{Proof of~\cref{thm:decreg}}}\label{proof:decreg}
\thmdecreg*
\begin{proof}

We bound the pessimal regret $\mathbb{E}\!\left[\underline{R}_{a}(T)\right]$
by decomposing it into regret incurred during the updating and committing phases
and bounding each term separately:
\begin{align*}
\mathbb{E}\!\left[\underline{R}_{a}(T)\right]
=
\mathbb{E}\!\left[\underline{R}_{a}(\mathcal{U})\right]
+
\mathbb{E}\!\left[\underline{R}_{a}(\mathcal{C})\right].
\end{align*}

For $\mathbb{E}\!\left[\underline{R}_{a}(\mathcal{U})\right]$, we write:
\begin{align}
\mathbb{E}\!\left[\underline{R}_{a}(\mathcal{U})\right] =\sum_{t \in \mathcal{U}}
\left(
u_{a,\underline{f^*_a}}
-
\mathbb{E}[X_{a,\FM_{a}(t)}]
\right)
&\le
3n^2 \cdot\,
\mathbb{E}\!\left[
\left|
\bigcup_{a' \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_{a'}\cup \mathcal{S}^{\mathrm{rej}}_{a'}
\right)
\right|
\right].
\label{ineq:genupdate-regret}
\end{align}
Before bounding the committing regret, we introduce the following notation.
Let
\[
\bigcup_{a \in \AG} \left(\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a\right)
= \{t_1,t_2,\ldots\}
\]
denote the set of switching times, ordered increasingly.
The $j$-th committing phase is defined as the interval
\[
[t'_j : t_{j+1}],
\qquad
\text{where } t'_j \doteq t_j + 3n^2 + 1,
\]
which corresponds to the period between the $j$-th and $(j+1)$-th distributed executions of $\FGS$.
Accordingly, the collection of committing intervals is
\[
\mathcal{K}
\doteq
\left\{
[t'_j,\, t_{j+1}] :
j \in \left[\left|\!\bigcup_{a \in \AG}(\mathcal{S}^{\mathrm{inc}}_a \cup \mathcal{S}^{\mathrm{rej}}_a)\right|-1\right]
\right\}.
\]

Now for the committing regret we write 

{\small\begin{align}
\mathbb{E}\!\left[\underline{R_{a}}(\mathcal{C})\right]
&= \sum_{t \in \mathcal{C}}
\left(
u_{a,\underline{f^*_a}}
-
\mathbb{E}[X_{a,\FM_{a}(t)}]
\right) \nonumber\\
&=
\mathbb{E}\!\left[
\sum_{j=1}^{|\mathcal{K}|}
\sum_{t \in [t'_j,\, t_{j+1}]}
\Big(
u_{a,f}
-
X_{a,\FM_{a}(t'_j)}(t)
\Big) 
\right],\nonumber\\
&\overset{(a)}{\le} \mathbb{E}\!\left[
\left|
\bigcup_{a' \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_{a'} \cup \mathcal{S}^{\mathrm{rej}}_{a'}
\right)
\right|
\right] +
\mathbb{E}\!\left[
\sum_{j \in [|\mathcal{K}|]}
\bigl(t_{j+1}-1-t'_j\bigr)
\;\middle|\;
\FM_{a}(t'_j) \in \mathcal{L}_{a,\underline{f^*_a}}
 \land (a'',\FM_{a''}(t'_j))_{\forall a'' \in \AG} \text{ is not stable }\right],  \nonumber\\
&\overset{(b)}{\le}
\mathbb{E}\!\left[
\left|
\bigcup_{a' \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_{a'} \cup \mathcal{S}^{\mathrm{rej}}_{a'}
\right)
\right|
\right]+
\mathbb{E}\!\left[\left|\Bar{\Gamma}^{(n)}_{\AG} \cup \Bar{\Gamma}_{\FI}^{(n)}\right|\right],\label{ineq:finaldec}
\end{align}
}
The inequality~(a) is obtained by separating, within each committing phase, the single
\emph{signaling round} during which an agent intentionally abstains from applying in order
to signal a switching condition. Each committing phase contributes at most one such round,
and therefore the total number of signaling rounds is bounded by
\(
\mathbb{E}\!\left[
\left|
\bigcup_{a' \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_{a'} \cup \mathcal{S}^{\mathrm{rej}}_{a'}
\right)
\right|
\right].
\)
The second term captures the expected regret accumulated during the remaining rounds of
each committing phase. Since we analyze the \emph{pessimal regret} of agent~$a$, regret is
incurred only when $a$ is matched to a firm that it strictly prefers less than its
pessimal stable match $\underline{f^*_a}$.
Equivalently, regret is incurred only when
\(
\FM_a(t'_j) \in \mathcal{L}_{a,\underline{f^*_a}}.
\) In this case, the perfect matching reached at the end of the most recent updating stage, $(a'',\FM_{a''}(t'_j))_{\forall a'' \in \AG}$,
is necessarily unstable, as agent~$a$ is matched to a suboptimal firm. This observation
justifies conditioning the second term in~(a) on the instability of the matching.

Inequality~(b) follows from~\cref{lemma:sortedcommit}, since the matching
\((a'', \FM_{a''}(t'_j))_{\forall a'' \in \AG}\) is unstable.
Specifically, consider the committing interval \([t'_j,\, t_{j+1}]\).
If every time step in this interval belongs to
\(\Bar{\Gamma}_{\AG} \cup \Bar{\Gamma}_{\FI}\),
then the entire interval is charged to the second term of
inequality~\cref{ineq:finaldec}, while the signaling round is accounted for
separately in the first term.
Otherwise, there exists a time step
\(t'' \in [t'_j,\, t_{j+1}]\) such that
\(t'' \in \Gamma_{\AG} \cap \Gamma_{\FI}\).
By~\cref{lemma:sortedcommit}, this time step must be the signaling round $t_{j+1}$ that
triggers the next updating phase, and hence it is counted in the first term of
inequality~\cref{ineq:finaldec}.

The first term of~\cref{ineq:finaldec},
\[
\mathbb{E}\!\left[
\left|
\bigcup_{a' \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_{a'} \cup \mathcal{S}^{\mathrm{rej}}_{a'}
\right)
\right|
\right],
\]
is bounded by~\cref{lemma:dec}. We therefore bound the remaining term
\(\mathbb{E}\!\left[\left|\Bar{\Gamma}_{\AG} \cup \Bar{\Gamma}_{\FI}\right|\right]\)
as follows:
\begin{align}
\mathbb{E}\!\left[\left|\Bar{\Gamma}^{(n)}_{\AG} \cup \Bar{\Gamma}_{\FI}^{(n)}\right|\right]
\le
\mathbb{E}\!\left[\left|\Bar{\Gamma}_{\AG}^{(n)}\right|\right]
+
\mathbb{E}\!\left[\left|\Bar{\Gamma}_{\FI}^{(n)}\right|\right] 
\le
\sum_{a' \in \AG}
\sum_{f' \in \FI^{(n)}_{a'}}
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{a',f'}\right|\right]
+
\sum_{f'' \in \FI}
\sum_{a'' \in \AG}
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{f'',a''}\right|\right]. \label{eq:deccomitreg}
\end{align}
The final inequality follows by expanding the definitions of
\(\Bar{\Gamma}_{\AG}\) and \(\Bar{\Gamma}_{\FI}\) and applying a union bound over
the corresponding agents and firms.

Thus, with respect to Inequalities~\eqref{ineq:genupdate-regret} and~\eqref{eq:deccomitreg} and the regret decompisition we considered at the beginning we can write

\begin{align*}
\mathbb{E}\!\left[\underline{R}_{a}(T)\right]
&=
\mathbb{E}\!\left[\underline{R}_{a}(\mathcal{U})\right]
+
\mathbb{E}\!\left[\underline{R}_{a}(\mathcal{C})\right],\\ &\overset{(a)}\leq \left(3n^2+1\right)\cdot\mathbb{E}\!\left[
\left|
\bigcup_{a' \in \AG}
\left(
\mathcal{S}^{\mathrm{inc}}_{a'} \cup \mathcal{S}^{\mathrm{rej}}_{a'}
\right)
\right|
\right] + \sum_{a' \in \AG}
\sum_{f' \in \FI^{(n)}_{a'}}
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{a',f'}\right|\right]
+
\sum_{f'' \in \FI}
\sum_{a'' \in \AG}
\mathbb{E}\!\left[\left|\Bar{\mathcal{E}}_{f'',a''}\right|\right] \in O\left(n^4m^2\right)
\end{align*}
  
\end{proof}


==> interview.tex <==

\subsection{Extended $\ALLP$ and $\ALLP^{\hat{\mu}}$}   
In this section we present the extended version of the $\ALLP^{\hat{\mu}}$ under which the learner aims for learning the $i$th best arm instead of the best arm which is the case in the matching markets cause each agent there is individually looking to learn their fixed match which is probable to not be their most preferred one. Before, extending this to the multi-agent setup, we consider the case of a single agent who is seeking to learn their $i$th best arm. So the regret for such case is defined as 
\begin{align}
R^i_{a}(T) \coloneqq T u_{a,f^i_a} - \sum_{t=1}^T \min\left\{u_{a,f^i_a}, \mathbb{E}\left[\max\left\{ X_{a,f^i_a(t)}(t), X_{a,f^{i+1}_a(t)}(t)\right\}\right]\right\} \label{reg:eap}
\end{align}


\section{Matching-Markets with Interviews (Multi-Agent Bandits with Hints}
\subsection{Centralized $\UCB'$ Interview Allocation} \label{sec:cucbp}
After analyzing the $\EAP$ algorithm for a single learner, we extend its application to a multi-agent setting, where interview allocation is managed by a central platform. This section is inspired by the result in \cite{liu2020competing}. In this scenario, agents maintain and update their estimations using $\UCB'$, as defined in \eqref{cucbp:2}. At each time step $t$, the agents submit their sorted lists of $\UCB'$ estimations to the central platform, which is responsible for allocating $\intesize$ interviews (observations) to the agents which is assumed to be equal $3$ which replicates $\EAP$.


The centralized platform should allocate the interviews in such a way that the firms likely to hire $a$ appear in $I_a(t)$ while not allowing overqualified applicants appear in $I_a(t)$ that may block $a$ to find their stable match. Here, we propose an algorithm \emph{Centralized Interview Allocation} ($\CIAP$), which calls another subroutine \emph{Two-Stage $\FGS$ Interview Allocation} ($\TSGIA$), where two runs of $\FGS$ with elimination over the values of $\UCB'$ help the central platform determine the $f'_a$ and $f''_a$ to be in $I_a(t)$. The third firm to interview $f_{\text{rr}}$ is determined in round-robin manner. We now define a \emph{Good Observation}, under which the $f^*_a\in I_a(t)$ or the firms in $I_a(t)\setminus f_{\text{rr}}$ are preferred over $f^*_a$ according to the values of $\UCB'$s. For example, if agent $a$ submits $\EPL_a(t) = \langle f_1, f_2, f_3, \dots, f^*_a, \dots, f_{m} \rangle$, then the interview allocation $I_a(t)= \{f_1, f_2, f_{\text{rr}}\}$, $I_{f_1} = \{a\}$, and $I_{f_2} = \{a\}$ provides agent $a$ with a Good Observation. The more \emph{Good Observations} agents receive, the more the multi-agent setting resembles the single-agent setting, according to the important $\alpha$-reducibility assumption, which has been proven to result in a regret of $O(m^2)$ for each agent.


The  helps the Central Platform provide each agent with \emph{Good Observations} at most time steps. 

The pseudo-code below describes how agent $a$ interacts with the Centralized Interview Allocation ($\CIAP$) and the role the centralized platform plays in this process.

\begin{algorithm}[H]
\caption{ Centralized Interview Allocation $(\CIAP)$}\label{routin:cucbp}
\begin{algorithmic}[1]
\For{$ t \in  [T]$}
\State agent $a$ submits $\EPL_a(t)$ to the $\CIAP$
\State $\CIAP$ runs $\TSGIA$ over the \(\EPL_a(t)\)'s for all agent \(a\)  and returns $I_a(t)$s
\State agent $a$ observes $I_a(t)\doteq\{f'_a(t),f''_a(t),f_{\text{rr}}(t)\}$
\State agent $a$, interviews with $I_a(t)$ and updates the $\EPL_a(t+1)$.
\State agent $a$ submits the $\EPL_a(t+1)$ to the $\FGS$ and obtains the utility of the firm they get matched to.

\EndFor
\end{algorithmic}
\end{algorithm}



\subsubsection{Two-Stage $\FGS$  Interview Allocation ($\TSGIA$)}
Under $\TSGIA$ algorithm agents are interviewing with the firms that are likely to hire them. Thus, $\FGS$ run over the uncertain submitted $\EPL_a$s might be useful to help the agents interview with plausible firms during the learning process. As described in routine \ref{routin:cucbp}, $\CIAP$ is responsible to help the agents to attend interviews which increases their probability of getting hired. 
In this algorithm, the central platform runs one-to-many version of $\FGS$ over the submitted preference lists,lets assume that $f'_a(t)$ be the match of agent $a$ at the end of this step. Then the platform eliminates the $f'_a(t)$ from the preference list of each agent $a$ and runs the many-to-one version of $\FGS$ on the new preference lists and the result would be $f''_a(t)$ as the matched firm for some agents $a$.

The reason behind this approach is that one-to-one $\FGS$ to the one-to-many $\FGS$ is to make sure that acceptable ratio (preferably all) of agents gains \empty{"Good Observation"} in $\alpha$-\empty{reducible} markets. Here we present an example that shows why using many-to-one $\FGS$ for the interview allocation can help all agent's to observe \empty{"Good Observation"}s. Let's assume that at time step $t$ $$\EPL_{a_1}(t) = \langle f^*_{a_2}, f^*_{a_1},\dots\rangle \quad \EPL_{a_2}(t) = \langle f^*_{a_3}, f^*_{a_2}, f^*_{a_4},\dots\rangle$$
$$\PL_{f^*_{a_1}} = \langle a_1,\dots\rangle \quad \PL_{f^*_{a_2}} = \langle a_1,a_2,\dots\rangle\quad \PL_{f^*_{a_3}} = \langle a_2,\dots\rangle$$
Running $\TSGIA$ with two stages of one-to-one $\FGS$ would have $I_{a_1}(t) = \{f^*_{a_2}, f^*_{a_1},f_{\text{rr}}\}$ and $I_{a_2}(t) = \{f^*_{a_3}, f^*_{a_4},f_{\text{rr}}\}$ which means $a_1$ gains \empty{"Good Observation"}s but $a_2$ does not. However, if we allow the interview allocation be a one-to-many matching with the budget at least two for each firm then the interview allocation of $\TSGIA$ would be $I_{a_1}(t) = \{f^*_{a_2}, f^*_{a_1},f_{\text{rr}}\}$ and $I_{a_2}(t) = \{f^*_{a_3}, f^*_{a_2},f_{\text{rr}}\}$ which provides \empty{"Good Observation"}s for both. 

Now that we can make sure that the $\TSGIA$ with two stages of many-to-one can help the agents to get \empty{"Good Observation"}s more often but how to set the budgets? What about the result of the main one-to-one $\FGS$; In other words, does having good observations guarantee that the agents will be hired by that one firm they are looking for? The short answer to both questions is how we define regret and the structure of the underlying $\alpha$-\empty{reducible} market. 

\begin{itemize}
    \item ((Disjoint Interview Allocation))

    This approach of interview allocation allows the agents to have mutually disjoint interviewing sets $I_a(t)$. If we can guarantee that $\TSGIA$, that applies the Disjoint Interview Allocation approach, provides all agents with the  \empty{"Good Observation"}s then every agent would suffer from a constant regret. 
    Here the $\TSGIA$ would be like:
    \begin{algorithm}[H]
\caption{ $\TSGIA$ with disjoint interviews}\label{alg:TSGIA_DI}
\begin{algorithmic}[1]
\Require $\EPL_a(t)$ for all agents \(a\), $Ib(f) = 1$

\State $M_1 \leftarrow \FGS(\EPL)$
\State $\EPL_a' = \EPL_a \backslash M_1(a) \quad  \forall a \in \mathcal{A}$

\State $M_2 \leftarrow \FGS(\EPL')$
\State return $I_a(t) = \{M_1(a),M_2(a),f_{\text{rr}}\}$ to each agent \(a\)
\end{algorithmic}
\end{algorithm}

This algorithm allows us to let the notion of regret to remain as what is defined in \eqref{reg:eap}. However, the problem is that the result of running $\CIAP$ using this variation of $\TSGIA$ depends strongly on the structure of the market. To shed some light on the issue, based on what is mentioned in the corollary \ref{cor1:eap}, if the $f^*_{a}$ is the $i$-th preferred firm, having $M_1(a)\text{ and }M_2(a)$ located at any two indices in the interval $[1,i]$ the observation would be counted as a \empty{"Good Observation"}. So the portion of \empty{"Good Observation"}s an agent $a$ receives through time highly depends on where the fixed match of others are lying in their preference lists as well as how the preference list of the first looks like. The more similarity among the the preference lists, the more collisions pops up, and the less \empty{"Good Observation"}s the agents in the lower layers of $\alpha$-\empty{reducibility} would get.
\end{itemize}



==> intro-new-backup.tex <==
\section{Introduction} \label{sec:intro}


Two-sided matching markets~\citep{roth1992two} are one of the most fundamental models in economics and computer science, with wide applications ranging from labor markets~\cite{roth1984evolution} to school choice~\cite{abdulkadirouglu2003school} and dating platforms~\citep{hitsch2010matching}, etc.
A two-sided matching market consists of two sides, e.g., \(m\in\mathbb{N}^+\) firms and \(n\in\mathbb{N}^+\) workers (\(n\le m\)), where each side has preferences over the other side.
A matching of both sides is \emph{stable} if there is no worker-firm pair that would both prefer to match with each other rather than keep their current assignments~\cite{gale1962college}.
Recently, there has been a growing interest in bandit learning in two-sided matching markets~\cite{liu2020competing,maheshwari2022decentralized,liu2021bandit} \todo{citer another 5 papers here}, where agents (workers) do not know their preferences initially and need to learn them through repeated interactions with the market,
and the interactions provide \emph{stochastic} rewards that help agents learn their preferences over time.
This setting corresponds to many real-world markets where both sides have incomplete information about their preferences and need to learn them through repeated interactions with the market.

However, in many real-world markets, before making a commitment to a match, agents can often gather some preliminary information about their potential matches through low-cost interactions, such as interviews or meetings.
For example, consider a labor market consisting of \(n\) workers (e.g., job seekers) and \(m\) firms (e.g., employers) with \(n\le m\).
For one round of full interactions, each worker can first conduct interviews (e.g., site visits, phone screenings, etc.) with a subset of firms to gather information about their preferences.
Then, based on the interview results, each worker applies to one of the interviewed firms and gets hired only if they are the most preferred applicant of that firm.
Similar preliminary interaction stages also exist in many other problems: in dating markets, individuals may go on several dates before deciding to commit to a relationship;
in college admissions, students may attend open days or campus tours before submitting or confirming their applications.
While studied in the offline setting~\cite{lee2017interviewing,beyhaghi2021randomness}, the role of such preliminary interactions (called \emph{interview} hereafter) in the learning dynamics of two-sided matching markets~\citep{liu2020competing}\todo{cite more here as well} has been largely overlooked.

To study how interviews can facilitate learning in two-sided matching markets, this paper considers a setting where agents (workers) can conduct interviews with a subset of firms before making their application decisions.
Specifically, in each round \(t\), each agent (worker) \(a\) first chooses a subset of firms \(\mathcal S_{a,t}\) to interview, where \(|\mathcal S_{a,t}|\) is upper bounded by an integer \(k\) called the \emph{interview budget}.
Then, from the interviews, agent \(a\) receives \emph{stochastic} reward signals, drawn from an unknown distribution with mean \(\mu_{a,f}\) for each interviewed firm \(f\in\mathcal S_{a,t}\).
After receiving the interview results, agent \(a\) applies to one of the interviewed firms and gets hired only if they are the most preferred applicant of that firm, obtaining a stochastic reward drawn from an unknown distribution with mean \(\mu_{a,f}\).
The goal of all agents in the market is to learn a stable matching while minimizing their \emph{regret}, defined as the difference between the expected reward of the stable match and that of the agent's actual matches over \(T\in \mathbb{N}^+\) rounds.

While following prior works~\cite{liu2020competing,maheshwari2022decentralized,liu2021bandit} without accounting for the interview stage yields algorithms achieving a \(O(\log T)\) regret,
we aim to study \emph{can the interview stage help agents learn a stable matching more efficiently (i.e., with lower regrets)?}





\paragraph{Our Contributions.}
We start from the centralized setting (Section~\ref{sec:centralized}), where a central planner controls all agents and coordinates their actions.
\tdmark~add (1) algorithmic design ideas, (2) the regret bound, and (3) the proof techniques.

We then move to the decentralized setting (Section~\ref{sec:decentralized}), where each agent acts independently without a central planner.
Specifically, we consider two types of decentralizations: \tdmark


\paragraph{Related Works.}
\tdmark~One paragraph on bandit learning on two-sided matching markets.
At the end, highlight none of them consider the interview stage.

\tdmark~One paragraph on stable matching with interviews.
At the end, highlight none of them consider the learning dynamics.

\tdmark~One brief paragraph on online learning with hints or predictions. Just say our work can also be placed in this line of works, but we focus on the two-sided matching market setting.





==> intro-new-v2.tex <==

\section*{Introduction} \label{sec:intro}
Two-sided matching markets~\citep{roth1992two} are fundamental models in economics and computer science, with applications from labor markets~\citep{roth1984evolution} to school choice~\citep{abdulkadirouglu2003school}, and dating platforms~\citep{hitsch2010matching}. Such a market consists of two sides, e.g., \(m\in\mathbb{N}^+\) firms and \(n\in\mathbb{N}^+\) workers, each holding preferences over the other. A matching is \emph{stable} if no worker--firm pair would both prefer to match with each other rather than remain with their current assignments~\citep{gale1962college}. 

Recent work has studied \emph{bandit learning} in these markets~\citep{liu2020competing,maheshwari2022decentralized,liu2021bandit,kong2023player,ghosh2024competing}, where \textit{only} the workers initially lack knowledge of their preferences and must learn them along with achieving stability through repeated interactions by applying to different firms. Each interaction yields a \emph{stochastic} reward that reflects the hiring outcome—determined by the firm’s preferences, with no match implying no reward—gradually helping agents refine their own preferences over time.







In many real-world matching markets, participants can often obtain preliminary information about potential matches through low-cost interactions, such as \emph{interviews} or visits, before making application decisions. This framework naturally connects to recent work on \emph{bandit learning with hints}~\cite{bhaskara2022online,mirfakhar2025heterogeneous} and, more broadly, to \emph{algorithms with predictions} that leverage such information before taking actions~\cite{lykouris2021competitive}, as well as to the learning in markets' literature.
% \textcolor{red}{references?}\amcomment{we made references to such works in the previous par so i avoided re citing them to save some space}.  
However, the role of such pre-matching interviews, which can provide both sides with early impressions of potential \emph{rewards} from being matched, has been largely overlooked in existing studies on bandit learning in two-sided markets, motivating the work herein.

% \amedit{To look into another overlooked dimension in prior work,} 
We also consider environments where uncertainty exists on the firm side. Firms, like agents, may be \emph{uncertain} about their own preference lists (\emph{unknown a priori}). Such uncertainty can cause firms to misjudge or even reject high-quality applicants during interviews, making the pursuit of stable matchings, an inherently mutual objective, a two-sided learning problem. This setting requires firms to operate with a richer action space: rather than always hiring as in prior works, they may \emph{strategically} choose to remain unmatched when current applicants, though of high quality, are perceived as not meeting the desired standard. This flexibility makes the model more realistic and challenging and is essential for achieving learning stability, as uncertain firms influence the dynamics through their hiring decisions. Most existing studies assume firms know their preferences in advance; only one prior work~\cite{zhangbandit} considers uncertain, non-strategic (always hiring) firms and relies on strong coordination across agents and firms to achieve low regret.



For instance, in a labor market, a worker may first conduct \emph{interviews} (e.g., site visits or phone screenings, etc.) with a subset of firms to learn about their preferences, while firms simultaneously form impressions of the candidates. Based on these interactions, the worker applies to one of the interviewed firms and is hired only if the firm decides to hire and the worker is its most preferred applicant. In practice, however, firms may also \emph{strategically} choose to defer hiring when none of the interviewed candidates meet their desired standard. Similar pre-matching stages and firm-side \emph{strategic} behaviors arise in other contexts as well, such as dating markets, where individuals may go on several dates before committing, and in college admissions, where schools may defer decisions until final applications. Such preliminary stages have been explored in offline settings~\cite{lee2017interviewing,beyhaghi2021randomness}, yet their role in the \emph{learning dynamics} of two-sided matching markets has been largely overlooked. 



We model two-sided matching markets with interviews and uncertain firms. In each round \(t\), every agent \(a\) selects up to \(k\) firms, \(\INT_a(t)\), to interview. Through these interviews, both the agent and each firm \(f \in \INT_a(t)\) \emph{observe} stochastic reward signals drawn from unknown distributions with means \(\mu_{a,f}\) and \(\mu_{f,a}\), representing their expected utilities from matching with each other. The agent then applies to one of the interviewed firms and is hired only if it is the firm’s most preferred applicant, unless the firm decides to remain unmatched due to uncertainty about its preferences. When a match occurs, the agent and firm each \emph{receive} a stochastic reward drawn from the distributions with the same means \(\mu_{a,f}\) and \(\mu_{f,a}\). This setup captures the learning dynamics induced by interviews and uncertainty on both sides. 
% \textcolor{red}{this paragraph seems slightly overlapping with the contribution section}

The goal of each agent is to learn a stable matching while minimizing its \emph{regret}, defined as the difference between the expected reward of its stable match and the reward obtained over \(T \in \mathbb{N}^+\) rounds. Although we formally define and analyze regret only for agents, this remains appropriate even in the presence of \emph{uncertain} firms who, in the two-sided learning process, gradually learn their own preferences. Since stability is a mutual objective, convergence to a stable matching with bounded agent regret naturally yields analogous guarantees for firms. Notably, most prior works~\cite{liu2020competing,maheshwari2022decentralized,liu2021bandit} do not model pre-matching interviews or strategic uncertain firms, and their decentralized algorithms achieve only \(O(\log T)\) regret. 
% \textcolor{red}{more elaborations on $\log{T}$, e.g., what's the problem with it or just remove this and say sth like suboptimal.}

In contrast, we ask \emph{whether incorporating interviews can enable both sides to learn a stable matching more efficiently—as interviews reveal additional information—achieving lower regret and, crucially, doing so \emph{without} agent–firm coordination, even when firms may strategically choose not to hire due to uncertainty. } Addressing this question introduces several technical challenges:



% \todo{HB: I feel like we need to set the stage better before the challenges. And maybe we can make the bullets a bit shorter? Terminology that not been defined and is being used: collisions, committing to the learned stable match, uncertain estimations, learning a stable matching. \tdmark~Amirmahdi}
\noindent$\blacktriangleright$ \textit{Interviewing-induced limitations on decision-making:} Although the interview provides agents with more information to learn their preferences, it also constrains their final application decisions, since they can only apply to firms they have interviewed. This restriction on the agents' action space introduces significant difficulties in both algorithm design and analysis.

\noindent$\blacktriangleright$\textit{Regret minimization via interviews:}
Prior work on bandit learning with hints---including single-agent settings~\citep{wei2020taking,bhaskara2023bandit} and multi-agent hinted learning~\citep{mirfakhar2025heterogeneous}---does not address the two-sided structure of matching markets. Incorporating interview feedback as hints in this setting is substantially more challenging due to interdependent agent behavior, firms' uncertainty and strategic choices, and the need to preserve stability.


\noindent$\blacktriangleright$\textit{Agents’ coordination in decentralized learning:}
While an \emph{omniscient} central interview allocator can enforce compatible interview choices that preserve stability, the fully decentralized setting allows no firm–agent coordination. Agents act independently and must select interviews without knowing others’ choices, making it difficult to ensure that the interviewed subsets are mutually compatible for reaching the stable matching. This lack of coordination significantly increases the likelihood of collisions and the resulting regret.




\noindent$\blacktriangleright$ \textit{Incorporating firm uncertainty:}
While a central interview allocator can readily manage \emph{firm-side uncertainty}, handling it in fully decentralized settings becomes significantly more challenging, especially without firm–agent coordination. Under uncertain preferences, firms may mistakenly reject high-quality agents, causing those agents to ignore these firms in future rounds due to earlier rejections. 




 \noindent$\blacktriangleright$ \textit{Modeling strategic uncertain firms:}
The outer layer of complexity comes from the richer action space for uncertain firms, who may decide not to hire in certain rounds. As shown in Example~\ref{sec:strategic}, this behavior is necessary for designing decentralized algorithms. It therefore calls for a dedicated algorithm for such firms, one that neither prevents agents from learning a stable matching nor incurs high regret due to non-hiring, while remaining aligned with firms’ incentives toward learning stability.






\paragraph{Our Contributions.}
In this paper, we study both centralized and decentralized settings for learning stable matchings. In the centralized case, an omniscient interview allocator coordinates agents' actions. In the decentralized case, we design two algorithms under mild model assumptions: one where agents can coordinate their interviews and one that is fully coordination free. Across all settings, our algorithms incorporate firm uncertainty and achieve time-independent \(O(1)\) regret through adaptive interviewing. Below, we summarize our main contributions.



\noindent $\blacktriangleright$ We introduce a realistic model that incorporates \emph{strategic uncertain firms} (\autoref{sec:model}). These firms may choose to remain unmatched, preventing them from getting stuck with low quality matches caused by uncertain preferences and allowing them to adjust as their preferences evolve. This strategic flexibility is essential for learning stability in decentralized settings and mirrors offline insights showing that strategic firm behavior can meaningfully affect stable outcomes~\cite{kupfer2018influence}.


\amcomment{make the following smoother}
\noindent$\blacktriangleright$ In line with the bandit learning view of interviews as hints, all our algorithms employ two interviews per round, with one firm selected in a round-robin manner. \amcomment{by lemma X} We show that this design suffices to achieve time-independent regret\amcomment{or here (lemma)}. In contrast,~\citet{bhaskara2023bandit} conjectured that even in a single-agent setting, three hints per round (one chosen round-robin) were necessary for such guarantees. Our results demonstrate that, even in a far more complex multi-agent competitive environment with strategic uncertain firms, two hints per round are sufficient. Moreover, while~\citet{zhangbandit} used round-robin exploration in a similar model without interviews or strategic firms to achieve $O(\log T)$ regret, our findings extend this framework to the richer interview-based setting with stronger guarantees.


\noindent $\blacktriangleright$ We start with the centralized setting
(\autoref{sec:centralized}), where a central interview allocator (\texttt{CIA}) controls all agents and coordinates their actions. %\todo{HB: I think it'd be better not to use $\FGS$ in the introduction, or at least we should define it and cite them first. We can say something like ``We design a centralized algorithm based on the classic stable matching algorithm by Gale and Shapley \cite{ }, ...''}
We design a centralized $\FGS$-based algorithm~\cite{gale1962college} that, under both certain and uncertain firm setups, learns the agent-optimal stable matching in $O(nm)$ time. In this centralized framework, the interview allocator resolves potential collisions arising from uncertain preference lists, and agents do not reject decisions during learning. 

% \rev{Following~\cite{kupfer2018influence}, firms in such cases can strategically improve their utility; however, whether such strategic behavior remains beneficial when preferences are uncertain and evolving over time---without compromising stability---remains an interesting open question.}
% \mo{this looks out of context, not contribution, more like a concluding remark and future direction in conclusion section, instead of this, add more about alg itself, and say round-robin with 2 is enough to achieve whatever we are looking for.}

\noindent $\blacktriangleright$ Lastly, we move to the decentralized setting (\autoref{sec:decentralized}), where each agent acts independently without a central planner.  
A naive approach—where agents perform round-robin interviews until their preference lists are confidently sorted and reapply $\FGS$ after every order swap—would incur $O(m^2n^3)$ regret, exceeding the centralized bound of $O(mn)$ by an extra factor of $m$, given the inherent $O(n^2)$ cost of distributed $\FGS$.  
To address this, we introduce \emph{firm-side feedback}, shown to be essential for designing deterministic decentralized algorithms with time-independent regret (Appendix~\ref{Sec:justig}).  
Leveraging this feedback, we achieve decentralized—and even coordination-free—learning under the presence of strategic firms with a significantly improved bound of $O(n^3m)$ in structured markets, matching the centralized performance in order. As an additional contribution, we show that in structured markets, our regret bounds not only match the centralized order but also align in their constant factors, achieving true gap-independence.





==> intro-new.tex <==
\section{Introduction} \label{sec:intro}

Two-sided matching markets~\citep{roth1992two} are among the most fundamental models in economics and computer science, with broad applications ranging from labor markets~\cite{roth1984evolution} to school choice~\cite{abdulkadirouglu2003school} and dating platforms~\citep{hitsch2010matching}. A two-sided matching market consists of two sides, e.g., \(m\in\mathbb{N}^+\) firms and \(n\in\mathbb{N}^+\) workers (\(n\le m\)), where each side holds preferences over the other. A matching between the two sides is \emph{stable} if no worker–firm pair would both prefer to match with each other rather than remain with their current assignments~\cite{gale1962college}. In recent years, there has been a growing interest in studying bandit learning within two-sided matching markets~\cite{liu2020competing,maheshwari2022decentralized,liu2021bandit,kong2023player,ghosh2024competing}, where agents (workers) initially lack knowledge of their preferences\amedit{, described as \emph{uncertain},} and must learn them through repeated interactions. These interactions yield \emph{stochastic} rewards that gradually enable agents to refine their preferences over time. \amedit{Most existing works, however, treat firms as \emph{certain} entities in hiring---always assumed to know their preferences in advance and to hire the most preferred applicant whenever they receive applications. }




\amedit{However, unlike those cases, in many real-world markets, before committing to a match, agents can often gather preliminary information about potential matches through low-cost interactions such as interviews or visits, and then decide where to apply. In turn, firms, which may themselves be \emph{uncertain} about their preferences, may decide to \amedit{strategically} reject all current applicants if their most preferred candidate, although of relatively high quality, is perceived during the interviews as not meeting the desired standard.} For instance, consider a labor market consisting of \(n\) workers (e.g., agents, students) and \(m\) firms (e.g., employers, schools).
% \rev{with \(n\le m\)}.\todo{\mo{do we need to say this here? usually is the other way. }\xw{removed.}}
In each round of full interactions, a worker may first conduct interviews (e.g., site visits, phone screenings, etc.) with a subset of firms to gather information about their preferences. Based on the interview outcomes, each worker then applies to one of the interviewed firms and is hired only if the firm decides to hire one among the applicants and the worker is the most preferred. Similar preliminary interaction stages and firm-side \emph{strategic} confirmations also appear in other contexts: in dating markets, individuals may go on several dates before committing to a relationship; and in college admissions, students may attend open days or campus tours before submitting or confirming applications. While such preliminary interactions \amedit{(hereafter termed as \emph{interviews} but broadly refer to open house, career fair visit, introductory date, etc.)} have been studied in offline settings~\cite{lee2017interviewing,beyhaghi2021randomness}, their role in the learning dynamics of two-sided matching markets has been largely overlooked in the literature~\citep{liu2020competing,maheshwari2022decentralized,liu2021bandit,kong2023player,ghosh2024competing}.


To investigate how interviews facilitate learning in two-sided matching markets with \emph{strategic} firms—\amedit{where hiring decisions are made after interviews over an action set of hiring or not}—we consider a setting in which agents (workers) can interview a subset of firms before applying. In each round \(t\), each agent \(a\) selects a subset of firms \(\INT_a(t)\) to interview, with \(|\INT_a(t)| \leq k\) for some interview budget \(k \geq 2\). From these interviews, agent \(a\) observes \emph{stochastic} reward signals drawn from an unknown distribution with mean \(\mu_{a,f}\) for each interviewed firm \(f \in \INT_a(t)\), reflecting the expected utility of matching with \(f\). \amedit{After obtaining the interview results, agent \(a\) applies to one of the interviewed firms and is hired only if they are the firm’s most preferred applicant, with the firm \emph{strategically} deciding whether to hire post-interview. Upon hiring, the agent receives a stochastic reward drawn from an unknown distribution with mean \(\mu_{a,f}\). Each firm likewise gains information from its interviewed applicants by observing stochastic reward signals drawn from an unknown distribution with mean \(\mu_{f,a}\) for each agent \(a \in \INT_f(t)\), particularly when uncertain, as otherwise interviews would not alter their pre-interview preferences.}


The ultimate goal of all agents in the market is to learn a stable matching while minimizing their \emph{regret}, defined as the difference between the expected reward of the stable match and that of the agent's actual matches over \(T\in \mathbb{N}^+\) rounds. \amedit{While we define and analyze regret only for the agents, the presence of strategic and uncertain firms inherently makes this a two-sided learning problem, as firms also learn their preferences over time. Since stability is a mutual objective, convergence to a stable matching with bounded agent regret naturally implies analogous regret guarantees for the firms.}


The prior works~\cite{liu2020competing,maheshwari2022decentralized,liu2021bandit}, which do not consider the interview stage \rev{nor} the presence of uncertain or strategic firms, yield decentralized algorithms with \(O(\log T)\) regret over \(T\) rounds of interaction. \amedit{Additionally,~\cite{zhangbandit} studies decentralized learning with uncertain but non-strategic firms, relying heavily on firm–agent coordination (and thus implicit agent coordination) to achieve the same regret.} In contrast, we ask whether incorporating the interview stage can enable agents to learn a stable matching more efficiently—as more information is revealed through interviews—achieving lower regret and, crucially, without agent–firm coordination, even in the presence of \amedit{strategic uncertain firms} that may choose not to hire based on their current preference estimates, thereby incurring extra regret despite convergence to a stable matching by the agents.



Answering \rev{this question} involves several technical challenges: 

\amedit{$\blacktriangleright$ \textbf{Interviewing-Induced Limitations on Decision-Making:} Although the interview stage provides agents with more information to learn their preferences, it also constrains their final application decisions, since they can only apply to firms they have interviewed. This restriction on the action space introduces significant difficulties in both algorithm design and analysis. 

$\blacktriangleright$\textbf{Regret Minimization via Interviews:}  
While bandit learning with informative feedback has been explored in related frameworks—such as bandits with hints~\citep{wei2020taking,bhaskara2023bandit} \amedit{(single-agent hinted learning)} and~\cite{mirfakhar2025heterogeneous} \amedit{(multi-agent hinted learning)}—or more broadly through algorithms with predictions~\citep{lykouris2021competitive,bamas2020primal}, incorporating interview feedback as hints in two-sided matching markets is considerably more challenging due to interdependent agent behavior and the need to maintain stability \amedit{as a mutually defined objective} in the resulting matchings. 

$\blacktriangleright$\textbf{Agents’ Coordination in Decentralized Learning:}  
While an \emph{omniscient} central interview allocator can prevent collisions (or conflicts) by leveraging the learned preferences of both sides, in the fully decentralized setting, agents and firms cannot directly coordinate. Each agent acts independently and may struggle to align interview selections, potentially leading to collisions or conflicts when committing to the learned stable match.

$\blacktriangleright$ \textbf{Incorporating Firm Uncertainty:}  
While a central planner can potentially handle \emph{firm-side uncertainty}, addressing it in fully decentralized algorithms—where firms and agents cannot coordinate—remains a major challenge largely overlooked in prior work (excluding~\cite{zhangbandit}). Under such uncertain estimations, firms may mistakenly reject high-quality agents, causing those agents to disregard the firms in future rounds due to past rejections.

$\blacktriangleright$ \textbf{Modeling Strategic Firms:}  
The final layer of complexity arises from the presence of \emph{strategic firms} that may deliberately choose not to hire in certain rounds. This necessitates a dedicated algorithm for such firms—one that neither prevents agents from learning a stable matching nor induces high regret, while also remaining aligned with firms’ incentives toward learning stability. We assume all firms are strategic and design a parametric algorithm that, depending on whether a firm is certain or uncertain, adjusts its parameters to ensure incentive compatibility. Overall, this enables agents to leverage interviews effectively and achieve lower regret compared to settings without strategic or uncertain firms.
} \amcomment{Refer the author to an example in the appendix to clarify each challenge)}

In this paper, we consider both the \emph{centralized} setting, where a central planner coordinates all agents’ actions (as in online dating platforms), and the \emph{decentralized} setting, where each agent acts independently without a central planner (as in labor markets and college admissions). Our algorithms account for both firm uncertainty and strategic behavior, and—perhaps surprisingly—achieve time-independent $O(1)$ regret through adaptive interviewing in coordination-free and agent-only coordinating settings under mild assumptions.




\paragraph{Our Contributions.}
\amcomment{I added this as main contributions feel free to}

$\blacktriangleright$ We introduce a realistic model that incorporates \emph{strategic firms}, motivated by the observation that firms may misreport their preferences to improve the quality of their matches by choosing to remain unmatched rather than hiring low-quality agents. This aspect is crucial for firms to handle preference changes in decentralized setups. The addition captures uncertainty on the firm side and aligns with existing literature showing that strategic behavior can influence stability. Our decentralized and coordination-free algorithms explicitly account for such strategic firms while ensuring that the learning of stability remains achievable. Finally, we present an algorithm for strategic firms that is compatible with their incentive to learn stability.


$\blacktriangleright$ The works most closely related to our algorithmic framework are~\cite{liu2020competing,maheshwari2022decentralized}, both of which consider only non-strategic (certain) firms. Moreover, the latter assumes that agents know firm preferences in advance—an assumption we completely eliminate in our setting.

$\blacktriangleright$ focus on learning stability as the core objective and thein maximizing utility so firms and agent both are not willing to lose stability toward maximizing their utilities.

 $\blacktriangleright$ our main goal algorithm design is to achieve time-independent regret to learn stability through interviews with reveal information to both sides as a prior-decision making information as hints. While, the study of hints toward learning time independent regret. Among a few most recent ones in~\cite{bhaskara2023bandit,mirfakhar2025heterogeneous}, we adopt the idea of round-robin interviewing from these works. Even though this might seem similar to regular ETC, employing roundrobing observations toward achieving time-independent regret is a challenging problem even in single agents setup. meanwhile our setup setup is competitive and multi agent, we show that it makes possible to learn stability even under the assumptioin of strategic firms in decentralized setup with uncertain strategic firms. 

 $\blacktriangleright$ We design a centralized $\FGS$-based algorithm that, under both certain and uncertain firm setups, learns the agent-optimal stable matching in $O(nm)$ time. In this centralized framework, the interview allocator resolves potential collisions arising from uncertain preference lists, and agents do not exercise rejection decisions during learning. Following~\cite{kupfer2018influence}, firms in such cases can strategically improve their utility; however, whether such strategic behavior remains beneficial when preferences are uncertain and evolving over time—without compromising stability—remains an interesting open question.
$\blacktriangleright$ As our analysis suggests, agents may simply adopt round-robin interviews until their preference lists are sorted with high confidence, after which a distributed run of $\FGS$ can be executed. However, the simplest decentralization approach would require $O(m^2n^3)$ interviews for agents to fully sort all pairs of $m$ firms in their preference lists before running $\FGS$. In contrast, by carefully designing our algorithms, we achieve decentralized—and even coordination-free—learning under the presence of strategic firms with a significantly improved bound of $O(n^3m)$, matching the performance of the centralized algorithm. This constitutes one of our main contributions. For tructured markets our bounds remain the same but with gap independent factors that completely matches the performance of centralized algorithms not in order but in actual constants.


$\blacktriangleright$ To design decentralized algorithms, we show the necessity of having firm-side feedback—such as the revelation of vacant positions or anonymous hiring announcements. Under the former, coordination among agents is required to achieve the ideal decentralized bounds, whereas under the latter, we can design coordination-free algorithms, even in the presence of strategic firms. both with regret bound $O(n^3m)$.



 \subsection{Contributions}

    \noindent $\blacktriangleright$ We introduce a realistic model that incorporates \emph{strategic firms} (Section~\ref{sec:model}), motivated by the observation that firms may misreport their preferences to improve the quality of their matches by choosing to remain unmatched rather than hiring low-quality agents. This aspect is crucial for firms to handle preference changes in decentralized setups. The addition captures uncertainty on the firm side and aligns with existing literature showing that strategic behavior can influence stability. 

   \noindent $\blacktriangleright$ We start with the centralized setting
(Section~\ref{sec:centralized}), where a central interview allocator (\texttt{CIA}) controls all agents and coordinates their actions.
We design a centralized $\FGS$-based algorithm that, under both certain and uncertain firm setups, learns the agent-optimal stable matching in $O(nm)$ time. In this centralized framework, the interview allocator resolves potential collisions arising from uncertain preference lists, and agents do not exercise rejection decisions during learning. Following~\cite{kupfer2018influence}, firms in such cases can strategically improve their utility; however, whether such strategic behavior remains beneficial when preferences are uncertain and evolving over time—without compromising stability—remains an interesting open question.

\noindent $\blacktriangleright$ Lastly, we move to the decentralized setting (Section~\ref{sec:decentralized}), where each agent acts independently without a central planner,
and we consider two types of feedback from the firm side. 
While simply adopting round-robin interviews until their preference lists are sorted with high confidence and then applying $\FGS$ is a feasible algorithm design, it would require $O(m^2n^3)$ interviews, which is much worse than the $O(mn)$ bound in the centralized case.
By utilizing the firm-side feedback, we achieve decentralized---and even coordination-free---learning under the presence of strategic firms with a significantly improved bound of $O(n^3m)$, matching the performance of the centralized algorithm.\todo{\xw{confused, central is $O(nm)$, right?}} This constitutes one of our main contributions. As a side contribution, we also demonstrate that for structured markets, our bounds remain the same \todo{\xw{make it explicit, same $O(n^3m)$?}}, but with gap-independent factors that completely match the performance of centralized algorithms, not in order but in actual constants.


% For both types of feedback, we develop corresponding decentralized learning algorithms with \xw{\tdmark~add expressions here} regret bounds, respectively.
% \xw{\tdmark~add (1) algorithmic design ideas and (3) the proof techniques.}

% \tdmark
% \mx{I adjust the structure, and please check. My point is that we should put the emphasis on regret and the sufficiency of stable matching, instead of on the optimal matching,}
% \paragraph{Related Works.}
% \tdmark~One paragraph on bandit learning on two-sided matching markets.
% At the end, highlight none of them consider the interview stage.

% \tdmark~One paragraph on stable matching with interviews.
% At the end, highlight none of them consider the learning dynamics.

% \tdmark~One brief paragraph on online learning with hints or predictions. Just say our work can also be placed in this line of works, but we focus on the two-sided matching market setting.





==> intro-v3.tex <==
\section{Introduction}\label{sec:intro}
Two-sided matching markets~\citep{roth1992two} are a foundational model with applications in labor markets~\citep{roth1984evolution}, school choice~\citep{abdulkadirouglu2003school}, and dating platforms~\citep{hitsch2010matching}. A market comprises two sides (e.g., \(m\) firms and \(n\) agent), each with preferences over the other side. A matching is \emph{stable} if no agent--firm pair would both prefer to deviate from their current assignments~\citep{gale1962college}.

In practice, preferences are rarely known a priori and must be learned, e.g., through agent-firm interactions. This motivates \emph{bandit learning} in matching markets~\citep{liu2020competing,maheshwari2022decentralized,liu2021bandit,kong2023player,ghosh2024competing}, where agents repeatedly apply to firms, observe stochastic outcomes, and aim to learn a stable matching while minimizing regret. Existing literature largely assumes that (i) only agents are uncertain and (ii) firms always hire according to fixed, known preferences.

Despite substantial progress, two salient features of real markets remain underexplored in prior work: \textbf{pre-matching interviews} and \textbf{firm-side uncertainty}. First, participants often engage in low-cost preliminary interactions (e.g., interviews or visits) before submitting final applications, obtaining early but noisy signals about match quality. This perspective connects naturally to \emph{bandits with hints}~\citep{bhaskara2022online,mirfakhar2025heterogeneous} and, more broadly, to \emph{algorithms with predictions}~\citep{lykouris2021competitive}. However, incorporating interviews into two-sided learning introduces challenges absent from existing hinted-bandit settings: interviews simultaneously \emph{reveal information} and \emph{constrain decision-making}, since agents may apply only to firms they have interviewed.


Second, firms may be uncertain about their own preferences (i.e., preferences are unknown a priori); early misrankings can lead them to reject strong candidates, slowing convergence to a stable matching and increasing regret. To hedge against this uncertainty---and motivated by real-world hiring behavior---we expand the firm action space to permit \emph{strategic deferral}: a firm may choose to remain unmatched in a decision round rather than commit to a hire it currently deems suboptimal. This added flexibility is crucial for learning stable matching in decentralized settings and aligns with offline evidence that firm-side strategic behavior can shape stable outcomes~\citep{kupfer2018influence,lee2017interviewing,beyhaghi2021randomness}.


\paragraph{Model and objective.}
We study two-sided bandit learning with \emph{interviews}, capturing uncertainty on both the agent and firm sides. In each round \(t\), every agent \(a\) selects a fixed number of firms to interview, denoted \(\INT_a(t)\). Each interviewed pair \((a,f)\) yields stochastic, noisy feedback to \emph{both} sides with unknown means \(\mu_{a,f}\) and \(\mu_{f,a}\), representing their expected utilities from matching with each other. After interviewing, each agent applies to one of its interviewed firms; a firm hires only if the applicant is its most preferred among current applicants \emph{and} the firm chooses to hire (otherwise it may defer and remain unmatched). When a match occurs, both sides receive stochastic rewards drawn from the corresponding distributions.

We evaluate performance via \emph{agent regret}: the gap between the expected reward of the agent’s (true-mean) stable partner and the reward accrued over \(T\) rounds. We study both a \emph{centralized} setting with an omniscient interview allocator and \emph{decentralized} settings with no (or minimal) coordination. Crucially, in decentralized markets we allow only a \emph{minimal public firm-side signal} revealed to all agents at the end of each round—either \emph{vacancy-only} feedback (whether a firm filled its position) or \emph{anonymous hiring-change} feedback (whether a firm’s hire changed), with no identities revealed; see Appendix~A.2. As shown in Appendix~\ref{Sec:justig}, some such (necessarily coarse) firm-side signal is required to obtain decentralized algorithms with time-independent regret. 


Most prior work on bandit learning for stable matchings~\citep{liu2020competing,maheshwari2022decentralized,liu2021bandit} does not model pre-matching interviews or strategic uncertain firms, and the best-known decentralized guarantees scale at least logarithmically with the horizon, typically \(O(\log T)\) regret. In contrast, interviews provide additional low-cost feedback before committing to an application, suggesting the possibility of substantially faster learning. This raises a natural question: \emph{can interviews be leveraged to learn a stable matching with lower---ideally time-independent---regret, and can this be achieved in a decentralized manner without explicit agent--firm coordination, even when firms are uncertain and may strategically choose to defer hiring?}

\paragraph{Technical challenges.}
Answering the above question requires overcoming several challenges.

\noindent$\blacktriangleright$ \textit{Interviews as hinted learning in two-sided markets:}
Interviews provide low-cost, noisy signals that can accelerate preference learning, but they also \emph{restrict} actions: an agent can apply only to firms it interviewed.
Unlike prior bandits-with-hints work---in single-agent~\citep{wei2020taking,bhaskara2023bandit} and multi-agent settings~\citep{mirfakhar2025heterogeneous}---our problem couples agents through competition and stability constraints. Exploiting interview feedback is therefore harder because agents’ choices interact, and firms are simultaneously learning and acting strategically.

A central interview allocator can enforce globally compatible interview sets, but in decentralized markets agents choose interviews independently, without firm--agent coordination, so \emph{collisions} (many agents chasing the same firms) can prevent stability and drive regret. Moreover, unlike prior decentralized bandit-matching work such as~\citet{liu2021bandit}—which assumes agents know firms’ preferences and observe the \emph{identity} of each firm’s current match—here firms may be uncertain and agents receive only coarse, \emph{anonymous} signals (Appendix~\ref{Sec:justig}): whether a firm is vacant or whether its hire changed, but never who was hired and never firms’ preferences; designing low-regret stable dynamics under such non-identifying feedback is nontrivial.

\noindent$\blacktriangleright$ \textit{Firm uncertainty: early rejections and strategic deferral:}
With uncertain rankings, firms may reject strong agents during interview phases. Such early rejections can redirect agents’ future behavior and slow the convergence to stability in decentralized dynamics.
Further, allowing firms to defer hiring (Example~\ref{sec:strategic}) expands their action space and is necessary for decentralized learning, but it requires careful control: deferral must not inflate regret or obstruct stability, while remaining aligned with firms’ incentives.



\paragraph{Our contributions.}
We introduce and analyze a two-sided bandit model with interviews and \emph{uncertain, strategic firms}, and show that interviews enable \emph{time-independent} learning of stable matchings in both centralized and decentralized markets. In all setups below, we obtain \(O(1)\) (time-independent) agent regret, with explicit dependence on market parameters. Below, we summarize our contributions.

\noindent $\blacktriangleright$ We model \emph{firm-side uncertainty} and its impact on hiring, and integrate it into a two-sided learning process (\autoref{sec:model}). To make decentralized learning viable, we extend firms’ action space by allowing them to strategically abstain from hiring. We then design an incentive-compatible \emph{strategic rejection policy}~(\cref{alg:fdrr}) that controls deferral so it supports stability and learning, consistent with offline evidence that strategic rejections can improve firms’ stable outcomes~\cite{kupfer2018influence}.

\noindent$\blacktriangleright$ We formalize interviews as \emph{bandit hints} in a competitive, two-sided market and show that \emph{two interviews per round} (except one appendix extension that uses three) suffice for time-independent regret (\cref{thm:ciarr}). This strengthens the conjecture of~\citet{bhaskara2023bandit} (posed for single-agent learning) which suggested that three hints per round may be required for time-independent regret: we establish that two hints already suffice in the substantially more challenging setting of double-sided, competitive learning with strategic uncertain firms. Moreover, whereas~\citet{zhangbandit} used round-robin exploration in a related model without interviews or strategic firms to obtain \(O(\log T)\) regret, we extend the framework to interview-based learning and strengthen the guarantee to time-independent regret.

\noindent $\blacktriangleright$ In the centralized setting (\autoref{sec:centralized}), we design a central interview allocator (\texttt{CIA}) that coordinates interviews and applications. Building on \(\FGS\)~\cite{gale1962college}, we give an algorithm that (under both certain and uncertain firm setups) learns the agent-optimal stable matching in \(O(nm^2)\) time (\cref{thm:ciarr}). In this framework, the allocator resolves collisions arising from uncertain preference lists, and agents or firms do not need to coordinate.

\noindent $\blacktriangleright$ In the decentralized setting without a central planner, we give two algorithms that match the minimal-information nature of real markets. Under vacancy-only feedback \(\VF\) (\cref{sec:decwithvf}), we provide a \emph{coordinated} algorithm (\cref{alg:drr}) using two interviews per round, achieving \(O(n^3m^2)\) regret in structured markets (\cref{thm:alphadecreg}) and \(O(n^4m^2)\) regret in general markets (\cref{thm:decreg}). Under anonymous hiring-change feedback \(\VFP\) (\cref{sec:non-coop}), we design a \emph{coordination-free} algorithm (\cref{alg:ancdrr})—again with two interviews per round—achieving \(O(n^3m^2)\) regret in structured markets (\cref{thm:noncoalphadecreg}). Extending this coordination-free approach to general markets (\cref{sec:noncoopgen}) requires an extension to three interviews per round and additional mild assumptions, yielding \(O(1)\) regret (\cref{thm:noncogendecreg}).

% \xw{better to give the detail here as the above big-O results}.


% The bounds for strucmatching the centralized order. Moreover, in structured markets our bounds are truly gap-independent, matching the centralized constants as well.


% We introduce a bandit model of matching with interviews that captures \emph{firm-side uncertainty} and allows \emph{strategic deferral} (\autoref{sec:model}), extending prior work that either assumes known firm preferences or considers uncertain but non-strategic firms with strong coordination requirements~\citep{zhangbandit}. Our algorithms treat interviews as noisy hints and achieve \emph{time-independent} \(O(1)\) regret through adaptive interviewing; notably, they use two interviews per round with one chosen in a round-robin fashion, strengthening the hinted-learning view relative to conjectures in single-agent hinted bandits~\citep{wei2020taking,bhaskara2023bandit}. We provide algorithms in both centralized and decentralized regimes. In the centralized setting (\autoref{sec:centralized}), we give an \(\FGS\)-based procedure~\citep{gale1962college} that learns the agent-optimal stable matching in \(O(nm)\) time under both certain and uncertain firms. In decentralized settings (\autoref{sec:decentralized}), we show that \emph{firm-side feedback} is essential and design deterministic algorithms using vacancy announcements and anonymous revelation of new hires; these achieve time-independent regret, and under mild structure, decentralized performance approaches the centralized benchmark up to polynomial factors in \(n\) and \(m\).



==> intro.tex <==


\section{Introduction} \label{sec:intro}


Making decisions under uncertainty is a core challenge in modern machine learning.
Algorithms must adapt to unknown conditions as they interact with the world.
A natural testbed is the multi-agent setting, where many agents learn simultaneously and each agent’s outcome depends not only on its own actions but also on the behavior of others~\cite{cesa2006prediction}.
Motivated by applications such as hiring in labor markets, dating apps, and ride-sharing platforms, learning stability in matching markets has become a key focus, with a line of work initiated by~\cite{liu2020competing}.
These models consider heterogeneous agents and heterogeneous resources (e.g., firms, schools, potential partners), each with preferences over the other side.
A matching is \emph{stable} if there is no agent--resource pair that would both prefer to match with each other rather than keep their current assignments.
In this line of work, online statistical methods, such as Multi-Armed Bandits~\cite{lattimore2020bandit} are used to learn stable matchings when agents start not knowing about their own preferences: they compete for resources while estimating their valuations and, through competition outcomes, inferring the resources’ preferences.

Within this growing body of work~\cite{maheshwari2022decentralized,liu2020competing,liu2021bandit},
exploration in learning-based matching typically proceeds by attempting \emph{actual} matches—an approach that can be costly like the firms spending one hiring season to just evaluate of what quality the graduates of some schools are that can be mitigated through a bit of extra-pre hiring information.
We ask an underexplored question: \emph{How much can agents gain, when learning stable matchings~\cite{gale1962college}, if they are given extra pre-match information about the factors shaping their preferences—without committing to a match, especially when commitment is expensive?}
This question arises naturally in labor markets—where a mismatched hire can be extremely costly—and in dating/marriage markets, where commitment is long-term and proposals are high-stakes. The classical “stable matching with interviews” model, introduced by~\cite{lee2017interviewing} and extended by~\cite{beyhaghi2021randomness}, assumes a single interview stage that effectively reveals all relevant preferences.
In contrast, we study learning dynamics where interviews act as low-cost, \emph{incremental} signals: agents adaptively decide whom to interview and when to apply, using these hints to curb costly exploration and accelerate convergence to stability.


\textcolor{red}{make it shorter on defining the stability and the stuff about the matching markets. clarify the word uncertain}\textcolor{orange}{second paragraph to be shorter, for now put "although bandit in two sided is studied we raise this underexplored question of:}

We take this one step further by asking the underexplored question of:
\emph{how can supplementary information about preferences help agents reach stability when exploration is costly?}

In both cases, low-cost \amcomment{cost is something might me misleading, and add the stuff like the interviewing process is common and helpful} sources of additional information—such as interviews with graduates of a school,
or a series of low-stakes romantic meetings—can provide valuable insights.
Such information allows agents to make better-informed decisions and avoid the high cost of direct trial-and-error exploration.
Motivated by this, we study the problem of learning stable matchings in settings where firms can interview applicants before making hiring decisions.
Beyond filling specific positions, these interviews also help firms form general beliefs about the quality of graduates from different schools.
Our findings show that this additional source of information can significantly accelerate the learning process,
leading to stable matches more quickly and efficiently.  \textcolor{red}{expand the information about the labor market and keep the others less expanded but count a few more applications instead}

\amcomment{bandit stuff} To model the underlying uncertainty, we follow prior work and employ the \emph{Multi-Armed Bandits} framework.
Here, job-seeking agents are treated as the learners, while firms play the role of the arms.
At each round, an agent applies to a firm and is hired only if they are the firm’s most preferred applicant,
in which case the agent observes a reward that feeds into their learning algorithm.
This framework was first introduced by [\dots] and later extended in [\dots]. Building on this well-defined model, we introduce a new formulation that embeds the acquisition of additional information through interviews.
The idea of augmenting bandit learning with extra signals has been studied in the single-agent setting under the name
\emph{multi-armed bandits with hints}, where a learner may query for side information before taking an action.
In contrast, our \emph{multi-agent bandits with hints}~\cite{bhaskara2022online,mirfakhar2025heterogeneous} framework adapts this idea to matching markets:
agents must first reach out to a subset of firms, conduct interviews, and then choose one of the interviewed firms to apply to.
This captures the natural role of interviews as a low-cost but informative step before making costly commitment decisions. \textcolor{red}{remove all the stuff about the mab and just mention the our setup while pointing out to the MAB model without mentioning what others have done}


\paragraph{Our Contribution.}

\paragraph{Related Words.}








==> model-new-v2.tex <==
\vspace{-0.5em}
\section{Model and Preliminaries}\label{sec:model}

Consider a two-sided market $\MARK(\AG,\FI)$ with $n$ agents $\AG$ and $m$ firms $\FI$, where $n\leq m$.
The terminology is generic: in the platform applications motivating this work, agents may be creators, job seekers, users, or mentees, while firms may be brands, employers, campaigns, mentors, or reciprocal-recommendation opportunities; Appendix~\ref{app:digital-platform-motivations} gives a detailed mapping.
Each agent--firm pair $(a,f)$ is associated with two reward distributions: $\DIS_{a,f}$ for agent $a\in\AG$, with mean $u_{a,f}$, and $\DIS_{f,a}$ for firm $f\in\FI$, with mean $u_{f,a}$.
Rewards are independent across agent--firm pairs and time steps, and are bounded in $[0,1]$.
We assume a heterogeneous market with no ties: for every agent $a$ and distinct firms $f,f'\in\FI$, $u_{a,f}\neq u_{a,f'}$, and for every firm $f$ and distinct agents $a,a'\in\AG$, $u_{f,a}\neq u_{f,a'}$.
Thus preferences are strict and induce well-defined rankings on both sides.

For each agent $a\in\AG$, the \emph{ground-truth preference list} $\PL_a$ ranks firms by decreasing $u_{a,f}$, and we write $f\underset{\PL_a}{>}f'$ if $u_{a,f}>u_{a,f'}$.
Analogously, each firm $f\in\FI$ has a ground-truth preference list $\PL_f$ ranking agents by decreasing $u_{f,a}$, with $a\underset{\PL_f}{>}a'$ defined similarly.
Agents do not know their preferences \emph{a priori} and must learn them from observations.
On the firm side, we consider two cases: \emph{certain firms}, which know their preference lists in advance, and \emph{uncertain firms}, which must learn them over time.
Each agent maintains an estimate $\hat{u}_{a,f}(t)$ of $u_{a,f}$, and each firm maintains an estimate $\hat{u}_{f,a}(t)$ of $u_{f,a}$.
The induced estimated preference lists are denoted by $\EPL_a(t)$ and $\EPL_f(t)$.
For a certain firm $f$, $\hat{u}_{f,\cdot}(t)=u_{f,\cdot}$ and hence $\EPL_f(t)=\PL_f$ for all $t\in\mathcal{T}$.


% Consider a two-sided market $\MARK(\AG,\FI)$ with $n$ agents (forming set $\AG$) and $m$ firms (forming set $\FI$), where $n \leq m$. Each agent-firm pair $(a,f)$ is associated with two reward distributions: $\DIS_{a,f}$ for agent $a \in \AG$, with mean $u_{a,f}$ (the expected reward of $a$ when matched with $f$), and $\DIS_{f,a}$ for firm $f \in \FI$, with mean $u_{f,a}$. Without loss of generality, we assume that the distributions are independent across different agent--firm pairs and across time steps, and that the rewards are bounded in $[0,1]$, consistent with the standard literature. We further assume a heterogeneous market with strictly ordered preferences. Specifically, for every agent $a \in \AG$ and any two distinct firms $f,f' \in \FI$, we have $u_{a,f} \neq u_{a,f'}$, and similarly, for every firm $f \in \FI$ and any two distinct agents $a,a' \in \AG$, $u_{f,a} \neq u_{f,a'}$. This assumption rules out indifferences and induces a strict total ordering of firms for each agent and of agents for each firm, ensuring well-defined preference lists on both sides of the market. For each agent $a \in \AG$, the \emph{ground-truth preference list} $\PL_a$ ranks firms in $\FI$ by decreasing $u_{a,f}$, and we write $f \underset{\PL_a}{>} f'$ if $u_{a,f} > u_{a,f'}$. Analogously, each firm $f \in \FI$ has a ground-truth preference list $\PL_f$ ranking agents in $\AG$ by decreasing $u_{f,a}$, with $a \underset{\PL_f}{>} a'$ defined similarly.

 % (the expected reward of $f$ when matched with $a$) \mx{$f_i$, $f_j$ are not defined and thus this example is not clear\amcomment{Done!}}.

% In our model, agents do not know their preferences \emph{a priori} (equivalently, the underlying reward distributions) and must learn them over time. On the firm side, we consider two scenarios: \emph{certain firms}, which know their preference lists in advance, and \emph{uncertain firms}, which must learn their preference lists over time. Each agent maintains an estimate $\hat{u}_{a,f}(t)$ of $u_{a,f}$ at time $t$, and each firm maintains an estimate $\hat{u}_{f,a}(t)$ of $u_{f,a}$. The preference lists induced by these estimates are the \emph{estimated preference lists}, denoted by $\EPL_a(t)$ and $\EPL_f(t)$. For a certain firm $f$, we have $\hat{u}_{f,\cdot}(t)=u_{f,\cdot}$ and thus $\EPL_f(t)=\PL_f$ for all $t\in\mathcal{T}$.

% For \emph{certain firms}, $\hat{u}_{f,a}(t)=u_{f,a}$ for all $t$, and hence $\EPL_f(t)=\PL_f$.
 % \mx{this means that the hat estimator also holds for certain firms, but in the previous sentence, hat estimators are only for uncertain firms, please make sure they are consistent.\amcomment{Done!}}





% If firms are \emph{uncertain} and choose to hire ($\NH_f(t)=1$), they admit their most preferred applicant according to $\EPL_f(t)$, i.e.,
% \(
% \FFM_f(t) = \{a \in \APP_f(t) : a \underset{\EPL_f(t)}{>} a', \forall a' \in \APP_f(t)\}.
% \)

% When an agent $a$ is matched to a firm $f$, the agent receives a stochastic reward drawn from an unknown distribution $\DIS_{a,f}$ with mean $u_{a,f}$, and the firm receives a stochastic reward drawn from an unknown distribution $\DIS_{f,a}$ with mean $u_{f,a}$.

\textbf{Decision Process.}
Given \(T\) rounds, let \(\mathcal{T}\) denote the set of decision-making rounds with \(|\mathcal{T}|=T\). We exhibit the following sequential interaction dynamics between agents and firms (whether \emph{certain} or \emph{uncertain}), consisting of three stages: \emph{interview}, \emph{application}, and \emph{firm-side feedback revelation}. Specifically, in each round \(1 \leq t \leq T\):


$\blacktriangleright$ \emph{Interview stage.}
Each agent $a \in \AG$ selects a subset of firms $\INT_a(t) \subseteq \FI$ to interview\footnote{Although, we refer to this stage as an \emph{interview}, it is more akin to an open house or participation in a career fair.}, with size $2 \leq |\INT_a(t)| \leq k$, where $k \in \mathbb{N}^+$ is the \emph{interview budget}.
For each interviewed firm $f \in \INT_a(t)$, the agent observes a stochastic signal $X_{a,f}(t) \sim \DIS_{a,f}$ drawn from distribution $\DIS_{a,f}$ with mean $u_{a,f}$; notably, these signals are not counted as rewards.
Similarly, each firm $f$ interviews agents in $\INT_f(t)$ and observes $X_{f,a}(t) \sim \DIS_{f,a}$ for each $a \in \INT_f(t)$.

$\blacktriangleright$ \emph{Application stage.}
After obtaining the interview results, each agent \(a\) applies to one of the interviewed firms \(\FA_a(t)\in\INT_a(t)\).

     (i) Each firm \(f\) collects applications from agents, denoted by \(\APP_f(t)=\{a\in\AG:\FA_a(t)=f\}\).
           %The
            If firm \(f\) decides to hire, it admits
            its most preferred applicant
            within \(\APP_f(t)\) according to its current preference as \(\FFM_f(t) = \argmax_{\APP_f(t)} \hat{u}_{f,a}(t).\) 

           
     (ii) If \(\FFM_{\FA_a(t)}(t) = a\), then agent \(a\) is hired by firm \(\FA_a(t)\) and receives a stochastic reward \(X_{a,\FA_a(t)}(t)\sim \DIS_{a,\FA_a(t)}\); otherwise, agent \(a\) receives no reward.
           We denote the match of agent $a$ at round $t$ by
           \(\FM_a(t)\)
           where $\FM_a(t) = \FA_a(t)$ if $a$ is admitted by its applied firm, and $\FM_a(t) = \emptyset$ otherwise.
           The match of firm $f$ is similarly denoted as $\FFM_f(t)$. Precisely, the reward received by agent $a$, denoted $X_{a,\FM_a(t)}$, is defined as
           \begin{align} X_{a,\FM_a(t)}=X_{a,\FA_a(t)}\mathbbm{1}\left\{\FM_a(t) \neq \emptyset\right\}.\label{def:rewards1}
           \end{align}
           
$\blacktriangleright$ \emph{Firm-side feedback revelation stage.}
At the end of round $t$, agents observe one of the following firm-side feedback.

\begin{minipage}{0.40\linewidth}
{\small
\begin{align}
     \VF(t)  &\doteq \{f \in \FI : \FFM_f(t) = \emptyset\}, \label{def:vf}
\end{align}
}
\end{minipage}
\hfill
\begin{minipage}{0.60\linewidth}
{\small
\begin{align}
     \VFP(t) &\doteq \VF(t)\cup\{f \in \FI : \FFM_f(t-1) \neq \FFM_f(t)\}. \label{def:vfp}
\end{align}
}
\end{minipage}

Here, the \emph{vacancy-only} feedback $\VF(t)$ is the set of firms that are vacant at time $t$, whereas \emph{anonymous hiring changes} $\VFP(t)$ includes firms whose hiring status has changed since the previous round, without revealing their current matches, on top of the vacancies; i.e., $\VF \subseteq \VFP$. We view $\VF(t)$ as the weaker signal and $\VFP(t)$ as the stronger one; these feedback determine what information agents observe and play a central role in our algorithm design.

\noindent\textbf{Optimal and Pessimal Regrets.}
For policy $\pi$, we use regret to quantify performance from the agents' perspective. Since multiple stable matchings may exist, we focus on agent-optimal and agent-pessimal stable matches with corresponding analysis depending on whether we are in the centralized or decentralized model. 
% our goal is to learn the agent-optimal stable matching, where each agent is matched to its most preferred firm among all stable matchings. %, and otherwise converge to
% \hbedit{We also consider} the agent-pessimal one, defined analogously as the least preferred stable outcome for each agent.
More precisely, following the prior work~\cite{liu2021bandit}, we define the \emph{optimal} and \emph{pessimal} regrets under policy \(\pi\) for agent $a$ over $T$ rounds as follows

     {\small
\setlength{\abovedisplayskip}{-15pt}
\begin{align}
    \underbrace{\mathbb{E}[\overline{R}_a(\pi,T)]}_{\text{$a$-Optimal}} \doteq \sum_{t=1}^T u_{a,\overline{f^*_a}} - \mathbb{E}[X_{a,\FM_a(t)}(t)], 
    \qquad
    \underbrace{\mathbb{E}[\underline{R}_a(\pi,T)]}_{\text{$a$-Pessimal}} \doteq \sum_{t=1}^T u_{a,\underline{f^*_a}} - \mathbb{E}[X_{a,\FM_a(t)}(t)], \label{eq:optreg}
\end{align}
}
where $\overline{f^*_a}$ and $\underline{f^*_a}$ are the best and worst stable matches of agent $a$.
For brevity, we omit the policy $\pi$ from the regret and use $\mathbb{E}[\overline{R}_a(T)]$ and $\mathbb{E}[\underline{R}_a(T)]$, hereinafter. For each agent $a \in \AG$ and firm $f \in \FI$, we define the \emph{optimal reward gap} as $\overline{\Delta}_{a,f} \doteq |u_{a,\overline{f^*_a}} - u_{a,f}|$ and the \emph{pessimal reward gap} as $\underline{\Delta}_{a,f} \doteq |u_{a,\underline{f^*_a}} - u_{a,f}|$. Similarly, we define optimal reward gap as $\overline{\Delta}_{f,a} \doteq |u_{f,\underline{a^*_f}} - u_{f,a}|$ and pessimal reward gap as $\underline{\Delta}_{f,a} \doteq |u_{f,\overline{a^*_f}} - u_{f,a}|$, where $\overline{a^*_f}$ and $\underline{a^*_f}$ denote the firm-optimal and pessimal stable matches for firm $f$, noting the agent-optimal matching is firm-pessimal and vice versa~\cite{gale1962college}.

We note that when the market admits a unique stable matching, the pessimal and optimal regrets are identical, implying consistency. As such, for those markets, we denote the regret and reward gaps by $\mathbb{E}[R_a(T)]$, $\Delta_{a,f}$, and $\Delta_{f,a}$. An example of such a market is presented as follows.


\textbf{$\alpha$-Reducible Markets.} A key class of markets with a unique stable matching is $\alpha$-reducible markets, introduced for uniqueness by~\cite{clark2006uniqueness} and later used by~\cite{maheshwari2022decentralized} for coordination-free decentralized bandit learning. This structure is less restrictive than serial dictatorship~\citep{sankararaman2021dominate,wang2024optimal}, while still covering a broad family of unique-stable-matching markets. Formally, a pair $(a,f)\in \AG\times\FI$ is a \emph{fixed pair} if $a$ and $f$ are mutual top choices, i.e.,
$f \underset{O_a}{>} f'$ for all $f' \in \FI \setminus \{f\}$, and
$a \underset{O_f}{>} a'$ for all $a' \in \AG \setminus \{a\}$.

\vspace{-0.7em}
\begin{definition}
A market $\MARK(\AG,\FI)$ is \emph{$\alpha$-reducible} if every $\MARK(\AG',\FI')$ with $\AG'\subseteq\AG$ and $\FI'\subseteq\FI$ contains a fixed pair.
\end{definition}
\vspace{-0.7em}


In $\alpha$-reducible markets, we can iteratively remove fixed pairs: there exists a fixed pair $(a_1,f_1)$; removing it yields an $\alpha$-reducible sub-market; repeating yields pairs $(a_i,f_i)_{i\in[n]}$, which match all agents and induce the unique stable matching with firms in $\FI\setminus\{f_i\}_{i\in[n]}$ left unmatched. We focus on $\alpha$-reducible markets in the main body, as this layered structure highlights the analysis and the main proof ideas and defer the extension to general markets to the appendix.

%\vspace{-1em}
\subsection{Extended Action Space for Firms' Uncertainty}
A key departure from prior work is that firms may be \emph{uncertain} about their own preferences.
If an uncertain firm is forced to hire whenever it has applicants, early estimation errors can ``lock in'' an unstable outcome: the firm keeps hiring the agent it currently, but incorrectly, believes is best, while agents may receive no local evidence that the firm has learned otherwise.
We therefore extend the firm action space to allow a firm to \emph{strategically abstain} from hiring in selected rounds.
In platform terms, this corresponds to leaving a campaign slot open or postponing a hire or mentorship.
Crucially, abstention makes the firm publicly vacant through $\VF(t)$ and $\VFP(t)$, giving previously rejected agents a coarse signal that can unwind decentralized deadlocks.


\begin{example}[Why abstention is necessary]\label{examp:introstrategic}
Let $\MM$ have agents $\AG=\{a_1,a_2\}$ and (strategic) uncertain firms $\FI=\{f_1,f_2\}$ with ground-truth preferences
$
\PL_{a_1}:\langle f_1^\dagger \succ f_2\rangle, \PL_{a_2}:\langle f_1 \succ f_2^\dagger\rangle  \text{ and } \PL_{f_1}:\langle a_1^\dagger \succ a_2\rangle, \PL_{f_2}:\langle a_2^\dagger \succ a_1\rangle
$
The unique stable matching is $(a_i,f_i)_{i\in[2]}$ (marked by $\dagger$s). Suppose that at time $t$ the estimated preferences are
$
\EPL_{a_1}(t):\langle f_1 \succ f_2^*\rangle, \EPL_{a_2}(t):\langle f_1^* \succ f_2\rangle  \text{ and } \EPL_{f_1}(t):\langle a_2^* \succ a_1\rangle, \EPL_{f_2}(t):\langle a_2 \succ a_1^*\rangle,
$
so only $f_1$ is wrong (it swaps $a_1$ and $a_2$). The stable matching under $\EPL(t)$ is $(a_1,f_2)$ and $(a_2,f_1)$, marked by $(*)$s, which is unstable under the ground truth.

Now assume that at some later time $t'>t$, firm $f_1$ learns the correct order, i.e., $\EPL_{f_1}(t')=\PL_{f_1}$. In a decentralized setting, this correction may be \emph{unobservable} to agents, so if firms always hire, the market can remain stuck at $(a_1,f_2),(a_2,f_1)$. If instead $f_1$ can abstain at $t'$, it can \emph{reject} its current hire: by not hiring, $f_1$ becomes vacant and appears in the firm-side feedback, which all agents observe. This vacancy triggers $a_2$ to move to $f_2$, which displaces $a_1$ back to $f_1$, restoring the stable matching $(a_i,f_i)_{i\in[2]}$.
\end{example}

Formally, we allow each firm $f\in\FI$ to choose a private binary hiring decision $\NH_f(t)\in\{0,1\}$ each round, where $\NH_f(t)=1$ means hire and $\NH_f(t)=0$ means remain vacant. The decision is taken after interviews, once $f$ observes its applicant set $\APP_f(t)$. With this modification, the realized reward of agent $a$ becomes \refstepcounter{equation}\label{eq:reward} \noindent \(X_{a,\FM_a(t)}
=
\NH_{\FA_a(t)}(t)\,X_{a,\FA_a(t)}\,\mathbf{1}\{\FM_a(t)\neq \emptyset\}.\)\hfill(\theequation)

Accordingly, beyond agent-side learning, we introduce a \emph{strategic rejection policy} (\cref{alg:fdrr}) that selects $\NH_f(t)$ each round. We call any firm running \cref{alg:fdrr} \emph{strategic}, even if it never abstains; for a strategic \emph{certain} firm, \cref{alg:fdrr} never triggers abstention, so $\NH_f(t)=1$ for all $t$. Firms that hire every round are \emph{non-strategic} (even if uncertain). We defer the formal policy to~\cref{sec:uncertain-firms}.





% \begin{comment}
    


% \subsection{Extended Action Space for Firms' Uncertainty} We incorporate firm uncertainty into the learning process by extending the firm action space beyond always hiring, as in prior work, to allowing firms to \emph{strategically} abstain from hiring in a round. Under uncertainty, firms do not know their true preference lists a priori and therefore make hiring decisions based on estimated preferences. Consequently, a firm may repeatedly hire an agent it currently estimates to be high-quality, even when this differs from its ground-truth optimal match. Allowing firms to defer hiring lets them revise decisions as estimates evolve and, crucially, creates opportunities for agents who were previously rejected due to estimation error to reconsider the firm, since abstention makes the firm appear in the firm-side feedback $\VF(t)$ and $\VFP(t)$. This flexibility is essential for learning stable matchings in decentralized settings (see Example~\ref{examp:introstrategic} for intuition).

% % \begin{example}\label{examp:introstrategic}\label{sec:strategic}
% % Let $\MM$ have agents $\AG=\{a_1,a_2\}$ and strategic uncertain firms $\FI=\{f_1,f_2\}$ with ground-truth preferences
% % \[
% % \begin{array}{lr}
% % \PL_{a_1}:\langle f_1^\dagger \succ f_2\rangle & \PL_{f_1}:\langle a_1^\dagger \succ a_2\rangle\\
% % \PL_{a_2}:\langle f_1 \succ f_2^\dagger\rangle & \PL_{f_2}:\langle a_2^\dagger \succ a_1\rangle .
% % \end{array}
% % \]
% % The unique stable matching is $(a_i,f_i)_{i\in[2]}$.

% % Suppose that at some time $t$ the estimated preferences satisfy
% % \[
% % \begin{array}{lr}
% % \EPL_{a_1}(t):\langle f_1 \succ f_2^\dagger\rangle & \EPL_{f_1}(t):\langle a_2^\dagger \succ a_1\rangle\\
% % \EPL_{a_2}(t):\langle f_1^\dagger \succ f_2\rangle & \EPL_{f_2}(t):\langle a_2 \succ a_1^\dagger\rangle .
% % \end{array}
% % \]
% % Thus $a_1,a_2$ and $f_2$ are already correct, while $f_1$ is still uncertain and (incorrectly) ranks $a_2$ above $a_1$. The stable matching induced by $\EPL(t)$ is $(a_1,f_2)$ and $(a_2,f_1)$, which is unstable under the ground truth.

% % Since $a_1,a_2,$ and $f_2$ are already correct, the agents receive no local signal that would prompt them to deviate. Eventually, at some $t'>t$, firm $f_1$ learns the correct order and $\EPL_{f_1}(t')=\PL_{f_1}$, but this correction need not be observable to the agents, so the matching can remain $(a_1,f_2),(a_2,f_1)$ indefinitely.

% % Allowing $f_1$ to \emph{strategically reject} at $t'$ breaks this deadlock via the firm-side feedback. If $f_1$ rejects $a_2$ (chooses not to hire), then $f_1$ becomes vacant and this change is revealed to all agents. This triggers $a_2$ to move to $f_2$, which forces $a_1$ off $f_2$ and back to $f_1$, restoring $(a_i,f_i)_{i\in[2]}$.
% % \end{example}




% % To model this flexibility, we extend the firm action space by allowing each firm $f\in\FI$ to privately choose a binary hiring decision $\NH_f(t)$ at each time step $t$, where $\NH_f(t)=1$ indicates hiring and $\NH_f(t)=0$ indicates not hiring. Throughout the paper, we allow \emph{uncertain} firms to be strategic in this sense: in contrast to prior work, where firms were restricted to always hire, an uncertain firm may strategically refrain from hiring in selected rounds to cope with estimation error. The decision $\NH_f(t)$ is made after firm $f$ interviews its applicants and observes the applicant set $\APP_f(t)$. With this modification, we extend the reward previously defined in~\eqref{def:rewards1} to

% % {\small
% % \setlength{\abovedisplayskip}{-10pt}
% % \begin{align}\label{eq:reward}
% %     X_{a,\FM_a(t)}
% %     =
% %     \NH_{\FA_a(t)}\,
% %     X_{a,\FA_a(t)}\,
% %     \mathbb{1}\left\{\FM_a(t)\neq \emptyset\right\}.
% % \end{align}
% % }
% % Accordingly, in addition to designing agent-side algorithms, we introduce a \emph{strategic rejection policy}~(\cref{alg:fdrr}) that determines each firm’s hiring decision $\NH_f(t)$ each round. We call any firm with this extended action space (the ability to abstain from hiring) a \emph{strategic firm}, covering both certain and uncertain firms; in particular, \cref{alg:fdrr} ensures that every certain firm always hires, i.e., $\NH_f(t)=1$ for all $t$. We defer the formal policy description to~\cref{sec:uncertain-firms}.

% \end{comment}
 % \todo{\xw{the above paragraph tries to suggest the ``strategic firms'' are originated due to the ``uncertain firm.'' Here says both ``certain'' and ``uncertain'' are ``strategic.'' Either way, it would be better to let the readers know as early as possible, which type or both types are ``strategic''.}}






% \todo{\xw{add a discussion on why not strategic certain firms} \mo{add an intro paragraph and exclude all other cases where strategic does not matter.}}
%\todo{HB: I think this would fit better if we move to model section. \xw{revised}}

% While the setting of strategic uncertain firms adds complexity and potential sources of additional regret to the problem,
\vspace{-1em}
\subsection{Algorithmic Paradigms and Preliminaries} \label{sec:preliminaries}
\vspace{-0.5em}
Here, we first formally present two different algorithm design paradigms \emph{centralized} and \emph{decentralized}, and then introduce the preliminaries common to both.
% \vspace{-1em}

\textbf{Centralized vs. Decentralized Algorithms.}
We study two settings. In the \emph{centralized} setting, a coordinator allocates interviews to avoid collisions. In the \emph{decentralized} setting, agents choose interview sets independently, so multiple agents may apply to the same firm; such collisions must be resolved using firm-side feedback, either $\VF(t)$ or $\VFP(t)$. 

$\blacktriangleright$ \textit{Centralized algorithms.}
We assume an omniscient \textbf{C}entral \textbf{I}nterview \textbf{A}llocator ($\CIAP$) that observes the estimated preference lists of all agents and firms and selects the interview sets $\INT_a(t)$ at each round.

$\blacktriangleright$ \textit{Decentralized algorithms.}
Without $\CIAP$, each agent $a$ selects $\INT_a(t)$ from its \emph{local observations} (Definition~\ref{def:decentralized}), which include: (i) its estimated preference lists, (ii) whether its application was rejected, and (iii) the firm-side feedback from the previous round.

% \textbf{Algorithmic Paradigms: Degrees of Centralization.}\label{subsec:decentral-setup}
% We classify our algorithms according to their level of centralization into \emph{centralized} and \emph{decentralized} settings. In the decentralized setting, agents operate without an orchestrating center, so multiple agents may concurrently apply to the same firms, creating conflicts that must be resolved using the firm-side feedback they receive, either $\VF(t)$ or $\VFP(t)$. In contrast, the centralized setting resolves such conflicts directly through a central authority. 

% $\blacktriangleright$ \textit{Centralized algorithms.}
% We assume an omniscient oracle, referred to as the \textbf{C}entral \textbf{I}nterview \textbf{A}llocator ($\CIAP$), which observes the estimated preference lists of all agents and firms and determines the interview set $\INT_a(t)$ of each agent $a$ at every time step. With such centralization, agents no longer need to coordinate to avoid collisions, as conflicts are resolved by $\CIAP$ through careful interview allocation.

% $\blacktriangleright$ \textit{Decentralized algorithms.}
% In the decentralized counterpart, conflicts cannot be resolved by an external entity such as $\CIAP$, which is infeasible to maintain.  Instead, agents need to determine their interviewing sets $\INT_a(t)$ based on their \emph{Local Observations} (Definition~\ref{def:decentralized}), which include
% i) their current estimated preference lists,
% ii) whether they were rejected by the firm they applied to, and
% iii) the firm-side feedback revealed at the end of the previous round.

 % \amcomment{say something about conflicts and collisions here to give it a real meaning}
 % All algorithms build on the $\FGS$ procedure, which serves as their common backbone.
 

% \amcomment{reference for the word conflict, think about bringing the definition back, briefly mention what coordination is aiming for}





% Firm-side feedback enables agents to signal and coordinate their actions. 
% Under the vacancy-only feedback $\VF(t)$, an agent may intentionally refrain from reapplying to its current match, causing that firm to appear as vacant and hence be revealed to all agents in $\VF(t)$. Such vacancies can therefore serve as explicit coordination signals. 
% Under the richer feedback $\VFP(t)$, vacancies are also observed, but agents additionally receive anonymous information about hiring changes, which often makes coordination unnecessary by revealing market transitions directly.










\textbf{Algorithmic Preliminaries.}
Here, we introduce the preliminaries of our algorithmic designs.

% \textbf{Convergence.}
% From this point onward, we refer to the \emph{convergence} of a learning algorithm to a matching, which we formally define below. Intuitively, convergence occurs once all agents’ matches remain fixed thereafter. \amcomment{consider moving this whole section to the appendix}
% \amcomment{ellen's icml papers}



\textit{Empirical means as estimators.}
We use empirical averages to estimate expected utilities for each agent--firm pair \((a,f)\). For agent $a$ and firm $f$ at time $t$, the estimator is
$
    \hat{u}_{a,f}(t)
    = \frac{\sum_{t'=1}^{t} X_{a,f}(t')\, \mathbbm{1}\{f \in \INT_a(t')\}}{N_{a,f}(t)},
$
where $N_{a,f}(t) = \sum_{t'=1}^{t} \mathbbm{1}\{f \in \INT_a(t')\}$ is the number of interviews of $a$ at $f$ up to time $t$. For uncertain firms, the estimator $\hat{u}_{f,a}(t)$ is defined analogously.



\textit{The structure of the interview set $\INT_a(t)$}
Across all our algorithms, each agent interviews between two and $k$ firms per round, i.e., $2 \le |\INT_a(t)| \le k$. In the main body, we focus on the case $k=2$, i.e., showing only two interviews is sufficient for time-independent regret, and defer a special extension to unstructured markets with $k=3$ to~\cref{sec:noncoopgen}. The interviewing set is $\INT_a(t) = \{\RR_a(t), \FA_a(t)\}$, where $\FA_a(t)$ is the firm to which agent $a$ applies and $\RR_a(t)$ is selected in a round-robin manner for exploration, as follows.

$\blacktriangleright$ \textit{Interviewing round-robin firm $\RR_a(t)$.}
Each agent interviews a designated firm $\RR_a(t)$ such that over each block of $m$ rounds, every firm appears exactly once as the round-robin firm for every agent, ensuring uniform coverage. Formally, for agents indexed as $a_i$ and firms as $f_j$, we set $\RR_{a_i}(t) = f_{(t+i \bmod m)+1}$. This round-robin exploration resembles the exploration phase of Explore-then-Commit ($\texttt{ETC}$)  schemes~\citep{lattimore2020bandit}, but here it is specifically designed to achieve \emph{time-independent regret} rather than the $O(\log T)$ behavior typical of $\texttt{ETC}$.

$\blacktriangleright$ \textit{Interviewing to-be-applied firm $\FA_a(t)$.}
The other firm $\FA_a(t)$ that agent $a$ interviews with and applies to is chosen via the Gale–Shapley algorithm ($\FGS$) (or its distributed variant), which computes a stable matching with respect to the given preference lists of both sides.
% \mx{up to this point, this symbol of gale-shapley $\FGS$ is not introduced, which may lead to inconsistency; i would suggest adding one sentence explaining the context and definition of $\FGS$\amcomment{Done!}}.








% Since interviews serve as hints analogous to those in bandit-with-hints frameworks, we adopt the round-robin hint inquiry method of~\cite{bhaskara2023bandit,mirfakhar2025heterogeneous}, where each agent includes one round-robinly chosen firm in its interview set but never applies to it. 
% While similar in spirit to the Explore-then-Commit ($\texttt{ETC}$) strategy~\cite{lattimore2020bandit}—and to the round-robin $\texttt{ETC}$ approach of~\cite{zhangbandit} \amcomment{check the citation}—our goal is to achieve \emph{time-independent regret} rather than the usual $O(\log T)$ bound. 
% Accordingly, round-robin interviews are used purely for exploration: each agent applies only to the non–round-robin firm in $\INT_a(t)$, chosen based on current estimates, enabling $O(1)$ regret. 
% We formally define this round-robin interviewing procedure below.







==> model-new.tex <==
\section{System Model}\label{sec:model}

Consider a two-sided market $\MARK(\AG,\FI)$ with $n$ agents $\AG$ and $m$ firms $\FI$, where $n \leq m$.  
Each agent–firm pair $(a,f)$ is associated with two unknown reward distributions: $\DIS_{a,f}$ for agent $a \in \AG$, with mean $u_{a,f}$ (the expected utility of $a$ when matched with $f$), and $\DIS_{f,a}$ for firm $f \in \FI$, with mean $u_{f,a}$ (the expected utility of $f$ when matched with $a$).
% \todo{\xw{it would be better to use \(
%           v_{f,a}\) and \(\mathcal{G}_{f,a}\) for firms, to differ from those for agents.}\amcomment{dont get this one}}
For simplicity, we assume both distributions are independent across different pairs of agents and firms and across different time steps and that the rewards are bounded in $[0,1]$.
We also assume that for every agent $a \in \AG$ and any two distinct firms $f,f' \in \FI$, the expected utilities are distinct, i.e., $u_{a,f} \neq u_{a,f'}$.
Similarly, for every firm $f \in \FI$ and any two distinct agents $a,a' \in \AG$, we assume $u_{f,a} \neq u_{f,a'}$.

For each agent $a \in \AG$, the \emph{ground-truth preference list} $\PL_a$ is the ordering of firms in $\FI$ sorted in decreasing order of $u_{a,f}$.
For any list $L = \langle l_1, l_2, \ldots \rangle$, we write $l_i \underset{L}{>} l_j$ if $l_i$ is ranked higher than $l_j$ in $L$.
For instance, $f_i \underset{\PL_a}{>} f_j$ means that agent $a$ prefers firm $f_i$ to firm $f_j$ in the ground-truth preferences, i.e., $u_{a,f_i} > u_{a,f_j}$.

% When an agent $a$ is matched to a firm $f$, the agent receives a stochastic reward drawn from an unknown distribution $\DIS_{a,f}$ with mean $u_{a,f}$, and the firm receives a stochastic reward drawn from an unknown distribution $\DIS_{f,a}$ with mean $u_{f,a}$.

\paragraph{Sequential Decision Process.}
Given \(T \in \mathbb{N}^+\) rounds of interaction between agents and firms,  
we now describe the sequential interaction dynamics between agents and certain firms (with the extension to uncertain firms presented later),  
consisting of three stages:\footnote{Before the interview stage, there is often an outreach stage where agents contact firms to request interviews. Since the outreach stage does not yield any observations or rewards, we omit it here for simplicity.} \emph{interview}, \emph{application}, and \emph{firm-side feedback revelation}: In each round \(t\in[T]\),

$\blacktriangleright$ \emph{Interview stage.}
           Each agent $a \in \AG$ selects a subset of firms $\INT_a(t) \subseteq \FI$ to interview\footnote{Although we refer to this stage as an \emph{interview}, it is more akin to an open house or participation in a career fair.}, with size $2 \leq |\INT_a(t)| \leq k$, where $k \in \mathbb{N}^+$ is the \emph{interview budget}.  
        For each interviewed firm $f \in \INT_a(t)$, the agent observes a stochastic signal $X_{a,f}(t) \sim \DIS_{a,f}$ drawn from distribution $\DIS_{a,f}$ with mean $u_{a,f}$; these signals are not counted as rewards.  
        Similarly, each firm $f$ interviews agents in $\INT_f(t)$ and observes $X_{f,a}(t) \sim \DIS_{f,a}$ for each $a \in \INT_f(t)$.

$\blacktriangleright$ \emph{Application stage.}
           After obtaining the interview results, agent \(a\) applies to one of the interviewed firms \(\FA_a(t)\in\INT_a(t)\).
           \begin{itemize}
                \item Each firm \(f\in\FI\) then collects all applications from agents, denoted by \(\APP_f(t)=\{a\in\AG:\FA_a(t)=f\}\).
                % \todo{\xw{it would be better to use \(\mathcal{A}_f(t)\).}\amcomment{that is reserved for the set of agents}}
                      If \(\APP_f(t)\neq\emptyset\), firm \(f\) admits its most preferred applicant \(\FFM_f(t) = \{a \in \APP_f(t) :  a \underset{\PL_f}{>} a', \forall_{a' \in \APP_f(t)\setminus a} \}\) among those in \(\APP_f(t)\) according to its preference.
                \item
                      If \(\FFM_{\FA_a(t)}(t) = a\), then agent \(a\) is hired by firm \(\FA_a(t)\) and receives a stochastic reward \(X_{a,\FA_a(t)}(t)\sim \DIS_{a,\FA_a(t)}\); otherwise, agent \(a\) receives no reward.
                      We denote the final match of agent $a$ at round $t$ by
                      \(\FM_a(t)\)
                      where $\FM_a(t) = \FA_a(t)$ if $a$ is admitted by its applied firm, and $\FM_a(t) = \emptyset$ otherwise.
                      The final match of firm $f$ is similarly denoted as $\FFM_f(t)$.
                \item Agent $a$ receives 
                \begin{align}
                    \quad\quad X_{a,\FM_a(t)}=X_{a,\FA_a(t)}\cdot\mathds{1}\left\{\FM_a(t) = \FA_a(t) \right\}\label{def:rewards1}
                \end{align} as its reward.
        
           \end{itemize}
$\blacktriangleright$ \emph{Firm-Side Feedback Revelation stage.}
At the end of each round $t$, agent $a$ observes the firm-side feedback, which, depending on the setup, can be either $\VF(t)$ or $\VFP(t)$, defined as
\begin{align}
    \VF(t)   &= \{f \in \FI : \FFM_f(t) = \emptyset\},\\
    \VFP(t)  &= \VF(t)\cup\{f \in \FI : \FFM_f(t-1) \neq \FFM_f(t)\},
\end{align}
where $\VF(t)$ is the set of only firms with vacant positions and $\VFP(t)$ the set of firms with vacancies or whose hiring status has changed. These feedbacks---$\VF(t)$ as the weaker and $\VFP(t)$ as the stronger---are crucial for the design of our decentralized algorithms, whereas in the centralized setting, agents do not rely on them.



% The reward of agent $a$ at time $t$ is then
% \begin{align}
%       & X_{a,\FM_a(t)}(t) \nonumber
%      \\
%       & \qquad  =
%      \begin{cases}
%           \NH_{\FA_a(t)}.X_{a,\FA_a(t)}(t), & \text{if } \FM_a(t) = \FA_a(t)  \\[6pt]
%           0                                 & \text{if } \FM_a(t) = \emptyset
%      \end{cases}.
%      \label{eq:reward}
% \end{align}

\paragraph{Uncertain Firm Extension.}  
To generalize the model, we allow firms to act strategically by choosing not to hire in a given round after interviewing applicants. This flexibility is crucial for learning stable matchings via decentralized, and ideally coordination-free, algorithms when firms are uncertain about their preferences. Accordingly, each firm $f \in \FI$ privately maintains a binary variable $\NH_f(t)$ at each time step $t$ indicating its hiring decision: $\NH_f(t) = 1$ if $f$ hires, and $\NH_f(t) = 0$ otherwise. This variable is set after firm $f$ interviews and observes its set of applicants $\APP_f(t)$. For \emph{certain} firms, which know their preference lists in advance, we assume $\NH_f(t) = 1$ for all $t$. For \emph{uncertain} firms, which instead learn their preferences through interviewing and hiring, $\NH_f(t)$ is decided strategically, allowing them to deliberately pause hiring to potentially improve the quality of future matches.\todo{\xw{Is ``uncertain firm'' the right name? How about ``strategic firm''? It is not only uncertain preference, as studied in this paper~\citep{zhangbandit}, but also a space for decision-making to pick \(\gamma\). Also, certain firms can be strategic, right?}} At the same time, this forces agents to reconsider such firms, as they strategically place themselves in the firm-side feedback sets $\VF(t)$ or $\VFP(t)$. While designing algorithms we also describe the algorithm employed by the uncertain firms to set $\NH(_f(t)$ at each round. With this modification, we extend the reward previously defined in~\eqref{def:rewards1} to
{\small
\begin{align} \label{eq:reward}
     X_{a,\FM_a(t)} = \NH_{\FA_a(t)} \cdot X_{a,\FA_a(t)} \cdot \mathds{1}\left\{\FM_a(t) = \FA_a(t) \right\}.
\end{align}
}
 We show that, since learning stability is the core objective, this mechanism benefits both sides, especially in the decentralized case, as it incentivizes uncertain firms to adaptively refuse to hire. 





\paragraph{Optimal and Pessimal Regrets.}
For any learning policy $\Pi$, we define regret to evaluate its performance in learning a stable matching from the perspective of the agents.  Since multiple stable matchings may exist, our goal is to design algorithms that allow agents to learn the agent-optimal stable matching whenever possible, and otherwise converge to the agent-pessimal one.

Following the prior work by~\citet{liu2021bandit}, we define the \emph{optimal} and \emph{pessimal} regrets under policy \(\Pi\) for agent $a$ over $T$ rounds as follows
     {\small
          \begin{align}
               \text{Optimal Regret}:\ \mathbb{E}[\overline{R}_a(\Pi,T)]\doteq T  u_{a,\overline{f^*_a}}-\sum_{t=1}^T \mathbb{E}[ X_{a, \FM_a(t)}(t) ], \label{eq:optreg} \\
               \text{Pessimal Regret}:\ \mathbb{E}[\underbar{R}_a(\Pi,T)]\doteq T  u_{a,\underline{f^*_a}}-\sum_{t=1}^T \mathbb{E}[ X_{a, \FM_a(t)}(t) ]\label{eq:pessreg},
          \end{align}
     }
where $\overline{f^*_a}$ and $\underline{f^*_a}$ are the best and worst stable matches of agent $a$.
When the market only has a unique stable matching, the pessimal and optimal regret are identical.
For brevity, we omit the learning policy $\Pi$ and denote the regrets as $\mathbb{E}[\overline{R}_a(T)]$ and $\mathbb{E}[\underbar{R}_a(T)]$ in the remainder of this work. For each agent $a \in \AG$ and firm $f \in \FI$, we define the optimal utility gap as $\overline{\Delta}_{a,f} \doteq |u_{a,\overline{f^*_a}} - u_{a,f}|$ and the pessimal utility gap as $\underline{\Delta}_{a,f} \doteq |u_{a,\underline{f^*_a}} - u_{a,f}|$. \footnote{Analogously, we define the optimal utility gap as $\overline{\Delta}_{f,a} \doteq |u_{f,\underline{a^*_f}} - u_{f,a}|$ and the pessimal utility gap as $\underline{\Delta}_{f,a} \doteq |u_{f,\overline{a^*_f}} - u_{f,a}|$, where $\overline{a^*_f}$ and $\underline{a^*_f}$ denote the firm-optimal and pessimal stable matches for firm $f$, noting that the agent-optimal matching is firm-pessimal and vice versa~\cite{gale1962college}.}
For markets with a unique stable matching, we drop the overlines and underlines, denoting regret and utility gaps as $\mathbb{E}[R_a(T)]$, $\Delta_{a,f}$, and $\Delta_{f,a}$. Within this class, we focus on $\alpha$-reducible markets, first studied in the context of uniqueness by~\citet{clark2006uniqueness} and later adopted by~\citet{maheshwari2022decentralized} for coordination-free decentralized bandit learning. This assumption is weaker than the widely used serial dictatorship markets~\citep{sankararaman2021dominate,wang2024optimal}, yet covers a broader family of unique stable matching markets.



\paragraph{$\alpha$-Reducible Markets}
A pair $(a, f) \in \AG \times \FI$ is called a \emph{fixed pair} in a market $\MARK$ if agent $a$ ranks firm $f$ as its top choice, i.e.,
\[
     f \underset{O_a}{>} f' \quad \text{for all } f' \in \FI \setminus \{f\},
\]
and firm $f$ likewise ranks agent $a$ as its top choice, i.e.,
\[
     a \underset{O_f}{>} a' \quad \text{for all } a' \in \AG \setminus \{a\}.
\]

% \mo{I know that the name $\ alpha$-reducible is used in prior work, but it is not a descriptive name, and also the reader expects to see the role $\alpha$ in this def. Any chance of describing why this name is used and/or changing it to something more descriptive if it is used only in [13]? ok, I checked [13] and it seems that they also used from other refs, then we should also ref those initial work.}
% \todo{\xw{give the definition of \(\underset{O_f}{>}\) }\amcomment{it is already defined in the model}}


\begin{definition}
     A market $\MARK(\AG, \FI)$ is \emph{$\alpha$-reducible} if every sub-market of $\MARK(\AG, \FI)$---that is, $\MARK(\AG', \FI')$ with \(\AG' \subseteq \AG\) and \(\FI' \subseteq \FI\)---contains a fixed pair.
\end{definition}
When analyzing an $\alpha$-reducible market, we index agents and firms as $a_i$ and $f_i$, respectively. By definition, such a market contains an agent–firm pair that mutually rank each other as their top choice, denoted $(a_1, f_1)$. Removing this pair leaves a sub-market that remains $\alpha$-reducible, yielding another mutually top-ranked pair $(a_2, f_2)$. Repeating this process produces a sequence of pairs $(a_i, f_i)_{i \in [n]}$ that together form the unique stable matching of the market.

While our centralized and decentralized algorithms apply to general markets, we first focus on $\alpha$-reducible markets in the decentralized case. Their layered structure simplifies the analysis, allowing us to illustrate the main proof ideas and establish bounds matching the centralized case. We then extend our considerations to general markets.




% \tdmark~to incorporate in above:

% At the end of each time step, the set of firms that remain unmatched—either because they chose not to hire ($\NH_f(t)=0$) or because no agent applied to them—is revealed to all agents. We denote this set by
% \[
%      \VF(t) \doteq \{f \in \FI : \NH_f(t) = 0 \ \lor\ (\nexists a \in \AG,\  \FA_a(t) = f)\}.
% \]
% Thus, at each time step $t$, every agent observes $\VF(t)$, i.e., the set of firms with vacant positions at the end of the previous step $t-1$, which serves as the information available for decision-making at time $t$.



\section{Algorithm Design Paradigms and Preliminaries}
In this section, we first present two different algorithm design paradigms, followed by the preliminaries common to all algorithms (both centralized and decentralized).

\subsection{Algorithmic Paradigms: Degrees of Centralization}

We classify the proposed algorithms into two categories based on their degree of centralization: \emph{centralized} and \emph{decentralized}, with the latter further distinguished by the type of firm-side feedback, $\VF(t)$ or $\VFP(t)$. All of our algorithms use $\FGS$ as a backbone, described as follows.

\paragraph{Centralized Algorithms}  
We assume an omniscient oracle, referred to as the \textbf{C}entral \textbf{I}nterview \textbf{A}llocator ($\CIAP$), which observes the estimated preference lists of all, certain or uncertain, firms and runs $\FGS$ to specify one of the firms in the interview set $\INT_a(t)$ of agent $a$ at each time step. With such centralization, agents do not need to coordinate, as all conflicts are resolved by $\CIAP$.

$\blacktriangleright$ \textbf{Decentralized Algorithms.}  
In the decentralized setup, conflicts are not resolved by an external entity like $\CIAP$. Instead, agents determine their interviewing sets $\INT_a(t)$ based on local observations defined as \begin{definition}[Local Observations]\label{def:decentralized}
In the \emph{decentralized} setup, each agent $a \in \AG$ updates its interviewing set $\INT_a(t)$ solely based on its own local observations at time $t$, which include:
\begin{enumerate}
    \item Changes in its estimated preference list $\EPL_a(t-1)$ to $\EPL_a(t)$.
    \item Whether it was rejected by the applied firm $\FA_a(t-1)$.
    \item The firm-side feedback $\VF(t-1)$.
\end{enumerate}
\end{definition} 
Firm-side feedback, however, enables implicit coordination. For instance, under $\VF(t)$, an agent $a$ may refuse to apply to its previous match $\FM_a(t-1)$, leaving that firm vacant, i.e., $\FM_a(t-1)\in \VF(t)$, which is then revealed to all agents who may reconsider that firm. Accordingly, we design decentralized learning algorithms under both feedback models: with $\VF(t)$, agents must coordinate to distributedly run $\FGS$ under weaker feedback, whereas with $\VFP(t)$, we can design coordination-free algorithms in which each agent independently follows its own thread of distributed $\FGS$, applicable to both certain and uncertain firms.

\todo{\xw{add a discussion on why not strategic certain firms}}




\subsection{Algorithms Preliminaries}
\paragraph{Empirical Means as Estimators}
We use empirical averages to estimate expected utilities for each agent--firm pair. For agent $a$ and firm $f$ at time $t$, the estimate is
\[
     \hat{u}_{a,f}(t) = \frac{\sum_{t'=1}^{t} X_{a,f}(t') \, \mathds{1}\{f \in \INT_a(t')\}}{N_{a,f}(t)},
\]
where $N_{a,f}(t) = \sum_{t'=1}^{t} \mathds{1}\{f \in \INT_a(t')\}$ is the number of interviews of $a$ at $f$ up to time $t$.  
For uncertain firms, $\hat{u}_{f,a}(t)$ is defined analogously. The preference lists induced by these estimates at time $t$ are the \emph{estimated preference lists}, denoted $\EPL_a(t)$ for agents and $\EPL_f(t)$ for firms.  
If firms are \emph{certain}, then $\hat{u}_{f,a}(t) = u_{f,a}$ and $\EPL_f(t) = \PL_f(t)$ for all $t \in [T]$.  
If firms are \emph{uncertain} and choose to hire ($\NH_f(t)=1$), they admit their most preferred applicant according to $\EPL_f(t)$, i.e.,
\(
   \FFM_f(t) = \{a \in \APP_f(t) : a \underset{\EPL_f(t)}{>} a', \forall a' \in \APP_f(t)\}.
\)


\paragraph{Interview Set $\INT_a(t)$ Structure}
Across all our algorithms, each agent interviews with at most two firms per round, $|\INT_a(t)| \leq 2$, and applies to one of them. Our analysis shows that this suffices to achieve time-independent regret while learning a stable matching in a competitive setting. We denote these firms by $\FA_a(t)$ and $\RR_a(t)$, so that $\INT_a(t) = \{\RR_a(t), \FA_a(t)\}$, where $\FA_a(t)$ is the firm to which the agent applies, and $\RR_a(t)$ is used purely for exploration. Since interviews serve as hints analogous to those in bandit-with-hints frameworks, we adopt the round-robin hint inquiry method of~\cite{bhaskara2023bandit,mirfakhar2025heterogeneous}, where each agent includes one round-robinly chosen firm in its interview set but never applies to it. While this approach resembles the Explore-then-Commit ($\texttt{ETC}$) strategy~\cite{lattimore2020bandit}—and~\cite{zhangbandit} also studies a round-robin $\texttt{ETC}$ scheme in matching markets with uncertain firms—our objective is to achieve \emph{time-independent regret}, rather than the typical $O(\log T)$ guarantees. \amedit{To this end, we use round-robin interviewing solely for exploration: each agent applies only to the non–round-robin firm in $\INT_a(t)$, selected by the algorithm from current estimates, which enables time-independent $O(1)$ regret. Formally, the round-robin interviewing procedure—used by all our algorithms—is defined as follows.}


\paragraph{Interviewing Round-Robin Firm $\RR_a(t)$.}
Each agent $a$ includes a designated firm $\RR_a(t)$, chosen in a round-robin manner, in its interview set $\INT_a(t)$. Over each block of $m$ rounds, every firm appears exactly once as the round-robin firm for each agent, ensuring uniform coverage. Formally, we define
\(
\RR_{a_i}(t) = f_{\,(t+i \bmod m) + 1},
\) 
for $i \in [n]$. 

\paragraph{Interviewing To-Be-Applied Firm $\FA_a(t)$.}
The second firm in $\INT_a(t)$, denoted by $\FA_a(t)$, is the one to which agent $a$ applies. Such choice, determined by each algorithm,  varies across rounds depending on the setup, always through an $\FGS$-based procedure over estimated preference lists.







==> model.tex <==
\section{Model}
\amcomment{mobve the stuff required for the algorithm desing and not the model}
\mo{overall, I feel model section is too long, let's dicuss it in the meeting today, but some parts belong to algorithm section, e.g., keeping track of estimates and notations around that, e.g., $\hat{u}$ is something that is not needed in this section since this is something that the alg defines and uses. having a long model section will increase the risk of getting lost and missing what is the actual contribution of the paper. }
We consider a two-sided market $\MARK(\AG,\FI)$ with a set of $n$ agents $\AG$ and $m$ firms $\FI$ \todo{\xw{it is better to use \(A\) for the number of agents, and \(F\) for the number of firms. making the notation consistent}} such that $n \leq m$. Each agent $a \in \AG$ has a valuation $u_{a,f}$ to each firm $f \in \FI$, and each firm $f \in \FI$ has a valuation $u_{f,a}$ to each agent $a \in \AG$.
These valuations are the means of independent reward distributions supported on $[0,1]$, i.e., $u_{a,f} = \mathbb{E}_{X \sim \DIS_{a,f}}[X]$ and $u_{f,a} = \mathbb{E}_{Y \sim \DIS_{f,a}}[Y]$. We also assume that for every agent $a \in \AG$ and any two distinct firms $f,f' \in \FI$, the expected utilities are distinct, i.e., $u_{a,f} \neq u_{a,f'}$.


In general, both agents and firms may be uncertain about their preferences.
Throughout this work, we always assume that agents are uncertain, while firms may be either certain or uncertain depending on the context under consideration.
This naturally fits into a \textbf{M}ulti-\textbf{A}gent \textbf{M}ulti-\textbf{A}rmed \textbf{B}andit ($\texttt{MA2B}$) perspective: over $T \in \mathbb{N}$ rounds, agents repeatedly choose firms (arms), while firms, guided by their current preferences, decide which applicants to accept. To strengthen the learning process, we further allow agents to maintain auxiliary information through \emph{interviews}, in addition to the standard feedback from arm pulls. These interviews play a crucial role in enabling agents to achieve time-independent regret—a standard benchmark in the bandit literature for evaluating online learning algorithms.

\mo{the following paragraph could be moved to the next section.}
Before describing the interaction dynamics, we introduce notation for the metrics used to make decisions under uncertainty.
At each round $t \in [T]$, agents and firms base their choices on estimates of utilities for the opposite side of the market, updated from past observations.
Each agent $a$ maintains an estimate $\hat{u}_{a,f}(t)$ of its expected utility for firm $f$, and each firm $f$ maintains an estimate $\hat{u}_{f,a}(t)$ for agent $a$.
When preferences are uncertain, these estimates may deviate from the true valuations $u_{a,f}$ and $u_{f,a}$; when preferences are certain, they coincide with the true values at all times.
For instance, if all firms in $\FI$ know their exact valuations from the outset, then $\hat{u}_{f,a}(t) = u_{f,a}$ for every $t \in [T]$.
Throughout this work, we assume that estimates are maintained using empirical means, a standard choice in bandit learning, and formalize this in the following.

\mo{Similarly, the part related to the estimated preference list could be moved to the next section. }
Having defined the utilities and their estimates, we now introduce the preference lists.
For each agent $a \in \AG$, the \emph{ground-truth preference list} $\PL_a$ is the ordering of firms in $\FI$ sorted in decreasing order of $u_{a,f}$.
Similarly, for each firm $f \in \FI$, the ground-truth preference list $\PL_f$ is the ordering of agents in $\AG$ sorted in decreasing order of $u_{f,a}$. At each time step $t$, we define the \emph{estimated preference lists}.
For agent $a$, the estimated list $\EPL_a(t)$ is the ordering of firms by their estimated utilities $\hat{u}_{a,f}(t)$, and for firm $f$, the estimated list $\EPL_f(t)$ is the ordering of agents by $\hat{u}_{f,a}(t)$.
For any list $L = \langle l_1, l_2, \ldots \rangle$, we write $l_i \underset{L}{>} l_j$ if $l_i$ is ranked higher than $l_j$ in $L$.
For instance, $f_i \underset{\PL_a}{>} f_j$ means that agent $a$ prefers firm $f_i$ to firm $f_j$ in the ground-truth preferences, i.e., $u_{a,f_i} > u_{a,f_j}$.
The same notation applies to estimated lists; in particular, if
\(
\EPL_a(t) = \langle f_1, f_2, \ldots, f_m \rangle,
\)
then $\hat{u}_{a,f_i}(t) \geq \hat{u}_{a,f_j}(t)$ for all $j \geq i$.

We now describe the interaction dynamics between agents and firms, consisting of three stages: \emph{outreach}, \emph{interview}, and \emph{application}.
These stages aim to gather competitive information, refine utility estimates, and ultimately reach stable matches.
To generalize the model, we allow firms the option of not hiring any agent in a given round, a feature crucial for designing decentralized algorithms with uncertain firms. At each time step $t$, a binary variable $\NH_f(t)$, private to firm $f \in \FI$, indicates its hiring decision: $\NH_f(t) = 1$ if $f$ hires and $\NH_f(t) = 0$ otherwise. In the case of certain firms we assume $\NH_f(t) = 1$ for all $t$, while in the uncertain case firms may deliberately choose $\NH_f(t) = 0$ to improve the quality of their eventual hires.
Remaining unmatched at the end of a round incurs a cost for agents, forcing them to balance pursuing highly preferred firms with the risk of receiving no match.

At each round $t \in [T]$, every agent $a$ first engages in the \emph{outreach} stage by contacting a subset $\RO_a(t) \subseteq \FI$ of firms, chosen according to its estimated preference list $\EPL_a(t)$. The set of agents who reach out to firm $f$ is denoted $\RO_f(t) \subseteq \AG$, and the firm ranks these agents using its estimated list $\EPL_f(t)$. In the \emph{interview} stage, firm $f$ selects a subset $\INT_f(t) \subseteq \RO_f(t)$ for interviews.
We assume that whenever $|\RO_f(t)| \geq 2$, the firm interviews at least two of these agents, i.e., $|\INT_f(t)| \geq 2$, a condition necessary for achieving time-independent regret.
Since under our algorithms each firm is guaranteed to be contacted by at most two agents, we may, without loss of generality, identify $\RO_a(t)$ with $\INT_a(t)$.
Thus, when we refer to $\INT_a(t)$ or $\RO_a(t)$, symmetrically, we mean the set of firms to which agent $a$ both reaches out and interviews.
In most of this work, we focus on the case $\RO_a(t) = 2$, with a special case analyzing $\RO_a(t) = 3$.
\amcomment{Not sure whether to include this part explicitly; may be revised.} For each interviewing pair $(a,f)$ with $a \in \INT_f(t)$ and $f \in \INT_a(t)$, the \emph{interviewing phase} yields observations: the agent draws $X_{a,f}(t) \sim \DIS_{a,f}$ and the firm draws $Y_{f,a}(t) \sim \DIS_{f,a}$.
These observations are then used to update the estimates $\hat{u}_{a,f}(t)$ and $\hat{u}_{f,a}(t)$.  In the \emph{application} stage, each agent $a$ chooses a subset of interviewed firms $\APP_a(t) \subseteq \INT_a(t)$ and then applies to a single firm $\FA_a(t) \in \APP_a(t)$.
Each hiring firm $f$ with $\NH_f(t)=1$ admits its most preferred applicant among those with $\FA_a(t) = f$ and rejects the rest.
We denote the final match of agent $a$ at round $t$ by
\(
\FM_a(t) \in \{\FA_a(t), \emptyset\},
\)
where $\FM_a(t) = \FA_a(t)$ if $a$ is admitted by its applied firm, and $\FM_a(t) = \emptyset$ otherwise. The final match of firm $f$ is similarly denoted by $\FFM_f(t)$. The reward of agent $a$ at time $t$ is then

     {\small
          \begin{align} \label{eq:reward}
               X_{a,\FM_a(t)}(t) \;=\;
               \begin{cases}
                    \NH_{\FA_a(t)}.X_{a,\FA_a(t)}(t), & \text{if } \FM_a(t) = \FA_a(t),  \\[6pt]
                    0,                                & \text{if } \FM_a(t) = \emptyset.
               \end{cases}
          \end{align}
     }
At the end of each time step, the set of firms that remain unmatched—either because they chose not to hire ($\NH_f(t)=0$) or because no agent applied to them—is revealed to all agents. We denote this set by
\[
     \VF(t) \doteq \{f \in \FI : \NH_f(t) = 0 \ \lor\ (\nexists a \in \AG,\  \FA_a(t) = f)\}.
\]
Thus, at each time step $t$, every agent observes $\VF(t)$, i.e., the set of firms with vacant positions at the end of the previous step $t-1$, which serves as the information available for decision-making at time $t$. This three-stage process induces competition among agents, who must not only consider their own preferences but also anticipate the preferences and choices of firms.



For any learning policy $\Pi$, we define regret to evaluate its performance in learning a stable matching from the perspective of the agents.  Since multiple stable mathchings may exist, our goal is to design algorithms that allow agents to learn the agent-optimal stable matching whenever possible, and otherwise converge to the agent-pessimal one.
Because these outcomes are inherently agent-centric (with agents acting as proposers), we focus on algorithms that achieve time-independent regret for agents.
As learning the agent-optimal stable matching may be impossible in some cases, we follow~\cite{liu2021bandit} and define both \emph{optimal} and \emph{pessimal} regrets.  The expected regret of policy $\Pi$ for agent $a$ over $T$ rounds is

     {\small
          \begin{align}
               \text{Optimal Regret}:\ \mathbb{E}[\overline{R}_a(\Pi,T)]\doteq T  u_{a,\overline{f^*_a}}-\sum_{t=1}^T \mathbb{E}[ X_{a, \FM_a(t)}(t) ], \label{eq:optreg} \\
               \text{Pessimal Regret}:\ \mathbb{E}[\underbar{R}_a(\Pi,T)]\doteq T  u_{a,\underline{f^*_a}}-\sum_{t=1}^T \mathbb{E}[ X_{a, \FM_a(t)}(t) ]\label{eq:pessreg},
          \end{align}
     }
where $\overline{f^*_a}$ and $\underline{f^*_a}$ are the optimal and worst stable match of agent $a$. For the case of matching markets $\MARK$ with unique stable matching the pessimal and optimal regret are identical. For notational simplicity, we drop the dependence on the learning policy $\Pi$ and denote the regret as $\mathbb{E}[\overline{R}_a(T)]$ in the remainder of this work.

For each agent $a \in \AG$ and firm $f \in \FI$, we define the optimal utility gap as $\overline{\Delta}_{a,f} \doteq |u_{a,\overline{f^*_a}} - u_{a,f}|$ and the pessimal utility gap as $\underline{\Delta}_{a,f} \doteq |u_{a,\underline{f^*_a}} - u_{a,f}|$. Analogously, for each firm $f \in \FI$ and agent $a \in \AG$, we define the optimal utility gap as $\overline{\Delta}_{f,a} \doteq |u_{f,\underline{a^*_f}} - u_{f,a}|$ and the pessimal utility gap as $\underline{\Delta}_{f,a} \doteq |u_{f,\overline{a^*_f}} - u_{f,a}|$, where $\overline{a^*_f}$ and $\underline{a^*_f}$ denote the firm-optimal and pessimal stable matches for firm $f$, noting that the agent-optimal matching is firm-pessimal and vice versa.








\subsection{$\alpha$-Reducible Markets}
Among markets with a unique stable matching, we focus on \emph{$\alpha$-reducible markets}, introduced by~\cite{maheshwari2022decentralized} in the context of decentralized learning. Their layered structure is central to our analysis and the design of our algorithms. Examples include globally ranked and serial-dictatorship markets, both known to guarantee uniqueness of stable matchings.

A pair $(a, f) \in \AG \times \FI$ is called a \emph{fixed pair} in a market $\MARK$ if agent $a$ ranks firm $f$ as its top choice, i.e.,
\[
     f \underset{O_a}{>} f' \quad \text{for all } f' \in \FI \setminus \{f\},
\]
and firm $f$ likewise ranks agent $a$ as its top choice, i.e.,
\[
     a \underset{O_f}{>} a' \quad \text{for all } a' \in \AG \setminus \{a\}.
\]

\begin{definition}
     A market $\MARK = (\AG, \FI)$ is \emph{$\alpha$-reducible} if every sub-market of $\MARK$ contains a fixed pair.
\end{definition}



\subsection{Empirical Means as Estimation Statistics}
We focus on empirical means as the estimation metric. For agent $a$ and firm $f$ at time $t$, the estimate is
\[
     \hat{u}_{a,f}(t) = \frac{\sum_{t'=1}^{t} X_{a,f}(t') \, \mathbbm{1}\{f \in \INT_a(t')\}}{N_{a,f}(t)},
\]
where $N_{a,f}(t)$ is the number of interviews between $a$ and $f$ up to time $t$. For uncertain firms, $\hat{u}_{f,a}(t)$ is defined analogously. These estimates suffice to learn the stable matching and guarantee time-independent regret.



% \fbox{\begin{minipage}{31em}
% The following model, that can serve as the main model, fits well with the idea of decentralization on $\alpha$-reducible markets. Under this model, 
% \begin{enumerate}
%     \item Each agent applies to and interviews with the firms in $A_a(t)$ and $I_a(t)$ respectively.

%     \item Then each agent is matched with the most preferred firm which is not matched 
% \end{enumerate}

% \end{minipage}}
% \subsection{Notes}
% \begin{enumerate}
%     \item \textbf{Effect on Observations:} The parameter \(\intesize\) controls the number of observations (i.e., applications or interviews) an agent can make in each round. 
%     \begin{itemize}
%         \item It is important to understand how \(\intesize\) shapes the learning dynamics. In particular, we ask: for what values of \(\intesize\) does the bandit problem effectively reduce to an expert setting? Notably, when \(\intesize \geq cK\) for some constant \(c \in (0,1)\), the problem resembles a stochastic expert problem, where exploration is less constrained.
%     \end{itemize}

%     \item \textbf{Constraint on Matching:} The value of \(\intesize\) also serves as a structural constraint in the matching process: agents can only be matched with firms that belong to their applied subset of size at most \(\intesize\).

%     \item \textbf{Special Case—No Firm Preferences:} When firms are indifferent among agents (i.e., the firm side has no preferences), the model reduces to a heterogeneous reward setting, as studied in~\cite{shi2021heterogeneous}.
% \end{enumerate}






==> unique_vs_multi.tex <==
\subsection{Multiple \textit{vs} Unique Stable Matchings}
There is a notable argument in \cite{liu2020competing} regarding the difference in regret bounds for the $\ETC$ and $\UCB$ algorithms. The authors define \emph{optimal regret} for the $\ETC$ algorithm by comparing its performance to the best stable matching, while they analyze \emph{pessimal regret} for the $\UCB$ algorithm by comparing it to the worst stable matching. Before delving into the intuition behind using different regret definitions for centralized $\ETC$ and $\UCB$, it is important to note that the existence of both worst and best stable matchings implies at least two stable equilibria. In markets with only one stable matching, pessimal and optimal regrets converge.


\begin{theorem}\label{thm:uniqucb}
According to regret definition 
\begin{align*}
     \text{Pessimal Regret}:\quad\overline{R}_a(T)\doteq T  u_a(\overline{f^*_a})-\sum_{t=1}^T \mathbb{E}[ X_{a, f_a(t)}(t)], \\
     \text{Optimal Regret}:\quad\underbar{R}_a(T)\doteq T  u_a(\underline{f^*_a})-\sum_{t=1}^T \mathbb{E}[ X_{a, f_a(t)}(t)],\\
\end{align*}
where $\overline{f^*_a}$ and $\underline{f^*_a}$ are the optimal and worst stable match of agent $a$. Then, $\UCB$ algorithm can always achieve sub-linear regret according to pessimal regret.  
\end{theorem}

Before proving Theorem \ref{thm:uniqucb}, we refer to an example from \cite{liu2020competing} which clarifies why centralized $\UCB$ can not always find the optimal stable matching while more than one stable matching exist.

\begin{example}\label{examp:ucb}
    Let $\mathcal{A}=$ $\left\{a_1, a_2, a_3\right\}$ and $\mathcal{F}=\left\{f_1, f_2, f_3\right\}$, with true preferences given by:

$$
\begin{array}{lr}
a_1: \langle f_1 \succ f_2 \succ f_3\rangle &  f_1:\langle a_2 \succ a_3 \succ a_1\rangle \\
a_2: \langle f_2 \succ f_1 \succ f_3 \rangle & f_2:\langle a_1 \succ a_2 \succ a_3\rangle\\
a_3:\langle f_3 \succ f_1 \succ f_2 \rangle & f_3: \langle a_3 \succ a_1 \succ a_2 \rangle\\
\end{array}
$$


The agent-optimal stable matching is $\left(a_1, f_1\right),\left(a_2, f_2\right),\left(a_3, f_3\right)$. When $a_3$ incorrectly ranks $f_1 \succ f_3$ and the other two players submit their correct rankings, the Gale-Shapley Platform outputs the matching $\left(a_1, f_2\right),\left(a_2, f_1\right),\left(a_3, f_3\right)$. In this case $a_3$ will never correct their mistake because they never get matched with $f_1$ again, and hence their upper confidence bound for $f_1$ will never shrink.
\end{example}

This example highlights how even small inaccuracies in any agent’s preference list can influence the outcome of $\FGS$, especially when $\UCB$ estimations guide the process. It is implied by the Theorem \ref{thm:uniqucb} following parts that such bad events cannot occur when either $\UCB$ is compared with the pessimal stable matching or when only a unique stable matching exists. Furthermore, we argue that information acquisition, through interviews or hints, can resolve the issue presented in Example \ref{examp:ucb}.

We begin the proof of Theorem \ref{thm:uniqucb} by analyzing a special case presented in Lemma \ref{lemma:uniq}, where the presence of a unique stable matching ensures that the pessimal and optimal matchings are equivalent.

\begin{lemma}\label{lemma:uniq}
    In markets with a unique stable matching, the $\UCB$ algorithm guarantees sub-linear regret when compared to both the pessimal and optimal stable regrets.
\end{lemma}

a direct implication of Lemma \ref{lemma:uniq}, hands us with the Corollary \ref{cor:uniqalpha} about the $\alpha$-reducible markets which are guaranteed to have a well-structured unique stable matching we described above. The proof of Corollary $\ref{cor:uniqalpha}$ provides a good vision about the main idea in the proof of Lemma \ref{lemma:uniq}.

\begin{corollary}\label{cor:uniqalpha}
In $\alpha$-reducible markets, the $\UCB$ algorithm guarantees sub-linear regret when compared to both the pessimal and optimal stable regrets.
\end{corollary}
% \begin{proof}
% Let the pairs in the unique stable matching be indexed as $(a_1, f_1), (a_2, f_2), \dots, (a_n, f_n)$, in the order defined by the layers of the underlying $\alpha$-reducible market. Specifically, $(a_1, f_1)$ is the top pair, where both $a_1$ and $f_1$ rank each other first in their preference lists: $\langle f_1, \dots \rangle$ and $\langle a_1, \dots \rangle$, respectively. Recursively, each pair $(a_i, f_i)$ is defined as the top mutual choice after removing all previously formed pairs $\{(a_j, f_j)\}_{j < i}$.

% Now, consider each round $t$ in which the $\FGS$ algorithm is applied using submitted $\UCB$ estimates. At time $t$, agent $a_1$ is either matched with firm $f_1$ or with a firm $f_{a_1}(t)$ such that $f_{a_1}(t) \underset{\UCB_{a_1}}{\geqslant} f_1$. This follows because $a_1$ applies only to firms it prefers under $\UCB$, and if $f_{a_1}(t) \neq f_1$, then $a_1$ must have been rejected by all firms $f' \underset{\UCB_{a_1}}{\geqslant} f_1$, each of which prefers other agents over $a_1$. Importantly, once $a_1$ applies to $f_1$, the pair $(a_1, f_1)$ becomes stable—since no other agent can displace $a_1$ at $f_1$—and remains matched for all subsequent rounds.

% Therefore, whenever $f_{a_1}(t) \neq f_1$, the $\UCB$-sorted list of $a_1$ is of the form $\langle \dots, f_{a_1}(t), \dots, f_1, \dots \rangle$, and the $\UCB$ value of $f_1$ increases by definition of the estimator in~\eqref{eq:UCB-index}. Eventually, the ranking flips and $f_{a_1}(t) = f_1$ holds. Thus, agent $a_1$—being at the top layer of the $\alpha$-reducibility structure—always converges to its correct match and incurs sublinear regret.

% This property extends to all agents $\{a_i\}_{i \geq 2}$. We argue that the $\UCB$ algorithm cannot remain indefinitely in a configuration where every agent $a_i$ satisfies $f_{a_i}(t) \neq f_i$ and $f_{a_i}(t) \underset{\UCB_{a_i}}{\geqslant} f_i$. In such a case, the $\UCB$ values of the true firms $f_i$ increase over time, ensuring that $a_1$ is eventually matched with $f_1$.

% There may, however, be instances where $a_1$ is matched with $f_1$ even though it does not rank $f_1$ highest under $\UCB$. This occurs when $a_1$ is blocked or blocking other agents in lower layers from reaching their true matches. In such cases, overestimated $\UCB$ values for blocked firms persist, potentially causing linear regret for lower-layer agents.

% To rule out this possibility, assume $f_{a_1}(t) = f_1$ and let $i$ be the smallest index such that $a_i$ is blocked from matching with its true firm $f_i$ due to higher-layer agents. Let $j$ be such that $f_{a_j}(t) = f_i$. By $\alpha$-reducibility, $j < i$ since lower-index agents cannot be blocked by higher ones. Moreover, $a_j$ is not blocked from accessing $f_j$, meaning $f_{a_j}(t) = f_i \underset{\UCB_{a_j}}{\geqslant} f_j$. Consequently, the $\UCB$ value of $f_j$ increases until $f_j \underset{\UCB_{a_j}}{\geqslant} f_{a_j}(t)$ holds. This lowers the index $i$ of the topmost blocked agent.

% This process continues recursively, eventually reaching $a_1$, for whom no blocking is possible. Once the pair $(a_1, f_1)$ stabilizes, it can be removed from the market, and the same argument applies inductively to the remaining agents.


% \end{proof}





\section{Centralized UCB Algorithm}\label{sec:cucb}
The key distinction between this algorithm and the previous one lies in the fact that the $\UCB$ algorithm does not require agents or the central platform to know $\Delta$. For simplicity, we assume $\intesize = 1$ in this case. In this algorithm, all agents submit their $\UCB$ estimates to the central platform, which then allocates the interviews by running the $\FGS$ algorithm on the submitted estimates. Following this, the platform assigns each firm an interview with their corresponding match. Subsequently, the agents update their $\UCB$ estimates for the next round.


Here is the formula of how agents update their UCB estimations at time step $t$:
\begin{align}
 \hat{u}_{a,f}(t) =\UCB_{a,f}(t)= \begin{cases}\infty & \text { if } T_{a,f}(t)=0 \\ \hat{\mu}_{a,f}(t)+\sqrt{\frac{3 \log t}{2 T_{a,f}(t-1)}} & \text { otherwise. }\end{cases}   \label{eq:UCB-index}
\end{align}

Where $T_{a,f}(t)$ is the number of times agent $a$ has interviewed with firm $j$ before round $t$.

We define $\Delta_{a,f}=u_a(f^*_a)-u_a(f)$ and $M_{a,f}$ as a set of all achievable matchings, which are not stable regarding the ground truth, and they include $a$ and $f$ matched together. We can argue that:
$$ \label{cucb1:1}
R_a(T) \leq \sum_{f: \Delta_{a,f}>0} \Delta_{a,f}\left(\sum_{m \in M_{a,f}} \mathbb{E} [T_m(T)]\right)
$$
$T_m(t)$ is the number of times matching $m$ is played by time step $t$.

\begin{theorem}\cite{liu2020competing}\label{theorem:rcucb}
Regret of agent $a$ up to time step $T$ satisfies:
    $$
R_a(T) \leq \sum_{f: \Delta_{a,f}>0} \Delta_{a,f}\left[\min _{\mathcal{Q} \in \mathcal{C}\left(M_a(f)\right)} \sum_{\left(a', f', f''\right) \in \mathcal{Q}}\left(\frac{4}{\sqrt{T}}+\frac{12 \log (T)}{\Delta_{a', f', f''}^2}\right)\right] ,
$$
\end{theorem}
where the triplet $(a',f',f'')$ corresponds to matchings under which $a'$ is matched with $f''$ but $a',f'$ makes a blocking pair there.

While existing algorithms achieve sublinear regret bounds, typically \( O(\log T) \), our goal is to leverage the power of interviews to significantly reduce the regret, ideally attaining a bound of \( O(1) \). To this end, we present learning algorithms that incorporate hint information to achieve such time-independent performance. We begin by introducing a single-agent bandit algorithm with hints, denoted by \(\ALLP\), and then adapt its structure by modifying the underlying metric, resulting in the variant \(\ALLP^{\hat{\mu}}\), which provably achieves \( O(1) \) regret.

